Optimizing Item and Subgroup Configurations for Social-Aware VR Shopping

Shopping in VR malls has been regarded as a paradigm shift for E-commerce, but most of the conventional VR shopping platforms are designed for a single user. In this paper, we envisage a scenario of VR group shopping, which brings major advantages over conventional group shopping in brick-and-mortar stores and Web shopping: 1) configure flexible display of items and partitioning of subgroups to address individual interests in the group, and 2) support social interactions in the subgroups to boost sales. Accordingly, we formulate the Social-aware VR Group-Item Configuration (SVGIC) problem to configure a set of displayed items for flexibly partitioned subgroups of users in VR group shopping. We prove SVGIC is NP-hard to approximate within $\frac{32}{31} - \epsilon$. We design an approximation algorithm based on the idea of Co-display Subgroup Formation (CSF) to configure proper items for display to different subgroups of friends. Experimental results on real VR datasets and a user study with hTC VIVE manifest that our algorithms outperform baseline approaches by at least 30.1% of solution quality.

==> stash/sec1_intro.tex <==
\section{Introduction} \label{sec:intro}

%With the rapid growth of mobile computing power, network bandwidth, and display technologies, 
Virtual Reality (VR) has emerged as a disruptive technology for social \cite{FBsocial}, travel \cite{VRtourism}, and E-commerce applications. \revise{Particularly, a marketing report about future retails from Oracle \cite{Oracle} manifests that 74\% of online retailers already had or were planning to implement VR and AI. Recently, International Data Corporation (IDC) forecasts the worldwide spending on VR/AR to reach USD 18.8 billion in 2020 \cite{IDC} including USD 1.5 billion in retails. It also foresees the VR/AR market to continue a huge growing trend (annual growth rate of 77\%) through at least 2023. Therefore, shopping in VR malls is regarded as a paradigm shift for E-commerce stores, evident by emerging VR stores such as Amazon's VR kiosks \cite{Amazon}, eBay and Myer's VR department store \cite{eBay}, Alibaba Buy+ \cite{Alibaba}, and IKEA VR Store \cite{IKEA}.} Although these VR shopping platforms look promising, most of them are designed only for a single user instead of a group of friends, who also often appear in brick-and-mortar stores. As a result, existing approaches for configuring the displayed items in VR shopping malls are based on personal preference (similar to online web shopping) without considering potential social discussions amongst friends on items of interests, which is reported as beneficial for boosting sales in the marketing literature \cite{MY14, ZX14, XZ18}. In this paper, with the support of \textit{\notionfull} (\notion), we envisage the scenario of group shopping with families and friends in the next-generation VR malls, where item placement is customized flexibly in accordance with both user preferences and potential social interactions during shopping.%\footnote{\label{vrchat}Customized display with different objects for each user has been widely adopted in VR shopping \cite{IKEA} and social \cite{VRChat} applications, e.g., in the IKEA demo \cite{IKEA} (at 0:40), the displayed furniture in the store may adapt to the preference of the user.}

%Comparison of scenarios (online/offline/VR(\notion) shopping systems)
The \notion\ technology \cite{RL14,LH18} naturally enables VR group shopping systems with two unique strengths:  1) \textit{Customization}. \revise{IKEA (see video \cite{IKEA} at 0:40) and Lowe's \cite{Lowes} respectively launch VR store applications where the displayed furnitures may adapt to the preferences of the users, which attracts more than 73\% of the users to recommend IKEA VR store \cite{IKEAsteam}. Alibaba's \cite{AlibabaForbes} and eBay's VR stores \cite{ebaymacy} also devote themselves to provide personalized product offers. According to a marketing survey, 79\% of surveyed US, UK, and China consumers are likely to visit a VR store displaying customized products \cite{forbessurvey}.} Similar to group traveling and gaming in VR, the virtual environments (VEs) for individual users in VR group shopping need not be identical. While it is desirable to have consistent high-level layout and user interface for all users, the displayed items for each user can be customized based on her preferences. As CID allows different users to view different items at the same display slot, personalized recommendation is supported.

2) \textit{Social Interaction}. While a specific slot no longer needs to display the same items to all users, users viewing a common item may engage a discussion on the item together, potentially driving up the engagement and purchase conversion \cite{ZX14, XZ18}. As a result, the displayed items could be tailored to maximize potential discussions during group shopping. \revise{A survey of 1,400 consumers in 2017 shows that 65\% of the consumers are excited about VR shopping, while 54\% of them acknowledge social shopping as their ways to purchase products~\cite{wssurvey}. The L.E.K. consulting survey \cite{leksurvey} shows that 70\% of 1,000 consumers who had already experienced VR technology are strongly interested in virtual shopping with friends who are not physically present. Embracing the trend, Shopify \cite{shopify} and its technical partner Qbit \cite{Qbit} build a social VR store supporting attendance of multiple users with customized display \cite{Qbitstore}.} In summary, compared with brick-and-mortar shopping, VR group shopping can better address the preferences of individuals in the group due to the new-found flexibility in item placement, which can be configured not only for the group as a whole but also for individuals and subgroups. On the other hand, compared with conventional E-commerce shopping on the Web, VR group shopping can boost sales by facilitating social interactions and providing an immersive experience.

\begin{figure}[tp]
	\centering
	\subfigure[b][Comparison of different approaches.] {\
		\centering \includegraphics[width = 0.95 \columnwidth]{fig/Example_New_Short.pdf}
		\label{fig:example} }
	\subfigure[b][Item assignments of different approaches.] {\
		\centering \includegraphics[width = 0.95 \columnwidth]{fig/Example_New_Add.pdf}
		\label{fig:example_add} }
	\subfigure[b][\centering Alice's view at slot 1.] {\
		\centering \includegraphics[width = 0.46 \columnwidth]{fig/example_slot1_zipped.pdf}
		\label{fig:example_slot1} } 
		\hfill
	\subfigure[b][\centering Alice's view at slot 2.] {\
		\centering \includegraphics[width = 0.46 \columnwidth]{fig/example_slot2_zipped.pdf}
		\label{fig:example_slot2} }
	\caption{Illustrative example.}
	\label{fig:comp_example}
\end{figure}

% Comparison of recommendation systems (personalized, group, social-aware, ours)
\revise{Based on the above evidence, we make the first attempt to formulate the challenging problem of configuring displayed items for {\em \scenariofull} (\scenario) shopping. } Our strategy is to meet the item preferences of individual users via customization while enhancing potential discussions by displaying common items to a shopping group (and its subgroups). For customization, one possible approach is to use existing personalized recommendation techniques \cite{HR16AAAI, XH17, JC17SIGIR} to infer individual user preferences, and then retrieve the top-$k$ favorite items for each user. However, this \personalized\ approach fails to promote items of common interests that may trigger social interactions. 
%Even though social-aware personalized recommendation systems have been proposed \cite{HL16KDD, WXZ16TKDE}, their emphases are still on deriving individual preferences on items \textbf{from the influence and preferences of friends}. In other words, typical personalized recommendation systems \textbf{(e.g., for online web shopping)} cannot be directly exploited to simultaneously form subgroups and choose different items to encourage social interactions in the same subgroup. 
To encourage social discussions, %An alternative \textit{\group\ approach} is to leverage 
conventional group recommendation systems \cite{LH14,SQ16,SD17, CYS18} may be leveraged to retrieve a bundled itemset for all users. Nevertheless, by presenting the same configuration for the whole group of all users, this approach may sacrifice the diverse individual interests. 
% A third approach is to first partition the users into subgroups with similar interests \cite{SBR15}, then exploit group recommendation systems to determine separate configurations for different subgroups. However, by partitioning the users into static subgroups, this approach does not exploit the flexible CID technology to render flexible subgroup configurations. Also, grouping users with similar interests together do not guarantee the social tightness between subgroup members for them to enjoy social interactions. Furthermore, \textit{fairness} among personal preferences are left unaddressed, as members of a subgroup still view a universal set of items. 
%With the power of \notion, in this paper, we study the problem of configuring item displays for \scenario\ shopping flexibly by simultaneously examining personal preferences, social interactions, and subgroup partitioning. %, while also controlling the changes between the partitioned subgroups at adjacent display slots. 
In the following example, we illustrate the difference amongst the aforementioned approaches, in contrast to the desirable \scenario\ configuration we target on.

\begin{example} [Illustrative Example] \label{example:illustrative}
Figure \ref{fig:example} depicts a scenario of group shopping %compares a flexibly constructed configuration designed for \scenario\ shopping (thus denoted by \scenario) against the \personalized\ and \group\ approaches %, and two subgroup formation schemes, namely \textit{\preference} and \textit{\friendship}, 
for a VR store of digital photography. At the upper left is a social network $G = (V, E)$ of four VR users, Alice, Bob, Charlie, and Dave (indicated by red circles, green squares, blue pentagons, and brown hexagons, respectively). On top is an item set $C$ consisting of five items: tripod, DSLR camera, portable storage device (PSD), memory card, and self-portrait (SP) camera. Given three display slots, the shaded areas, corresponding to different configuration approaches, illustrate how items are displayed to individuals or subgroups (in black rectangles), respectively. For instance, in \scenario, the SP camera is displayed at slot 1 to Alice, Charlie, and Dave to stimulate their discussion. \revise{Figure \ref{fig:example_add} shows the same configuration as Figure \ref{fig:example} by depicting the individual item assignments for each user in each approach.} %Note that all slots for each user are filled for full utilization, e.g., for user Bob, the DSLR camera, tripod, and memory card are displayed at slots 1 to 3, respectively. 

A configuration based on the \personalized\ approach is shown in the light-green shaded area. It displays the top-3 items of interests to individual users based on their preferences (\revise{which is consistent to the numerical example shown in Table \ref{table:sat} in Section \ref{sec:problem}}). This configuration, aiming to increase the exposure of items of interests to customers, does not have users seeing the same item at the same slot. Next, the configuration shaded in light-orange, based on the \group\ approach, displays exactly the same items to every user in the group. While encouraging discussions in the whole group, this configuration may sacrifice some individual interests and opportunities to sell some items, e.g., Dave may not find his favorite item (the memory card). %Finally, the \friendship\ and \preference\ approaches at the bottom partition the users into two subgroups either based on their friendships (shown in the grey area) or their preferences (shown in the blue area). Accordingly, the displayed items are configured targeting on each subgroup as a unit, which remains the same across different display slots. As a result, in the \friendship\ scheme, users with diverse interests may be forced to see the same items together. On the other hand, in the \preference\ scheme, some pairs of friends, e.g., Alice and Dave, never have a chance to interact, as they are partitioned into separate subgroups. Moreover, some users, e.g., Charlie and Dave, could share views of identical items but do not know each other. 
Aiming to strike a balance between the factors of individual preferences and social interactions, the \scenario\ configuration forms subgroups flexibly across the displayed slots, having some users seeing the same items at the same slots (to encourage discussions), yet finding items of individual interests at the remaining slots. For example, the tripod is displayed at slot 2 to all users except for Charlie, who sees the PSD on his own. The DSLR camera is displayed to Bob at slot 1 and to Alice at slot 3, respectively, satisfying their individual interests. Figures \ref{fig:example_slot1} and \ref{fig:example_slot2} show Alice's view at slot 1 and slot 2, respectively, in this configuration. As shown, Alice is co-displayed the SP camera with Charlie and Dave at slot 1 (informed by the user icons below the primary view of the item), then co-displayed the Tripod with Bob and Dave at slot 2. As shown, \scenario\ shopping displays items of interests to individuals or different subgroups at each slot, and thereby is more flexible than other approaches.\hfill \qedsymbol
\end{example}

%The aspects (challenges) in the research problem
%As illustrated above, SAVG configuration is made possible in VR shopping because 
%As suggested in the above example, the configuration of displayed items for \scenario\ shopping considers the factors of personal preferences, social interactions, and subgroup partition, because unlike brick-and-mortar stores, 
%\notion\ technology, \textbf{(widely adopted by [TODO]),} is able to display different or common items at the same slot for different individuals or subgroups \cite{RL14,LH18}, satisfying personal preferences while encouraging social discussions. While emphasizing personal preferences is an intuitive strategy for displayed item configuration, encouraging social discussions triggers interests and boosts sales of products, especially for those new arrivals \textbf{due to social influence among friends }\cite{ZX14}. Properly partitioning subgroups by taking into account these two factors may provide a balanced trade-off between them. 
%The novel notion and problem / problem gaps.
%To systematically incorporate the considered factors in configuring the displayed items for a group of VR shoppers
%Accordingly, 
As illustrated above, in addition to identifying which items to be displayed in which slots, properly partitioning subgroups by balancing both factors of personal preferences and social discussions is critical for the above-depicted \scenario\ shopping. In this work, we define the notion of \textit{\configuration}, which \textit{specifies the partitioned subgroups (or individuals) and corresponding items for each of the allocated $k$ slots.} We also introduce the notion of \textit{co-display} that represents users sharing views on common items. Formally, we formulate a new optimization problem, namely \textit{\problem} (\prob), to find the optimal \configuration\ that maximizes the overall 1) \textit{preference utility} from users viewing their allocated items and 2) \textit{social utility} from all pairs of friends having potential discussions on co-displayed items, where the basic preference utility of an individual user on a particular item and the basic social utility of two given users on a co-displayed item are provided as inputs. Meanwhile, we ensure that no duplicated items are displayed at different slots to a user. \delete{(called \textit{no-duplication} constraint).} The problem is very challenging due to a complex trade-off between prioritizing personalized item configuration and facilitating social interactions. \delete{Notice that it is different from traditional community detection and group query problems, since 1) distinct displayed items (correlated to preference) and the discussion subgroup for each item (correlated to social tightness) need to be found simultaneously; 2) the displayed items and the discussion subgroups vary across all display slots; 3) the no-duplication constraint for all individual users is essential. }Indeed, we prove that \revise{it is $\mathsf{NP}$-hard to approximate \prob\ within a ratio of $\frac{32}{31}-\epsilon$.}

%$\mathsf{APX}$-hard, i.e., it admits no polynomial-time approximation schemes (PTAS) unless $\mathsf{P}=\mathsf{NP}$.

To solve \prob, we first present an Integer Program (IP) as a baseline to find the exact solution which requires superpolynomial time. To address the efficiency issue while ensuring good solution quality, we then propose a novel approximation algorithm, namely \textit{\algofull} (\algo), to approach the optimal solution in polynomial time. Specifically, \algo\ first relaxes the IP to allow fragmented \configuration s, and obtains the optimal (fractional) solution of the relaxed linear program. It then assigns the fractional decision variables derived from the optimal solution as the \textit{\weight s} for various potential allocations of user-item-slot in the solution. Items of high \weight s are thus desirable as they are preferred to individuals or encouraging social discussions. Moreover, by leveraging an idea of \textit{dependent rounding}, \algo\ introduces the notion of \textit{\stagethreefull} (\stagethree) to strike a balance between personal preferences and social interactions in forming subgroups. \stagethree\ forms a \textit{target subgroup} of socially connected users with similar interests to display an item, according to a randomized \textit{\roundingalpha} on \weight s to determine the membership of the target subgroup. With \stagethree, \algo\ finds the subgroups (for all slots) and selects appropriate items simultaneously, and thereby is more effective than other approaches that complete these tasks separately in predetermined steps. Theoretically, we prove that \algo\ achieves 4-approximation in expectation. We then show that \algo\ can be derandomized into a deterministic 4-approximation algorithm for \prob. \revise{We design further LP transformation and sampling techniques to improve the efficiency of \algo.}

%Properly setting the \roundingalpha\ is essential for finding effective subgroups. Thus, we further propose two strategies, namely \textit{Randomized Focus Selection} (RFS) and \textit{Deterministic Focus Selection} (DFS), to determine the \roundingalpha s. Between them, the more efficient RFS uniformly samples the \roundingalpha s but achieves a weaker theoretical guarantee. In contrast, DFS carefully selects \roundingalpha s to jointly optimize the current and expected future increments of total utility obtained by \stagethree, in order to form subgroups selectively. Moreover, \textbf{[summarizing of the extensions this time.]} %we introduce additional variables and constraints in the IP to support a number of practical considerations, such as controlling the subgroup changes and enabling Multi-View Display in VR. 
 %Through the investigation, we also find that the computational problem of \prob\ has other applications not only for the context of VR but also for the physical world, such as Social Event Organization (SEO) \cite{KL14KDD,XW18WWW} for a series of events.% Compared with the above research focusing on a single event without considering the dependency of social benefits on the candidate events, we show that \algo\ can support the organization of \textit{``series of events''} with capacity constraints across a time period, while also complying to different user schedules.

Next, we enrich \prob\ by taking into account some practical VR operations and constraints. We define the notion of \textit{indirect co-display} to capture the potential social utility obtained from friends displayed a common item at two different slots in their VEs, where discussion is facilitated via the \textit{teleportation} \cite{BE16} function in VR. We also consider a \textit{subgroup size constraint} on the partitioned subgroups at each display slot due to practical limits in VR applications. Accordingly, we formulate the \problemtwo\ (\probtwo) problem, and prove that \probtwo\ is unlikely to be approximated within a constant ratio in polynomial time. Nevertheless, we extend \algo\ to support \probtwo\ and guarantee feasibility of the solution. \revise{Moreover, we have extended \algo\ to support a series of practical scenarios. 1) \textit{Commodity values}. Each item is associated with a commodity value to maximize the total profit.  2) \textit{Layout slot significance}. Each slot location is associated with a different significance (e.g., center is better) according to retailing researches \cite{slot, shelf}. 3) \textit{Multi-View Display}, where a user can be displayed multiple items in a slot, including one default, personally preferred item in the \textit{primary view} and multiple items to view with friends in \textit{group views}, and the primary and group views can be freely switched. 4) \textit{Generalized social benefits}, where social utility can be measured from not only the pairwise (each pair of friends) but also group-wise (any group of friends) perspectives. 5) \textit{Subgroup change}, where the fluctuations (i.e., change of members) between the partitioned subgroups at consecutive slots are limited to ensure smooth social interactions as the elapse of time. 6) \textit{Dynamic scenario}, where users dynamic join and leave the system with different moving speeds. Finally, we have also identified \textit{Social Event Organization} (SEO) as another important application of the targeted problem. \opt{short}{Due to the space limit, the details of \probtwo, as well as the above extensions, are presented in the full version \cite{Online} of this paper.}} 

The contributions of this work are as follows:
\begin{itemize}
    \sloppy \item We coin the notion of \configuration\ under the context of VR group shopping and formulate the \prob\ problem, aiming to return an \configuration\ that facilitates social interactions while not sacrificing the members' individual preferences. We prove \prob\ is \revise{$\mathsf{NP}$-hard to approximate within $\frac{32}{31} - \epsilon$.}
    \item We systematically tackle \prob\ by introducing an IP model and designing an approximation algorithm, \algo, based on the idea of \stagethreefull\ (\stagethree) that leverages the flexibility of \notion\ to partition subgroups for each slot and display common items to subgroup members. 
    \opt{full}{\item We define the \probtwo\ problem to incorporate teleportation and subgroup size constraint. We prove \probtwo\ admits no constant-ratio polynomial-time approximation algorithms unless ETH fails. We extend \algo\ to obtain feasible solutions of \probtwo.}
    \item A comprehensive evaluation on real VR datasets and a user study implemented in Unity and hTC VIVE manifest that our algorithms outperform the state-of-the-art recommendation schemes by at least 30.1\% in terms of solution quality. \opt{short}{The code and VR implementation can be downloaded at \cite{Online}.}
\end{itemize}

This paper is organized as follows. Section \ref{sec:related} reviews the related work. \opt{short}{Section \ref{sec:problem} formally defines the notion of \configuration, then formulates the \prob\ problem and an IP model.}\opt{full}{Section \ref{sec:problem} formally defines the notion of \configuration, then formulates the \prob\ and \probtwo\ problems and IP models for them.} Then, Section \ref{sec:algo} details the proposed \algo\ algorithm and the theoretical results. \revise{Section \ref{sec:extension} discusses the extension directions. }Section \ref{sec:exp} reports the experimental results, and Section \ref{sec:conclusion} concludes this paper.

==> stash/sec2_related.tex <==
\section{Related Work} \label{sec:related}
\para{Group Recommendation.}
\sloppy Various schemes for estimating group preference have been proposed by aggregating features from different users in a group \cite{SQ16,SD17}. Cao \etal \cite{DC18} propose an attention network for finding the group consensus. However, sacrificing personal preferences, the above group recommenders assign a unified set of items for the entire group based only on the aggregate preference without considering social topologies. For advanced approaches, recommendation-aware group formation \cite{SBR15} forms subgroups according to item preferences. SDSSel \cite{CYS18} finds dense subgroups and diverse itemsets. Shuai \etal \cite{HHS18WWW} customize the sequence of shops without considering \notion. However, the above recommenders find \textit{static} subgroups, i.e., a universal partition, and still assign a fixed configuration of items to each subgroup, where every subgroup member sees the same item in the same slot. In contrast, the \scenario\ approach considered in this paper allows the partitioned subgroups to vary across all display slots and thereby is more flexible than the above works.%, whereas VR-specific operation, i.e., teleportation, can be supported in \scenario\ to facilitate discussions across different slots.}

\para{Personalized Recommendation.}
Personalized recommendation, a cornerstone of E-commerce, has been widely investigated. A recent line of study integrates deep learning with Collaborative Filtering (CF) \cite{LZ15,JC17SIGIR} on heterogeneous applications \cite{RG17}, while Bayesian Personalized Ranking \cite{SR09, HC16CIKM} is proposed to learn the ranking of recommended items. However, the above works fail to consider social interactions. While social relations have been leveraged to infer preferences of products \cite{WXZ14KDD,WXZ16TKDE}, POIs \cite{HL16KDD}, and social events \cite{YL18TOIS}, they do not take into account the social interactions among users in recommendation of items. Thus, they fail to consider the trade-off between social and personal factors. In this paper, we exploit the preferences obtained from such studies to serve as inputs for the tackled problems.
%TRecSo \cite{PC16WWW} proposes a top-$k$ recommendation approach by incorporating social trust information. %VBPR \cite{HR16AAAI} combines visual features for fashion recommendation. He \etal \cite{JH16} propose a unified tensor-based latent model for POI recommendation by fusing check-in behavior and latent behavior pattern of each user.
%TranSIV \cite{XL17CIKM} learns social relations and item preferences simultaneously by transfer learning. 
%SBPR \cite{ZT14} and TBPR \cite{XW16CIKM} investigate how different levels of social strengths may affect users' ratings.

\para{Social Group Search and Formation.}
Research on finding various groups from online social networks (OSNs) for different purposes has drawn increasing attention in recent years. %Community detection extracts dense connected subgroups \cite{JY13, XJ13}. On the other hand, 
Community search finds similar communities containing a given set of query nodes \cite{JL17, LC18}. %, which does not extract all communities from a network as community detection. 
Group formation organizes a group of experts with low communication costs and specific skill combinations \cite{MK13, RSS13}. In addition, organizing a group in location-based social networks (LBSNs) based on certain spatial factors has also gained more attention \cite{CYS16TKDE, CYS16TKDD}. Socio-Spatial Group Queries \cite{DY12, CYS16TKDE} find socially tight groups and select proper rally points for the groups. %Geo-Social Ranking ranks $k$ users according to the distance to a query location and social relations \cite{AN15}. %Spatial-Social Team Query \cite{CYS16TKDD} and Geo-Social K-Cover Group Query \cite{YL15} forms socially tight groups covering spatial locations or skill requirements. 
The problems tackled in the above studies are fundamentally different from the scenario in this paper, since they focus on retrieving only \textit{parts} of the social network according to some criteria, whereas item selection across multiple slots is not addressed. Instead, \scenario\ group shopping aims to configure item display for all VR shopping users, whereas the subgroups partition the entire social network.%An intuitive approach is to make Point-of-Interests (POIs) as the items and the distance as the reverse of preference, such that the output rally point corresponds to an item. However, it still fails to flexibly organize the subgroups in \notion\ because the rally point is unified. Moreover, directly iterating the social queries for all slots does not control the subgroup changes to ensure user experience.

\revise{
\para{Related Combinatorial Optimization Problems.}
\prob\ is related to the \textit{Multi-Labeling} (ML) \cite{multilabeling} problem and its variations, including {Multiway Partition} \cite{multilabeling, multiwaypartition}, \textit{Maximum Happy Vertices/Edges} (MHV/MHE) \cite{homophyly}, and \textit{Multiway Cut} \cite{multiwaycut} in graphs. 
\opt{short}{In Section \ref{subsec:hardness_ip}, we revisit the challenging combinatorial nature of the proposed \prob\ problem and its relation with the related problems, whereas detailed introduction of each problem, as well as a summary table, are presented in the full version \cite{Online}.}\opt{full}{In Section \ref{subsec:combinatorial}, we revisit the challenging combinatorial nature of the proposed \prob\ problem and its relation with the related problems with detailed introduction of all problems and a summary table.}
}


==> stash/sec3_problem.tex <==
\section{Problem Formulation and Hardness Results} \label{sec:problem}

\newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\small
\begin{table*}[t]
\centering
\caption{Preference and social utility values in Example \ref{example:running}.}
\label{table:sat}
\begin{tabular}{c||c|c|c|c||c|c|c|c|c|c|c|c}
      & $\text{p}(u_A,\cdot)$ & $\text{p}(u_B,\cdot)$ & $\text{p}(u_C,\cdot)$ & $\text{p}(u_D,\cdot)$ & \specialcell{$\tau(u_A,$\\$u_B,\cdot)$} & \specialcell{$\tau(u_A,$\\$u_C,\cdot)$} & \specialcell{$\tau(u_A,$\\$u_D,\cdot)$} & \specialcell{$\tau(u_B,$\\$u_A,\cdot)$} & \specialcell{$\tau(u_B,$\\$u_C,\cdot)$} & \specialcell{$\tau(u_C,$\\$u_A,\cdot)$} & \specialcell{$\tau(u_C,$\\$u_B,\cdot)$} & \specialcell{$\tau(u_D,$\\$u_A,\cdot)$} \\ \hline
$c_1$ & 0.8 & 0.7 & 0 & 0.1               & 0.2 & 0 & 0.2 & 0.2 & 0 & 0 & 0.1 & 0.3\\
$c_2$ & 0.85 & 1.0 & 0.15 & 0          & 0.05 & 0.05 & 0.05 & 0.05 & 0.05 & 0.05 & 0.05 & 0.05\\
$c_3$ & 0.1 & 0.15 & 0.7 & 0.3            & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.05\\
$c_4$ & 0.05 & 0.2 & 0.6 & 1.0            & 0  & 0 & 0.05 & 0.05 & 0.2 & 0.05 & 0.2 & 0\\
$c_5$ & 1.0 & 0.1 & 0.1 & 0.95            & 0.05 & 0.3 & 0.2 & 0.05 & 0 & 0.3 & 0.05 & 0.25\\
\end{tabular}
\end{table*}
\normalsize

\opt{full}{
\begin{table}[t!]
\caption{Notations used in \prob.}
\begin{center}
\begin{tabular}{|c|l|}\hline
Symbol & Description \\\hline\hline
$n$ & number of users \\\hline
$m$ & number of items \\\hline
$k$ & number of display slots \\\hline
$G = (V,E)$ & social network \\\hline
$V$ & user set/shopping group \\\hline
$E$ & (social) edge set \\\hline
$\mathcal{C}$ & Universal Item Set \\\hline
$\mathbf{A}(\cdot, \cdot)$ & \configuration\ \\\hline
$\mathbf{A}^{\ast}$ & optimal \configuration\ \\\hline
$\text{p}(u,c)$ & preference utility \\\hline
$\tau(u,v,c)$ & social utility \\\hline
$\text{w}_{\textbf{A}}(u,c)$ & \scenario\ utility \\\hline
$\lambda$ & weight of social utility\\\hline
$\text{p'}(u,c)$ & scaled preference utility \\\hline
$u \xleftrightarrow[s]{c} v$ & Co-display (at slot $s$) \\\hline
$u \xleftrightarrow{c} v$ & Co-display (at some slot) \\\hline
$N_p(s)$ & user subgroups \\\hline
$V^s$ & collection of subgroups at slot $s$ \\\hline
\multirow{2}{*}{$x^c_{u,s}$} & decision variable of \\ & $u$ displayed $c$ at slot $s$\\\hline
\multirow{2}{*}{$x^c_u$} & decision variable of \\ & $u$ displayed $c$\\\hline
\multirow{2}{*}{$y^c_{e,s}$} & decision variable of \\ & $u,v$ co-displayed $c$ at slot $s$\\\hline
\multirow{2}{*}{$y^c_{e}$} & decision variable of \\ & $u,v$ co-displayed $c$\\\hline
\end{tabular}
\label{tab:symbols_prob1}
\end{center}
\end{table}
}

%============SHORT VERSION HEADER================
\opt{short}{In this section, we first define the notion of \configuration\ and then formally introduce the \prob\ problem. We also prove its hardness of approximation, and introduce an integer program for \prob\ as a cornerstone for the \algo\ algorithm.}
%============FULL VERSION HEADER================
\opt{full}{In this section, we first define the notion of \configuration\ and then formally introduce the \prob\ and \probtwo\ problems. We also prove their hardness of approximation, and introduce integer programs for \prob\ and \probtwo\ as cornerstones for the \algo\ algorithm.}

\subsection{Problem Formulation} \label{subsec:problem}

Given a collection $\mathcal{C}$ of $m$ items (called the \textit{Universal Item Set}), a directed social network $G=(V,E)$ with a vertex set $V$ of $n$ users (i.e., shoppers to visit a VR store) and an edge set $E$ specifying their social relationships. In the following, we use the terms \textit{user set} and \textit{shopping group} interchangeably to refer to $V$, and define \configuration\ to represent the partitioned subgroups and the corresponding items displayed at their allocated slots.

\begin{definition}{\textit{\configurationfull} \newline (\configuration).}
Given $k$ display slots for displaying items to users in a VR shopping group, an \configuration\ is a function $\mathbf{A}(\cdot, \cdot): (V \times [k]) \rightarrow \mathcal{C}$ mapping a tuple $(u,s)$ of a user $u$ and a slot $s$ to an item $c$. $\mathbf{A}(u,s) = c$ means that the configuration has item $c$ displayed at slot $s$ to user $u$, and $\mathbf{A}(u,:) = \langle \mathbf{A}(u,1), \mathbf{A}(u,2), ..., \mathbf{A}(u,k) \rangle$ are the $k$ items displayed to $u$. Furthermore, the function is regulated by a \textit{no-duplication constraint} which ensures the $k$ items displayed to $u$ are distinct, i.e., $\mathbf{A}(u,s) \neq \mathbf{A}(u,s'), \forall s \neq s'$.
\end{definition}

For shopping with families and friends, previous research \cite{MY14, ZX14, XZ18} demonstrates that discussions and interactions are inclined to trigger more purchases of an item. \revise{Specifically, the VR technology supporting social interaction has already been employed in existing VR social platforms, e.g., VRChat \cite{VRChat}, AltspaceVR \cite{AltspaceVR}, and Facebook Horizon \cite{fbHorizon}, where users, represented by customized avatars, interact with friends in various ways: 1) \textit{Movement and gesture.} Commercial VR devices, e.g., Oculus Quest and HTC Vive Pro/Focus, support six-degree-of-freedom (6DOF) headsets and hand-held controllers to detect the user movements and gestures in real-time. These movements are immediately updated to the server and then perceived by other users. For example, Rec Room \cite{RecRoom} uses a high-five gesture mechanism to let users befriend others. 2) \textit{Emotes and Emojis.} Similar to Emoticons in social network platforms, VR users can present their emotions through basic expressions (happy face, sad face, etc.) or advanced motions (e.g., dance, backflip, and die in VRChat \cite{VRChatGuide}). 3) \textit{Real sound.} This allows users to communicate with friends verbally through their microphones. As such, current VR applications support immersive and seamless social interaction, rendering social interactions realistic in shopping systems.}

\revise{With non-customized user environments in brick-and-mortar stores, discussing a specific item nearby its location is the default behavior. On the other hand, as users are displayed completely customized items in personalized e-commerce (e.g., the 20 items appearing at the main page of a shopping site can be completely disjoint for a pair of friends), it often requires a ``calibration'' step (e.g., sharing the exact hyperlink of the product page) to share the view on the target item before e-commerce users can engage in detailed discussion on some item. Therefore, shopping users are mostly used to having discussions on the common item they are viewing at the identical slot in their own Virtual Environments (VEs). Therefore, we devote to enhance the possibility of this intuitive setting in our envisioned VR shopping VEs even if other settings are also possible in VR.}

\revise{Therefore, for a pair of friends displayed a common item, it is the most convenient to display the item at the same slot in the two users' respective VEs such that they can locate the exact position easily (e.g., ``come to the second shelf; you should see this.''). Accordingly, upon viewing any item, It is expected that the user interface indicates a list of friends co-displayed the specific item to the current user, so that she is aware of the potential candidates to start a discussion with.} To display an item at the same slot to a pair of friends, we define the notion of \textit{co-display} as follows.

\begin{definition}{\textit{Co-display} ($u \xleftrightarrow[s]{c} v$).} Let $u \xleftrightarrow[s]{c} v$ represent that users $u$ and $v$ are \textit{co-displayed} % \opt{short}{\cite{Online}}\opt{full}{Section \ref{sec:extension}}. Moreover, \textit{group-wise} social utility will also be introduced in Section \ref{sec:extension}.}
an identical item $c$ at slot $s$, i.e., $\mathbf{A}(u,s) = \mathbf{A}(v,s) = c$. Let $u \xleftrightarrow{c} v$ denote that there exists at least one $s$ such that $u \xleftrightarrow[s]{c} v$.
\end{definition}

\noindent Naturally, the original group of users are partitioned into subgroups in correspondence with the displayed items. That is, for each slot $s \in [k]$, the \configuration\ implicitly partitions the user set $V$ into a collection of disjoint subsets. %\delete{$N_p(s)$ disjoint subsets $V^s = \{ V^s_1, V^s_2, \cdots, V^s_{N_p(s)} \}$, such that $u \xleftrightarrow[s]{c} v$ if and only if $u,v \in V^s_i, i = 1, \cdots, N_p(s)$.}

\revise{Under the scenario of brick-and-mortar group shopping, previous research \cite{XL05, LQS13, MY14, LB16, XZ18} indicates that the satisfaction of a group shopping user is affected by two factors: \textit{personal preference} and \textit{social interaction}. Furthermore, empirical research on dynamic group interaction in retail finds that shopping while discussing with others consistently boost sales \cite{MY14}, while within-group talk frequency has a significant impact on users' shopping tendency and purchase frequency \cite{ZX14, XZ18}. Accordingly, we capture the overall satisfaction by combining 1) the aggregated personal preferences and 2) the retailing benefits from facilitating social interactions and discussions. We note that, from an optimization perspective, these two goals form a trade-off because close friends/families may have diverse personal preferences over items. One possible way to simultaneously consider both factors is to use an end-to-end machine learning-based approach, which generates the \textit{user embeddings} and \textit{item embeddings} \cite{DC18} and designs a neural network aggregator to derive the total user satisfaction. However, this approach requires an algorithm to generate candidate configuration for ranking and relies on a huge amount of data to train the parameters in the aggregator. On the other hand, previous research \cite{HHS13, XW18WWW} has demonstrated that a \textit{weighted combination} of the preferential and social factors is effective in measuring user satisfaction, where the weight can be directly set by a user or implicitly learned from existing models \cite{ZT14,YL18TOIS}. Another possible objective is a weighted sum of the previous objective metric (the aggregated preference) with the aggregated social satisfaction as the constraint, or vice versa, which is equivalent to our problem after applying Lagrangian relaxation to the constraint. Therefore, we follow \cite{HHS13, XW18WWW} to define the \scenario\ utility as a combination of \textit{aggregated preference utility} and \textit{aggregated social utility}, weighted by a parameter $\lambda$.} 

% The original (pre-revision) paragraph
%Following previous research \cite{XL05, LQS13, LB16, XZ18}, the satisfaction of a group shopping user consists of two factors: 1) her individual preference on the displayed items and 2) the satisfaction from sharing views and having potential discussions with friends. One intuitive way of modeling both factors is to maximize the aggregated preference while ensuring the aggregated social satisfaction is over a predefined threshold. However, this approach requires fine-tuning of the threshold.\footnote{A low threshold of social satisfaction could be too easy to meet and thereby not optimized enough, whereas a high threshold is prone to render the problem infeasible.} In contrast, previous research \cite{HHS13, XW18WWW} has shown that a weighted combination of the preferential and social factors is effective in measuring user satisfaction. This formulation can also be viewed as a Lagrange Relaxation of the above constrained problem, and the best feasible solution of the constrained problem can thus be effectively approximated by scanning different combination weights.% of $\lambda$ (detailed later) in \prob.

Specifically, for a given pair of friends $u$ and $v$, i.e., $(u,v) \in E$, and an item $c \in \mathcal{C}$, let $\text{p}(u,c) \geq 0$ denote the \textit{preference utility} of user $u$ for item $c$, and let $\tau(u,v,c) \geq 0$ denote the \textit{social utility} of user $u$ from viewing item $c$ together with user $v$, %i.e., $u \xleftrightarrow{c} v$, 
where $\tau(u,v,c)$ can be different from $\tau(v,u,c)$.
Following \cite{HHS13, XW18WWW}, the \textit{\scenario\ utility} is defined as follows.

\begin{definition}{\textit{\scenario\ utility} \label{def:savg_utility} ($\mathbf{w}_{\textbf{A}}(u,c)$).}
Given an \configuration\ $\textbf{A}$, the \scenario\ utility of user $u$ on item $c$ in $\textbf{A}$ represents a combination of the preference and social utilities, where $\lambda \in [0,1]$ represents their relative weight.% between preference and social utilities.

\opt{short}{\vskip -10pt}

\begin{align*}
    \text{w}_{\textbf{A}}(u,c) = (1-\lambda)\cdot\text{p}(u,c) + \lambda\cdot\sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c)
\end{align*}

\opt{short}{\vskip -35pt}

\end{definition}

\noindent \revise{The preference and social utility values can be directly given by the users or obtained from social-aware personalized recommendation learning models \cite{ZT14,YL18TOIS}. Those models, learning from purchase history, are able to infer $(u,c)$ and $(u,v,c)$ tuples to relieve users from filling those utilities manually.} The weight $\lambda$ can also be directly set by a user or implicitly learned from existing models \cite{ZT14,YL18TOIS}. %\footnote{Another approach is to generate the user and item embeddings and design a neural network aggregator to derive the total \textit{\scenario\ utility}. However, this approach requires a huge amount of data to learn the parameters and still needs to generate candidates as the model input. 
\revise{To validate the effectiveness of this objective model, we have conducted a user study in real \notion\ VR shopping system which shows high correlations between user satisfaction and the proposed problem formulation (Please see Section \ref{sec:user_study} for the results).} 
%Moreover, we also study the influence of different values of $\lambda$ in Section \ref{sec:exp}.}
%Later our VR user study results verify that the proposed \scenario\ utility is highly representative of the user satisfaction in \scenario\ shopping (Spearman correlation of 0.835).} The impacts of different $\lambda $ are studied later in Section \ref{sec:exp}.

\begin{example} \label{example:running}
Revisit Example \ref{example:illustrative} where $\mathcal{C} = \{c_1, c_2, ..., c_5\}$ and let $V = \{u_A,u_B,u_C,u_D\}$ denote Alice, Bob, Charlie, and Dave, respectively. Table \ref{table:sat} summarizes the given preference and social utility values. For example, the preference utility of Alice to the tripod is $\text{p}(u_A, c_1) = 0.8$. In the \scenario\ 3-configuration described at the top of Figure \ref{fig:comp_example}, $\mathbf{A}(u_A,\cdot)=\langle c_5, c_1, c_2 \rangle$, meaning that the SP camera, the tripod, and the DSLR camera are displayed to Alice at slots 1, 2, and 3, respectively. Let $\lambda = 0.4$. At slot 2, Alice is \textit{co-displayed} the tripod with Bob and Dave. Therefore, $\mathbf{w}_{\textbf{A}}(u_A, c_1) = 0.6 \cdot 0.8 + 0.4 \cdot (0.2 + 0.2) = 0.64$. \hfill \qedsymbol
\end{example}
%

\noindent We then formally introduce the \prob\ problem as follows. \opt{full}{All used notations in \prob\ are summarized in Table \ref{tab:symbols_prob1}.}%\newpage

\vskip 0.06in
\hrule
\vskip 0.03in

\noindent \textbf{Problem:} Social-aware VR Group-Item Configuration.% (\prob).

\noindent \textbf{Given:} A social network $G=(V,E)$, a universal item set $\mathcal{C}$, preference utility $\text{p}(u,c)$ for all $u \in V$ and $c \in \mathcal{C}$, social utility $\tau(u,v,c)$ for all $(u,v) \in E$ and $c \in \mathcal{C}$, the weight $\lambda$, and the number of slots $k$.

\noindent \textbf{Find:} An \configuration\ $\mathbf{A}^{\ast}$ to maximize the total \scenario\ utility 
\opt{short}{\vskip -0.3in}
$$\sum_{u \in V} \sum_{c \in \mathbf{A}^{\ast}(u,\cdot)} \text{w}_{\mathbf{A}^{\ast}}(u,c),$$
%$$ \sum\limits_{u \in V} \sum\limits_{c \in \mathbf{A}^{\ast}(u,\cdot)} [(1-\lambda) \cdot \text{p}(u,c) + \lambda \cdot \sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c)]. $$
\noindent where $\text{w}_{\mathbf{A}^{\ast}}(u,c)$ is the \scenario\ utility defined in Definition \ref{def:savg_utility}, and the no-duplication constraint is ensured.

\vskip 0.03in
\hrule
\vskip 0.06in

\opt{short}{Finally, we remark here that the above additive objective function in \prob\ can be viewed as a generalization of more limited variations of objectives. For instance, some objectives in personal/group recommendation systems without considering social discussions, e.g., the AV semantics in \cite{SBR15}, %\footnote{Other optimization criteria in existing group recommenders, e.g., Least-Misery (LM) \cite{SBR15} that considers fairness, can be considered. Later we show that the regret ratio (a metric for fairness) of our proposed methods still outperforms other baselines on real datasets.} 
are special cases of \prob\ where $\lambda = 0$. We detail this in Section \ref{subsec:problem} in the full version \cite{Online}.}

\opt{full}{
\begin{table}[t!]
\caption{Notations used in \probtwo.}
\begin{center}
\begin{tabular}{|c|l|}\hline
Symbol & Description \\\hline\hline
$\text{w'}_{\textbf{A}}(u,c)$ & \scenario\ utility with indirect co-display \\\hline
$u \xleftrightarrow[s,s']{c} v$ & Indirect Co-display (at slots $s,s'$) \\\hline
$u \xleftrightarrow[\text{ind}]{c} v$ & Indirect Co-display (at some slots) \\\hline
$\text{d}_{\text{tel}}$ & discount factor \\\hline
$M$ & subgroup size constraint \\\hline
$z^c_e$ & decision variable of $u,v$ co-displayed $c$\\\hline
\end{tabular}
\label{tab:symbols_prob2}
\end{center}
\end{table}
}

%============END OF THE DEFINITION OF THE BASIC PROBLEM================

%============MISC ON THE BASIC PROBLEM (COMPARISON AGAINST SPECIAL CASES)================

\opt{full}{
Based on \prob, we have the following observation on several special cases of this problem. The \personalized\ approach, introduced in Section \ref{sec:intro}, is a special case of \prob\ with $\lambda$ set to $0$. In this special case, it is sufficient to leverage personalized (or social-aware personalized) recommendation systems to infer the personal preferences, because the problem reduces into trivially recommending the top-$k$ favorite items for each user. On the other hand, the \group\ approach is also a special case of \prob\ with $N_p(s) = 1$ for each $s$, i.e., all users view the same item at the same slot. However, the combinatorial complexity of the solution space for \prob\ is $\Theta(m^{nk})$ due to the flexible partitioning of subgroups across different display slots in \scenario. Formally, $\textbf{A}(u,s) = \textbf{A}(v,s), \forall u,v \in V, s = 1,\cdots, k$, which corresponds to a group recommendation scenario.  

Due to the complicated interplay and trade-off of preference and social utility, the following theorem manifests that the optimal objective value of \prob\ can be significantly larger than the optimal objective values of the special cases above, corresponding to \personalized\ and \group\ approaches. Specifically, for each problem instance $\mathbf{I}$, let $\text{OPT}(\mathbf{I})$ denote the optimal objective value of \prob. Let $\text{OPT}_{\text{P}}(\mathbf{I})$ and $\text{OPT}_{\text{G}}(\mathbf{I})$ respectively denote the optimal objective values of the special cases of \personalized\ and \group\ approaches in the above discussion, i.e., \prob\ with $\lambda = 1$, and \prob\ with $N_p(s) = 1$ for each slot $s$, respectively.

\begin{restatable}{theorem}{gap} \label{thm:problem_gap}
Given any $n$, there exists 1) a \prob\ instance $\mathbf{I}_\text{G}$ with $n$ users such that $\frac{\text{OPT}(\mathbf{I}_\text{G})}{\text{OPT}_{\text{G}}(\mathbf{I}_\text{G})} = n$. 2) a \prob\ instance $\mathbf{I}_\text{P}$ such that $\frac{\text{OPT}(\mathbf{I}_\text{P})}{\text{OPT}_{\text{P}}(\mathbf{I}_\text{P})} \geq \frac{\lambda}{1-\lambda} \cdot \frac{n-1}{2} = O(n)$.
\end{restatable}

\begin{proof}
We construct $\mathbf{I}_\text{G}$ and $\mathbf{I}_\text{P}$ as follows. For $\mathbf{I}_\text{G}$, each user $u_i$ in $\mathbf{I}_\text{G}$ prefers exactly $k$ items $\mathcal{C}_i = \{ c_i, c_{n+i}, \cdots, c_{(k-1)n+i} \}$, i.e., $\text{p}(u_i, c_j) = 1$ for $c_j \in \mathcal{C}_i$, and 0 for $c_j \notin \mathcal{C}_i$. Let $E = \emptyset$, and $\tau(u,v,c)$ thereby is 0 for all $(u,v,c)$. In the optimal solution of the \group\ approach, each slot $s$ contributes at most $1-\lambda$ to the total \scenario\ utility because every item is preferred by exactly one user. By contrast, the optimal solution in \prob\ recommends $u_i$ all the $k$ items in $\mathcal{C}_i$. Each $u_i$ then contributes $k(1-\lambda)$ to the total \scenario\ utility, and thus $\frac{\text{OPT}(\mathbf{I}_G)}{\text{OPT}_{\text{G}}(\mathbf{I}_G)} = \frac{nk(1-\lambda)}{k(1-\lambda)} = n$. 

\sloppy For $\mathbf{I}_\text{P}$, each user $u_i$ in $\mathbf{I}_\text{P}$ prefers the items in $\mathcal{C}_i$ only \textit{slightly more than} all the other items. Specifically, let $\text{p}(u_i, c_j) = 1$ for $c_j \in \mathcal{C}_i$, and $\text{p}(u_i, c_j) = 1 - \epsilon$ for $c_j \notin \mathcal{C}_i$. Let $G$ represent a complete graph here, and $\tau(u,v,c) = 1$ for all $u,v$ and $c$. The optimal solution of the \personalized\ approach selects all the $k$ items in $\mathcal{C}_i$ for each $u_i$ and contributes $(1-\lambda) \cdot n \cdot k$ to the total \scenario\ utility. Note that co-display is not facilitated because no common item is chosen. By contrast, one possible solution in \prob\ recommends to all users the same $k$ items in $\mathcal{C}_1$, where each item contributes $(1-\lambda) \cdot ((1-\epsilon)n + \epsilon)$ to the total preference and $\lambda \cdot \frac{n(n-1)}{2}$ to the social utility. Thus, as $\epsilon$ approaches 0, $\frac{\text{OPT}(\mathbf{I}_P)}{\text{OPT}_{\text{P}}(\mathbf{I}_P)} \geq \frac{k[(1-\lambda) \cdot ((1-\epsilon)n + \epsilon) + \lambda \cdot \frac{n(n-1)}{2}]}{(1-\lambda) \cdot n \cdot k} \approx 1 + \frac{\lambda}{1-\lambda} \cdot \frac{n-1}{2} = O(n)$, regarding $\lambda$ as a constant.
\end{proof}
}

%============START OF THE DEFINITION OF THE ADVANCED PROBLEM IN FULL VERSION================
\subsection{Indirect Co-display and \probtwo}

\revise{In \prob, we characterize the merit of social discussions by the social utilities to a pair of users when they see the same item at the \textit{same slot}. On the other hand, if a common item is displayed at different slots in two users' VEs, a prompt discussion is more difficult to initiate since the users need to locate and move to the exact position of the item first. \textit{Teleportation} \cite{BE16}, widely used in VR tourism and gaming applications, allows VR users to directly transport between different positions in the VE. Thus, for a pair of users Alice and Bob co-displayed an item at different slots, as long as they are aware of where the item is displayed, one (or both) of them can teleport to the respective display slot of the item to trigger a remote discussion. To model this event that requires more efforts for users, we further propose a generalized notion of \textit{indirect co-display} to consider the above-described scenario.}

\revise{\begin{definition}{\textit{Indirect Co-display.} ($u \xleftrightarrow[s,s']{c} v$).} Let $u \xleftrightarrow[s,s']{c} v$ denote that users $u$ and $v$ are \textit{indirectly} co-displayed an item $c$ at slots $s$ and $s'$ respectively in their VEs, i.e., $\mathbf{A}(u,s) = \mathbf{A}(v,s') = c$. We use $u \xleftrightarrow[\text{ind}]{c} v$ to denote that there exist different slots $s \neq s'$ such that $u \xleftrightarrow[s,s']{c} v$.
\end{definition}}

\opt{full}{\noindent Note that we use $u \xleftrightarrow{c} v$ to denote \textit{direct co-display}, i.e., there exists at least one $s$ such that $u \xleftrightarrow[s]{c} v$, while using $u \xleftrightarrow[\text{ind}]{c} v$ to denote \textit{indirect co-display}. Also note that these two events are mutually exclusive due to the no-duplication constraint. Also note that $u \xleftrightarrow[s,s]{c} v$ is equivalent to direct co-display: $u \xleftrightarrow[s]{c} v$.}

\revise{As social discussions on indirectly co-displayed items are less immersive and require intentional user manipulation, we introduce a discount factor $\text{d}_{\text{tel}} < 1$ on teleportation to downgrade the social utility obtained via indirect co-display. Therefore, the total \scenario\ utility incorporating indirect co-display is as follows.}

\opt{short}{
\revise{In the full version of this paper \cite{Online}, we explicitly formulate a more generalized \probtwo\ problem with the above notions of indirect display and a modified \scenario\ utility, where the problem is associated with an additional \textit{subgroup size constraint} to accommodate practical limits in existing VR applications. Tables of all used notations in both \prob\ and \probtwo\ are also provided in the full version \cite{Online}.}
}
\opt{full}{
\begin{definition}{\textit{\scenario\ utility with indirect co-display} \label{def:savg_utility_unaligned} \newline ($\text{w'}_{\textbf{A}}(u,c)$).}
Given an \configuration\ $\textbf{A}$, the \textit{\scenario\ utility with indirect co-display} of user $u$ on item $c$ in $\textbf{A}$ is defined as
\begin{align*}
     \text{w'}_{\textbf{A}}(u,c) &= (1-\lambda)\cdot\text{p}(u,c)\\ &+ \lambda\cdot \big( \sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c) + \sum\limits_{v | u \xleftrightarrow[\text{ind}]{c} v} \text{d}_{\text{tel}} \cdot \tau(u,v,c) \big).
\end{align*}
\end{definition}

Finally, we note that existing VR applications often do not accommodate an unlimited number of users in one shared VE, e.g., VRChat \cite{VRChat} allows at most 16 users, and IrisVR \cite{IrisVR} allows up to 12 users within the same VE. Therefore, we further incorporate a \textit{subgroup size constraint} $M$ as an upper bound on the number of users directly co-displayed the same item at the same location. More specifically, for all slot $s \in [k]$, all partitioned subgroups $V^s_i \in V^s$ contain no more than $M$ users; or equivalently, given a fixed slot $s$ and a fixed item $c$, $\mathbf{A}^{\ast}(u,s) = c$ for at most $M$ different users $u$. In the following, we introduce the \probtwo\ problem that incorporates indirect co-display and the subgroup size constraint.

\vskip 0.06in
\hrule
\vskip 0.03in

\noindent \textbf{Problem: \problemtwo} (\probtwo).

\noindent \textbf{Given:} A social network $G=(V,E)$, a universal item set $\mathcal{C}$, preference utility $\text{p}(u,c)$ for all $u$ and $c$, social utility $\tau(u,v,c)$ for all $u$,$v$, and $c$, the weight $\lambda$, the number of slots $k$, the teleportation discount $\text{d}_{\text{tel}}$, and the subgroup size upper bound $M$.

\noindent \textbf{Find:} An \configuration\ $\mathbf{A}^{\ast}$ to maximize the total \scenario\ utility (with indirect co-display)
$$\sum_{u \in V} \sum_{c \in \mathbf{A}^{\ast}(u,\cdot)} \text{w'}_{\mathbf{A}^{\ast}}(u,c),$$
\noindent \sloppy such that the subgroup size constraint is satisfied, and $\text{w'}_{\mathbf{A}^{\ast}}(u,c)$ is defined as in Definition \ref{def:savg_utility_unaligned}.

\vskip 0.03in
\hrule
\vskip 0.06in

Notations in \probtwo\ are summarized in Table \ref{tab:symbols_prob2}.
}
%============END OF THE DEFINITION OF THE ADVANCED PROBLEM IN FULL VERSION================

\subsection{Hardness Result and Integer Program} \label{subsec:hardness_ip} 
In the following, we prove that \prob\ is $\mathsf{NP}$-hard and \revise{also $\mathsf{NP}$-hard to approximate within a ratio of $\frac{32}{31} - \epsilon$. }\opt{full}{We then prove that \probtwo\ does not admit any constant-factor polynomial-time approximation algorithms, unless the Exponential Time Hypothesis (ETH) fails.}

\revise{
\begin{theorem} \label{thm:new_hardness}
For any $\epsilon > 0$, it is $\mathsf{NP}$-hard to approximate \prob\ within a ratio of $\frac{32}{31} - \epsilon$.
\end{theorem}
}

\revise{
\opt{short}{
\begin{proof}
We prove the theorem with a gap-preserving reduction from the $\mathsf{MAX-E3SAT}$ problem~\cite{MAX3SAT}. Due to space constraint, please see the full version \cite{Online} for the proof.
\end{proof}
}
}
\opt{full}{
\input{proof/new_reduction.tex}
}

\opt{short}{
\revise{
\label{para:comparison_combinatorial} \para{Comparison with Related Combinatorial Problems.} Among the related \textit{Multi-Labeling} (ML)-type problems detailed in Section \ref{sec:related}, \prob\ is particularly related to the graph coloring problem MHE~\cite{homophyly}, where, different from traditional graph coloring, vertices are encouraged to share the same color with neighbors. The optimization goals of MHE is to maximize the number of \textit{happy edges}, i.e., edges with same-color vertices. Regarding the displayed items in \prob\ as colors(labels) in MHE, the social utility achieved in \prob\ is closely related to preserved number of happy edges in MHE, and \prob\ thereby encourages partitioning all users into dense subgroups to preserve the most social utility. However, \prob\ is more difficult than the ML-type problems due to the following reasons. 1) The ML-type problems find a strict partition that maps each entity/vertex to only one color(label), while \prob\ assigns $k$ items to each user, implying that any direct reduction from the above problems can only map to the $k=1$ special case in \prob. 2) Most of the ML-type problems do not discriminate among different labels, i.e., switching the assigned labels of two different subgroups will not change their objective functions. This corresponds to the special case of \prob\ where all preference utility $\text{p}(
u, c)$ and social utility $\tau(u, v, c)$ do not depend on the item $c$. 3) Most of the ML-type problems admit a partial labeling (pre-labeling) in the input such that some entities have predefined fixed labels (otherwise labeling every entity with the same label is optimal and renders the problem trivial), while \prob\ does not specify any items to be displayed to specific users. However, \prob\ requires $k$ items for each user; moreover, even in the $k=1$ special case, it is still not optimal to simply display the same item to all users in \prob\ due to the item-dependent preference and social utility.
}
}

%============APX-HARDNESS OF THE BASIC PROBLEM (OBSOLETE)================
% \begin{theorem} \label{thm:nphard}
% \prob\ is $\mathsf{NP}$-hard and $\mathsf{APX}$-hard.
% \end{theorem}

% \opt{short}{
% \begin{proof}
% \sloppy We prove the theorem with a gap-preserving reduction from the $\mathsf{APX}$-hard Maximum $\mathcal{K}_3$-packing problem (Max-K3P) \cite{packing}. Due to space constraint, please see the full version \cite{Online} for the proof.
% \end{proof}
% }

% \opt{full}{
% \begin{proof}
% We prove the theorem with a gap-preserving reduction from the maximum $\mathcal{K}_3$-packing problem (Max-K3P) \cite{packing}. Given a graph $\hat{G} = (\hat{V}, \hat{E})$, Max-K3P aims to find a subgraph $\hat{H} \subseteq \hat{G}$ with the largest number of edges such that $\hat{H}$ is a union of vertex-disjoint edges and triangles. Given a Max-K3P instance $\hat{G} = (\hat{V}, \hat{E})$, we construct an \prob\ instance as follows. Let $G = \hat{G}$. For each edge $e = (u,v) \in \hat{E}$, we construct an item $c_{e}$. Let social utility $\tau(u,v,c_e) = \tau(v,u,c_e) = 0.5$. For each triangle $\Delta$ consisting of vertices $u,v$, and $w$ in $\hat{G}$, we construct an item $c_\Delta$. Let social utility $\tau(u,v,c_\Delta) = \tau(v,u,c_\Delta) = \tau(u,w,c_\Delta) = \tau(w,u,c_\Delta) = \tau(v,w,c_\Delta) = \tau(w,v,c_\Delta) = 0.5$. Let all other social utility values be 0. Also, let preference utility $p(u,c) = 0$ for all users $u$ and items $c$. Finally, let $k= \lambda = 1$.

% We first prove the sufficient condition. Assume there exists a feasible $\hat{H} \subseteq \hat{G}$ with $x$ edges. For each disjoint edge $e = (u,v) \in \hat{H}$, let $\mathbf{A}(u,1) = \mathbf{A}(v,1) = c_{e}$ in \prob. Similarly, for each disjoint triangle $\Delta$ consisting of vertices $u,v$, and $w$ in $\hat{H}$, let $\mathbf{A}(u,1) = \mathbf{A}(v,1) = \mathbf{A}(w,1) = c_{\Delta}$. Each edge in $\hat{H}$ achieves an \scenario\ utility of 1. Therefore, this configuration achieves a total \scenario\ utility of $x$. We then prove the necessary condition. If the optimal objective in the \prob\ instance is $x$, we let $\hat{H}$ include all edges $e = (u,v)$ such that $\mathbf{A}(u,1) = \mathbf{A}(v,1) = c$ and $\tau(u,v,c) = 0.5$ (Note that $c$ could be $c_e$ or some $c_{\Delta}$). It is straightforward to verify that any connected component in $\hat{H}$ is either an edge or a triangle. As each edge in $\hat{H}$ contributes 1 to the objective in \prob, there are exactly $x$ edges in $\hat{H}$. Finally, since Max-K3P is $\mathsf{APX}$-hard \cite{packing}, \prob\ is also $\mathsf{APX}$-hard (and thus also $\mathsf{NP}$-hard). 
% \end{proof}
% }

%============$\mathsf{NP}$-HARDNESS PROOF (OBSOLETE)================
% \begin{restatable}{theorem}{nphard} \label{thm:nphard}
% \prob\ is $\mathsf{NP}$-hard.
% \end{restatable}
% % \opt{short}{
% % \begin{proof}
% % We prove the theorem with a reduction from the Minimum Dominating Set problem in \cite{Online}.
% % \end{proof}
% % }

% %\opt{full}{
% \begin{proof}
% We prove \prob\ is $\mathsf{NP}$-hard with a reduction from the Minimum Dominating Set problem (mDS). Given a graph $G_D=(V_D, E_D)$, mDS finds a subset of $V_D$ with minimum cardinality such that every other vertex not in the subset is adjacent to at least one vertex in the subset. 
% %Note that we can assume there is no isolated vertices in $G_D$, since an isolated vertex should always be included in the mDS and therefore is uninteresting. 
% For any mDS instance $G_D=(V_D, E_D)$, we build the \prob\ instance as follows. Let $V = V_D = \{ v_1, v_2, \cdots, v_n \}$. For each $(v_i, v_j) \in E_D$, we add $(v_i, v_j)$ and $(v_j, v_i)$ to $E$. Let $C=\{c_1,...,c_n\}$, and $\text{p}(v, c) = 0$ for all $v, c$. For each $(v_i, v_j) \in E$ and $c$, let $\tau(v_i, v_j, c_i)=1$ and $\tau(v_i, v_j, c_{i'})=0 \, \forall i' \neq i$. Finally let $k= \lambda = 1$.

% Below we prove that the optimal solution of this \prob\ instance corresponds to the optimal solution of the mDS instance. %Observe that item $c_i$ can only contribute to the final satisfaction of $v_i$, and no others. 
% Let $S$ denote the set of users displayed their preferred items (i.e., $v_i$ displayed $c_i$) in the optimal solution of \prob . Let $\overline{S}$ denote the set of users not in $S$ but co-displayed with some user in $S$. Therefore, 1) the total \scenario\ utility of the \prob\ solution is exactly $|\overline{S}|$, since each user $v_j \in \overline{S}$ displayed $c_i$ contributes exactly $\tau(v_i, v_j, c_i)=1$ to the social utility. 2) $V \setminus \overline{S}$ corresponds to a dominating set on $G$ because every user in $V \setminus (V \setminus \overline{S}) = \overline{S}$ is adjacent to at least one vertex in $S \subseteq (V \setminus \overline{S})$ by definition. \prob\ maximizes $|\overline{S}|$ and thereby minimizes $|V \setminus \overline{S}|$ (i.e., the size of a dominating set for mDS) simultaneously. Therefore, any polynomial-time algorithm that finds the optimal solution of \prob\ also solves mDS. The theorem follows.
% \end{proof}
% %}

%============BEGIN OF THE HARDNESS OF THE ADVANCED PROBLEM IN FULL VERSION================
\opt{full}{
We then prove the hardness of approximation for the advanced \probtwo\ problem.

\begin{theorem} \label{thm:veryhard}
There exists no polynomial-time algorithm that approximates \probtwo\ within any constant factor, unless the exponential time hypothesis (ETH) fails.
\end{theorem}

\begin{proof}
We prove the theorem with a gap-preserving reduction from the Densest k-Subgraph problem (DkS) \cite{eth}. Given a graph $\hat{G} = (\hat{V}, \hat{E})$, DkS aims to find a subgraph $\hat{H} \subseteq \hat{G}$ with $\hat{k}$ vertices with the largest number of induced edges. (Note that for a fixed $\hat{k}$, maximizing the density is equivalent to maximizing the number of edges. We use $\hat{k}$ instead of the conventional $k$ to avoid confusion with the number of slots in \probtwo.) Given a DkS instance $\hat{G} = (\hat{V}, \hat{E})$ and $\hat{k}$, we construct an \prob\ instance as follows. Let $V = \hat{V} \cup S$, where $S = \{w_1, w_2, \cdots, w_{|S|} \}$ consists of $|S| = \hat{k} - (|\hat{V}|$ mod $\hat{k})$ additional vertices if $\hat{k} \nmid |\hat{V}|$, and $S = \emptyset$ if $\hat{k} \mid |\hat{V}|$. Let $E = \hat{E}$. Therefore, all vertices in $S$ are singletons. Let $\mathcal{C} = \{c_1, c_2, \cdots, c_m\}$, where $m = \frac{|V|}{\hat{k}}$. Let preference utility $p(u,c) = 0$ for all $u \in V$ and $c \in \mathcal{C}$. For each edge $e = (u,v) \in \hat{E}$, let $\tau(u,v,c_1) = \tau(v,u,c_1) = 0.5$. Let $\tau(u,v,c) = 0$ for all $(u,v) \notin \hat{E}$ or $c \neq c_1$. Finally, let $k=1$, $\lambda = 1$, and $M = \hat{k}$.

We first prove the sufficient condition. Assume that there exists a subgraph $\hat{H} \subseteq \hat{G}$ with $\hat{k}$ vertices and $x$ edges. We construct an \probtwo\ solution with objective $x$ by co-displaying $c_1$ to all vertices in $\hat{H}$ (and thereby obtaining social utility of 1 on each edge) and then randomly partitioning the vertices not in $\hat{H}$ to $m-1$ sets of cardinality $\hat{k}$. We then prove the necessary condition. Since there are $m = \frac{|V|}{\hat{k}}$ items, and the subgroup size constraint is $M = \hat{k}$, it follows that each item is co-displayed to exactly $M = \hat{k}$ users in a feasible solution. Assume the optimal objective in the \probtwo\ instance is $x$, then the $M = \hat{k}$ users co-displayed item $c_1$ collectively form a induced subgraph of exactly $x$ edges. Let $\hat{H}$ be the induced subgraph formed by these vertices in $\hat{G}$, then $\hat{H}$ has exactly $x$ edges. Finally, according to \cite{eth}, assuming the exponential time hypothesis (ETH) holds, there is no polynomial-time algorithm that approximates DkS to within a constant factor; in fact, a stronger inapproximability of $n^{(1/ \log \log n)^c}$ holds. The result for \probtwo\ directly follows.
\end{proof}

Here we further point out that both the hardness results of \prob\ and \probtwo\ are from a simple case where $k=1$, i.e., the considered problems are already very hard when only one display slot is in consideration. Therefore, the hardness of \prob\ and \probtwo\ with general values of $k$ may be even harder. We revisit this issue in Section \ref{subsec:combinatorial}.
}
%============END OF THE HARDNESS OF THE ADVANCED PROBLEM IN FULL VERSION================

%============BEGIN OF THE IP OF THE BASIC PROBLEM================
Next, we propose an Integer Programming (IP) model for \prob\ \opt{full}{and \probtwo\ }to serve as the cornerstone for the approximation algorithm proposed later in Section \ref{sec:algo}.\opt{full}{ We begin with the IP for \prob.} Let binary variable $x^c_{u,s}$ denote whether user $u$ is displayed item $c$ at slot $s$, i.e., $x^c_{u,s} = 1$ if and only if $\mathbf{A}(u,s) = c$. Let $x^c_u$ indicate whether $u$ is displayed $c$ at any slot in the \configuration. Moreover, for each pair of friends $e = (u,v) \in E$, let binary variable $y^c_{e,s}$ denote whether $u$ and $v$ are co-displayed item $c$ at slot $s$, i.e., $y^c_{e,s} = 1$ if and only if $u \xleftrightarrow[s]{c} v$. Similarly, variable $y^c_{e} = 1$ if and only if $u \xleftrightarrow{c} v$. The objective of \prob\ is specified as follows.

$$ \text{max} \sum\limits_{u \in V} \sum\limits_{c \in \mathcal{C}} [ (1-\lambda) \cdot \text{p}(u, c) \cdot x^c_u + \lambda \cdot \sum\limits_{e = (u,v) \in E} ( \tau(u,v,c) \cdot y^c_e) ] $$

\noindent subject to the following constraints,
\small
\begin{align}
    \sum_{s=1}^{k} x^c_{u,s} \leq 1, \quad & \forall u \in V, c \in \mathcal{C} \label{ilp:no_replicated_item}\\
    \sum_{c \in \mathcal{C}} x^c_{u,s} = 1, \quad & \forall u \in V, s \in [k] \label{ilp:one_slot_one_item}\\
    x^c_u = \sum_{s=1}^{k} x^c_{u,s}, \quad & \forall u \in V, c \in \mathcal{C} \label{ilp:user_recommended}\\
    y^c_{e} = \sum_{s=1}^{k} y^c_{e,s}, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \label{ilp:edge_recommended}\\
    y^c_{e,s} \leq x^c_{u,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \label{ilp:direct_relation_1} \\
    y^c_{e,s} \leq x^c_{v,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \label{ilp:direct_relation_2} \\
    x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e \in \{ 0,1 \}, \quad & \forall u \in V, e \in E, s \in [k], c \in \mathcal{C} \label{ilp:integrality}.
\end{align}

\normalsize
Constraint \ref{ilp:no_replicated_item} states that each item $c$ can only be displayed at most once to a user $u$ (i.e., the no-duplication constraint). Constraint \ref{ilp:one_slot_one_item} guarantees that each user $u$ is displayed exactly one item at each slot $s$. Constraint \ref{ilp:user_recommended} ensures that $x^c_u = 1$ ($u$ is displayed $c$ in the configuration) if and only if there is exactly one slot $s$ with $x^c_{u,s} = 1$. Similarly, constraint \ref{ilp:edge_recommended} ensures $y^c_{e} = 1$ if and only if $y^c_{e,s} =1 $ for exactly one $s$. Constraints \ref{ilp:direct_relation_1} and \ref{ilp:direct_relation_2} specify the co-display, where $y^c_{e,s}$ is allowed to be $1$ only if $c$ is displayed to both $u$ and $v$ at slot $s$, i.e., $x^c_{u,s} = x^c_{v,s} = 1$. Finally, constraint \ref{ilp:integrality} ensures all decision variables are binary. \revise{Note that the $x$ variables in the IP model are sufficient to represent the solution of \prob\ (i.e., $x^c_{u,s}$ denotes whether an item $c$ is displayed at slot $s$ for user $u$), whereas the $y$ variables are auxiliary to enable \prob\ to be formulated as an IP. Without incorporating the $y$ variables, the formulation will become nonlinear.}

\opt{short}{In \cite{Online}, we also prove that \probtwo\ admits no constant-ratio polynomial-time approximation algorithms unless the Exponential Time Hypothesis fails, 
 and propose an IP model for \probtwo.}

%============END OF THE IP OF THE BASIC PROBLEM================

%============BEGIN OF THE IP OF THE ADVANCED PROBLEM IN THE FULL VERSION================
\opt{full}{
Next, for each $e = (u,v) \in E$, let binary variable $z^c_e$ denote whether $u$ and $v$ are co-displayed (both directed \textit{or} indirected) item $c$. Note that $y^c_{e} = 1$ implies $z^c_{e} = 1$. To avoid repetitive calculation of the social utility, the coefficient before $y^c_{e}$ in the objective is modified to be $(1-\text{d}_{\text{tel}})$, such that a social utility of $\tau(u,v,c)$ is obtained when $y^c_{e} = z^c_{e} = 1$. The objective of \probtwo\ is thus

\begin{align*} \text{max} \sum\limits_{u \in V} \sum\limits_{c \in \mathcal{C}} &[ (1-\lambda) \cdot \text{p}(u, c) \cdot x^c_u + \lambda \cdot \sum\limits_{e = (u,v) \in E} \tau(u,v,c) \\ &\cdot \big( (1-\text{d}_{\text{tel}}) \cdot y^c_e + \text{d}_{\text{tel}} \cdot z^c_e \big) ] 
\end{align*}

\noindent subject to constraints \ref{ilp:no_replicated_item} to \ref{ilp:direct_relation_2} above, as well as the following constraints:
\small
\begin{align}
    z^c_{e} \leq x^c_u, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \label{ilp2:indirect_relation_1} \\
    z^c_{e} \leq x^c_v, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \label{ilp2:indirect_relation_2} \\
    x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e, z^c_e \in \{ 0,1 \}, \quad & \forall u \in V, e \in E, s \in [k], c \in \mathcal{C} \label{ilp2:integrality}.
\end{align}

\normalsize
Constraints \ref{ilp2:indirect_relation_1} and \ref{ilp2:indirect_relation_2} specify the co-display, where $z^c_{e}$ is allowed to be $1$ only if $c$ is displayed to $u$ and $v$ in some (not necessarily the same) slots, i.e., $x^c_u = x^c_v = 1$. Therefore, $y^c_{e} = z^c_{e} = 1$ for the case of direct co-display. Constraint \ref{ilp2:integrality} is the integrality constraint. The other constraints follow from the basic \prob\ problem. Note that in the optimal solution, whenever $y^c_{e} = 1$ for some edge $e$, the corresponding $z^c_{e}$ will also naturally equal $1$, as it is always better to have a larger $z^c_{e}$. Therefore, no additional constraint needs to be introduced to enforce this relation. Note that, similar to that in the IP for \prob, the $y$ and $z$ variables are auxiliary variables to enable linearity in this IP.
}
%============END OF THE IP OF THE ADVANCED PROBLEM IN THE FULL VERSION================

\opt{full}{
\subsection{Related Combinatorial Problems} \label{subsec:combinatorial}

\begin{table*}[t]
\begin{small}
\caption{Related Combinatorial Problems (approximation ratio for MAX problems inversed).}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Problem\\ Name\end{tabular} & Abbrev. & Prelabeling & Type & Objective & \begin{tabular}[c]{@{}l@{}}Hardness\\ Result\end{tabular} & \begin{tabular}[c]{@{}l@{}}Approx.\\ Result\end{tabular} & \begin{tabular}[c]{@{}l@{}}Is special\\ case of\end{tabular} & \begin{tabular}[c]{@{}l@{}}Is comple-\\ ment of\end{tabular} \\ \hline \hline
\begin{tabular}[c]{@{}l@{}}Submodular\\ Multi-Labeling \cite{multilabeling} \end{tabular} & Sub-ML & General & MIN & \begin{tabular}[c]{@{}l@{}}submodular\\ set function\end{tabular} & \begin{tabular}[c]{@{}l@{}}$2-\frac{2}{m}-\epsilon$\\ (UGC) \cite{multilabeling} \end{tabular}  & $2-\frac{2}{m}$ \cite{multilabeling} &  & Sup-ML \\ \hline
\begin{tabular}[c]{@{}l@{}}Supermodular\\ Multi-Labeling \cite{multilabeling} \end{tabular} & Sup-ML & General & MAX & \begin{tabular}[c]{@{}l@{}}supermodular\\ set function\end{tabular} & $\mathsf{NP}$-hard & $\frac{m}{2}$ \cite{multilabeling}  &  & Sub-ML \\ \hline
\begin{tabular}[c]{@{}l@{}}Submodular\\ Multiway Partition \cite{multiwaypartition} \end{tabular} & Sub-MP & $m$ terminals & MIN & \begin{tabular}[c]{@{}l@{}}submodular\\ set function\end{tabular} &  \begin{tabular}[c]{@{}l@{}}$2-\frac{2}{m}-\epsilon$\\ ($\mathsf{NP}=\mathsf{RP}$) \cite{mp13soda} \end{tabular} & $2-\frac{2}{m}$ \cite{mp13soda} & Sub-ML & Sup-MP \\ \hline
\begin{tabular}[c]{@{}l@{}}Supermodular\\ Multiway Partition \cite{multilabeling} \end{tabular} & Sup-MP & $m$ terminals & MAX & \begin{tabular}[c]{@{}l@{}}supermodular\\ set function\end{tabular} & $\mathsf{NP}$-hard &  & Sup-ML & Sub-MP \\ \hline
\begin{tabular}[c]{@{}l@{}}Maximum\\ Happy Vertices \cite{homophyly} \end{tabular} & MHV & General & MAX & \begin{tabular}[c]{@{}l@{}}\# happy\\ vertices\end{tabular} & $\mathsf{NP}$-hard & $\frac{m}{2}$ \cite{multilabeling} & Sup-ML & MUHV \\ \hline
\begin{tabular}[c]{@{}l@{}}Minimum\\ Unhappy Vertices \cite{multilabeling} \end{tabular} & MUHV & General & MIN & \begin{tabular}[c]{@{}l@{}}\# unhappy\\ vertices\end{tabular} & \begin{tabular}[c]{@{}l@{}}$2-\frac{2}{m}-\epsilon$\\ (UGC) \cite{multilabeling} \end{tabular}  & $2-\frac{2}{m}$ \cite{multilabeling} & Sub-ML & MHV \\ \hline
\begin{tabular}[c]{@{}l@{}}Maximum\\ Happy Edges \cite{homophyly} \end{tabular} & MHE & General & MAX & \begin{tabular}[c]{@{}l@{}}\# happy\\ edges\end{tabular} & $\mathsf{NP}$-hard & 1.1716 \cite{mhe} & Sup-ML &  \\ \hline
\multicolumn{2}{|l|}{Multiway Cut \cite{multiwaycut}} & $m$ terminals & MIN & \begin{tabular}[c]{@{}l@{}}\# edges\\ removed\end{tabular} & $\frac{8}{7}$ \cite{sdp} & 1.2965 \cite{multiwaycutapprox} & UML & \begin{tabular}[c]{@{}l@{}}Multiway\\ Uncut\end{tabular} \\ \hline
%\multicolumn{2}{|l|}{Weighted Multiway Cut} & $m$ terminals & MIN & \begin{tabular}[c]{@{}l@{}}\# edge weight\\ removed\end{tabular} & \begin{tabular}[c]{@{}l@{}}$2-\frac{2}{m}-\epsilon$\\ (UGC) \cite{mp13soda} \end{tabular}  & $2-\frac{2}{m}$ \cite{mp13soda} & Sub-MP &  \\ \hline
\multicolumn{2}{|l|}{Multiway Uncut \cite{multiwayuncut}} & $m$ terminals & MAX & \begin{tabular}[c]{@{}l@{}}\# edges\\ preserved\end{tabular} &$\mathsf{NP}$-hard  & 1.1716 \cite{multiwayuncut} & MHE & \begin{tabular}[c]{@{}l@{}}Multiway\\ Cut\end{tabular} \\ \hline \hline
%\multicolumn{2}{|l|}{0-Extension \cite{0extension}} & $m$ terminals & MIN & \begin{tabular}[c]{@{}l@{}}\# total cost\\ of edges\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\Omega((\log m)^\frac{1}{2})$\\ (UGC) \cite{sdp} \end{tabular} &  &  & \\ \hline
\begin{tabular}[c]{@{}l@{}}Uniform Metric\\ Labeling \cite{JK02} \end{tabular} & UML & $m$ terminals & MIN & \begin{tabular}[c]{@{}l@{}}\# total cost of\\edges/vertices\end{tabular} & \begin{tabular}[c]{@{}l@{}}$2-\frac{2}{m}$\\ (UGC) \cite{sdp} \end{tabular} & $2$ \cite{JK02} & \begin{tabular}[c]{@{}l@{}}Metric\\ Labeling\end{tabular} & \\ \hline
\end{tabular}
\label{tab:theory}
\end{center}
\end{small}
\end{table*}
}

\prob\ is related to the \textit{Multi-Labeling} (ML) \cite{multilabeling} problem and its variations, including {Multiway Partition} \cite{multilabeling, multiwaypartition}, \textit{Maximum Happy Vertices/Edges} (MHV/MHE) \cite{homophyly}, and \textit{Multiway Cut} \cite{multiwaycut} in graphs. In the Multi-Labeling (ML) problem, the general inputs are a ground set of entities $V$, a set of labels $L = \{1, 2, \cdots, m\}$, and a \textit{partial} labeling function $\ell : V \mapsto L$ that pre-assigns each label $i$ to a non-empty subset $T_i \subseteq V$, and a set function $f: 2^V \mapsto \mathcal{R}$. The goal of ML is to partition the ground set into $m$ subsets to optimize the aggregated set function on the partitioned subsets, i.e., $\sum\limits_{i=1}^{m} f(T_i)$. The special cases with set function $f$ being submodular or supermodular is called \textit{Submodular Multi-Labeling} (Sub-ML) and \textit{Supermodular Multi-Labeling} (Sup-ML) \cite{multilabeling}. Other work \cite{multiwaypartition} studies the case where the partial labeling function is required to assign a label $i$ to only one entity $v_i$. The above problems become \textit{Submodular Multiway Partition} (Sub-MP) and \textit{Supermodular Multiway Partition} (Sup-MP) in this context. Some special cases of Sub-ML and Sup-ML are described as graph problems, where the ground set $V$ is the vertex set on a graph $G = (V,E)$. In this context, the above assumption on $f$ in Sub-MP and Sup-MP can be interpreted as $m$ specified terminals on the graph. Two representative special cases are the \textit{Maximum Happy Vertices} (MHV) problem and the \textit{Maximum Happy Edges} (MHE) problem \etal \cite{homophyly}. Originally proposed to study homophyly effects in networks, MHV and MHE are described as coloring problems where, different from traditional graph coloring, vertices are encouraged to share the same color with neighbors. \textit{Edges with same-color vertices} and \textit{vertices sharing the same color with all neighbors} are characterized as \textit{happy edges} and \textit{happy vertices}, respectively. The optimization goals of MHV and MHE are thus to maximize the number of happy vertices and edges. The complement problem of MHV, \textit{Minimum Unhappy Vertices} (MUHV) \cite{multilabeling}, minimizes the number of unhappy vertices. When the above optimization goal of MHE is combined with the assumption of $m$ terminals, the resulted problem becomes the \textit{Multiway Uncut} problem \cite{multiwayuncut}, which is the complement of the classical and extensively studied \textit{Multiway Cut} problem \cite{multiwaycut}. The Multiway Cut problem asks for the minimum number of edges removed to partition a graph into $m$ subgraph, each containing one terminal. The Metric Labeling problem \cite{JK02} is a generalization of Multiway Cut considering edge weights and also a cost function on labeling the vertices. We summarize the problem characteristics, hardness results, currently best algorithmic results, and their interdependency in Table \ref{tab:theory}. All the problems are $\mathsf{NP}$-hard, while more advanced inapproximability results, relying on other complexity conjectures, are stated for some problems. Note that the approximation ratios for maximization problems are shown as inverses (i.e., values larger than 1) for better comparison and consistency with this paper.

Among the ML-type problems, \prob\ is particularly correlated to the MHE problem. Regarding the displayed items in \prob\ as colors(labels) in MHE, the social utility achieved in \prob\ is closely related to preserved number of happy edges in MHE, and \prob\ thereby encourages partitioning all users into dense subgroups to preserve the most social utility. However, \prob\ is more difficult than the above ML-type problems due to the following reasons. 1) The ML-type problems find a strict partition that maps each entity/vertex to only one color(label), while \prob\ assigns $k$ items to each user, implying that any direct reduction from the above problems can only map to the $k=1$ special case in \prob, where \algo\ can achieve a 2-approximation. 
2) The above problems do not discriminate among different labels, i.e., switching the assigned labels of two different subgroups will not change their objective functions. This corresponds to the special case of \prob\ where all preference utility $\text{p}(u, c)$ and social utility $\tau(u, v, c)$ do not depend on the item $c$.\opt{fullrevise}{ In contrast, \prob\ captures the item preferences as both utility measures in \prob\ depend on the item identity.}
3) The above problems admit a partial labeling (pre-labeling) in the input such that some entities have predefined fixed labels (otherwise labeling every entity with the same label is optimal and renders the problem trivial), while \prob\ does not specify any items to be displayed to specific users. However, \prob\ requires $k$ items for each user; moreover, even in the $k=1$ special case, it is still not optimal to simply display the same item to all users in \prob\ due to the item-dependent preference and social utility.

Finally, we note that while most of the minimization problems admit stronger hardness results than conventional $\mathsf{NP}$-hardness, no such type of results are known for all maximization problems above. As \prob\ is also a maximization problem, its hardness does not directly follow from any complementary minimization problems. Interestingly, the algorithmic aspect of all these problems share an obvious trend: almost all approximation results here, including our algorithm for \prob, utilizes some kind of (dependent) randomized rounding on some formulation of relaxed problem (not limited to linear relaxation). In this regard, this paper extends the scheme beyond labeling problems to the \prob\ problem that assigns a $k$-itemset to each user, which has an even more complicated combinatorial nature.

==> stash/sec4_algo.tex <==
\section{Algorithm Design}\label{sec:algo}

\opt{full}{
\begin{table}[t!]
\caption{Notations used in \algo.}
\begin{center}
\begin{tabular}{|c|l|}\hline
Symbol & Description \\\hline\hline
$X^\ast$ & optimal \fragsol\ \\\hline
${x^\ast}^c_{u,s}$ & optimal decision variable \\\hline
$(c,s,\alpha)$ & set of focal parameters \\\hline
$c/\hat{c}$ & \roundingitem\ \\\hline
$s/\hat{s}$ & \roundingslot\ \\\hline
$u/\hat{u}$ & current user/eligible user\\\hline
$\alpha$ & \roundingalpha\ \\\hline
$U$ & target subgroup \\\hline
$\text{OPT}$ & optimal \scenario\ utility \\\hline
$\mathcal{R}$ & achieved utility \\\hline
$\mathcal{R}_{\text{per}}$ & achieved preference utility \\\hline
$\mathcal{R}_{\text{soc}}$ & achieved social utility \\\hline
$S_{\text{cur}}$ & available display units \\\hline
$S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})$ & display units to be filled \\\hline
$S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})$ & display units not to be filled \\\hline
${\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s}))$ & \scenario\ utility gained by \stagethree\ \\\hline
${\text{OPT}}_{\text{LP}}(S_{\text{fut}}(c,s,{x^\ast}^c_{u,s}))$ & expected future \scenario\ utility \\\hline
$\text{w}^c_e$ & $\tau(\hat{u},\hat{v},c)+\tau(\hat{v},\hat{u},c)$\\\hline
$r$ & balancing ratio \\\hline
\end{tabular}
\label{tab:symbols_algo}
\end{center}
\end{table}
}

In this section, we introduce the \algofull\ (\algo) algorithm to tackle \prob. As shown in Example \ref{example:illustrative}, the \personalized\ and \group\ approaches do not solve \prob\ effectively, as the former misses on social utility from co-display while the latter fails to leverage the flexibility of \notion\ to preserve personal preference. An alternative idea, called the \textit{subgroup} approach, is to first pre-partition the shopping group (i.e., the whole user set) into some smaller social-aware subgroups (e.g., using traditional community detection techniques), and then determine the displayed items based on preferences of the subgroups. While this idea is effective for social event organization \cite{XW18WWW} where each user is assigned to exactly one social activity, it renders the partitioning of subgroups static across all display slots in \prob, i.e., a user is always co-displayed common items only with other users in the same subgroup. Therefore, this approach does not fully exploit the \notion\ flexibility, leaving some room for better results.

Instead of using a universal partition of subgroups as in the aforementioned subgroup approach, we aim to devise a more sophisticated approach that allows varied co-display subgroups across the display slots to maximize the user experience. Accordingly, we leverage Linear Programming (LP) relaxation strategies that build on the solution of the Integer Program formulated in Section \ref{subsec:hardness_ip} because it naturally facilitates different subgroup partitions across all slots while allocating proper items for those subgroups with CID. In other words, our framework partitions the subgroups (for each slot) and selects the items simultaneously, thus avoiding any possible shortcomings of two-phased approaches that finish these two tasks sequentially. By relaxing all the integrality constraints in the IP, we obtain a relaxed linear program whose \textit{fractional} optimal solution can be explicitly solved in polynomial time. For an item $c$ to be displayed to a user $u$ at a certain slot $s$, the fractional decision variable ${x^\ast}^c_{u,s}$ obtained from the optimal solution of the LP relaxation problem can be assigned as its \emph{\weight}. Items with larger \weight s\ are thus inclined to contribute more \scenario\ utility (i.e., the objective value), since they are preferred by the users or more capable of triggering social interactions.

Next, it is important to design an effective rounding procedure to construct a promising \configuration\ according to the \weight s. We observe that simple \textit{independent} rounding schemes may perform egregiously in \prob\ because they do not facilitate effective co-displaying of common items, thereby losing a huge amount of potential social utility upon constructing the \configuration, especially in the cases where the item preferences are not diverse. Indeed, we prove that independent rounding schemes may achieve an expected total objective of only $O(1/m)$ of the optimal amount. Motivated by the incompetence of independent rounding, our idea is to leverage \textit{dependent rounding} schemes that encourage co-display of items of common interests, i.e., with high \weight s to multiple users in the optimal LP solution. 

Based on the idea of dependent rounding schemes in \cite{JK02}, we introduce the idea of \textit{\stagethreefull} (\stagethree) that co-displays a \textit{\roundingitem} $c$ at a specific \textit{\roundingslot} $s$ to every user $u$ with a \weight\ $x^c_{u,s}$ greater than a \textit{\roundingalpha} $\alpha$. In other words, \stagethree\ clusters the users with high  \weight s to a \roundingitem\ $c$ to form a \textit{target subgroup} in order to co-display $c$ to the subgroup at a specific display slot $s$. Depending on the randomly chosen set of \textit{focal parameters}, including the \roundingitem, the \roundingslot, and the \roundingalpha, the size of the created target subgroups can span a wide spectrum, i.e., as small as a single user and as large as the whole user set $V$, to effectively avoid the pitfalls of \personalized\ and \group\ approaches. The randomness naturally makes the algorithm less vulnerable to extreme-case inputs, therefore resulting in a good approximation guarantee. Moreover, \stagethree\ allows the partitions of subgroups to vary across all slots in the returned \configuration, exploiting the flexibility provided by \notion. However, different from the dependent rounding schemes in \cite{JK02}, the construction of \configuration s in \prob\ faces an additional challenge -- it is necessary to carefully choose the displayed items at multiple slots to ensure the no-duplication constraint. %Moreover, the sizes of partitioned VR subgroups need to be monitored in the advanced \probtwo\ problem due to practical VR concerns\opt{short}{ (detailed in the full version\cite{Online})}. 

We prove that \algo\ is a 4-approximation algorithm for \prob\ and also show that \algo\ can be fully derandomized into a deterministic approximation algorithm. \opt{full}{We also tailor \stagethree\ to consider the size constraint so as to extend \algo\ for the more complicated \probtwo. }
In the following, we first deal with the case with $\lambda = \frac{1}{2}$. We observe that all other cases with $\lambda \neq 0$ can be reduced to this case by proper scaling of the inputs, i.e., $\text{p'}(u,c) = \frac{1-\lambda}{\lambda}\text{p}(u,c)$, whereas $\lambda = 0$ makes the problem become trivial. \opt{short}{We explicitly prove this property in Section \ref{subsec:enhancements} in the full version \cite{Online}.}\opt{full}{We explicitly prove this property in Section \ref{subsec:enhancements}.} Moreover, for brevity, the total \scenario\ utility is scaled up by 2 so that it is a direct sum of the preference and social utility. \opt{short}{A table of all notations used in \algo\ is also provided in \cite{Online}.}\opt{full}{All used notations in \algo\ are summarized in Table \ref{tab:symbols_algo}.}

\subsection{LP Relaxation and an Independent Rounding Scheme} \label{subsec:independent}

\revise{Following the standard linear relaxation technique \cite{approxalg}, the LP relaxation problem of \prob\ is formulated by replacing the integrality constraint (constraint \ref{ilp:integrality}) in the IP model, i.e., $ x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e \in \{ 0,1 \}$, with linear upper/lower bound constraints, i.e., $0 \leq  x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e \leq 1$. The optimal \fragsol\ of the relaxed problem can be acquired in polynomial time with commercial solvers, e.g., CPLEX \cite{CPLEX} or Gurobi \cite{Gurobi}. Recall that the $x$-variables are sufficient to represent the solution of \prob\ (i.e., $x^c_{u,s}$ denotes whether an item $c$ is displayed at slot $s$ for user $u$), whereas the $y$-variables are auxiliary. Therefore, the optimal solution can be fully represented by $X^\ast$ (the set of optimal $x$ variables).} The fractional decision variable ${x^\ast}^c_{u,s}$ in $X^\ast$ is then taken as the \textit{\weight} of item $c$ at slot $s$ for user $u$. Note that the optimal objective in the relaxed LP is an upper bound of the optimal total \scenario\ utility in \prob, because the optimal solution in \prob\ is guaranteed to be a feasible solution of the LP relaxation problem.

\small
\begin{table}[t]
	\centering
	\caption{Optimal \fragsol\ for slot 1 in Example \ref{example:running}.}
	\label{table:fragsol}
	\begin{tabular}{l|ccccc}
  &  ${x^\ast}^{c_1}_{\cdot,1}$ & ${x^\ast}^{c_2}_{\cdot,1}$ & ${x^\ast}^{c_3}_{\cdot,1}$ & ${x^\ast}^{c_4}_{\cdot,1}$ & ${x^\ast}^{c_5}_{\cdot,1}$ \\ \hline 
 $u_A$ &  $0.33$  & $0.33$  &  $0$    &  $0$    &  $0.33$ \\
 $u_B$ &  $0.33$  & $0.33$  &  $0$    &  $0.33$ &  $0$    \\
 $u_C$ &  $0$     & $0$     & $0.33$  &  $0.33$ &  $0.33$ \\
 $u_D$ &  $0.33$  & $0$     & $0$     &  $0.33$ &  $0.33$ \\
	\end{tabular}
\end{table}
\normalsize

\begin{example} \label{example:lp_relax}
Table \ref{table:fragsol} shows the \weight s in Example \ref{example:running}, where the \fragsol\ is identical for all slots 1-3 (thereby only slot 1 is shown). For example, the \weight\ of $c_1$ (the tripod) to Alice at each slot is ${x^\ast}^{c_1}_{u,1} = {x^\ast}^{c_1}_{u,2} = {x^\ast}^{c_1}_{u,3} = 0.33$. %Therefore, the utility factor of $c_1$ (the tripod) to Alice at slot 1 is 0.33.
\end{example}

Note that three items ($c_1, c_2$, and $c_5$) have nonzero \weight s to Alice at slot 1 in Example \ref{example:lp_relax}, which manifests that the optimal LP solution may not construct a valid \configuration\ because each user is allowed to display exactly one item at each display slot in \prob. Therefore, a rounding scheme is needed to construct appropriate \configuration s from the \weight s. Given $X^\ast$, a simple rounding scheme is to randomly (and independently) assign item $c$ to user $u$ at slot $s$ with probability ${x^\ast}^c_{u,s}$, i.e., the \weight\ of $c$ to $u$ at $s$, so that more favorable items are more inclined to be actually displayed to the users. \opt{full}{This rounding scheme is summarized in Algorithm \ref{alg:trivial_rounding}. 

\input{algo/trivial_rounding.tex}}

However, as this strategy selects the displayed items independently, for a pair of friends $u$ and $v$, the chance that the algorithm obtains high social utility by facilitating co-display is small, since it requires the randomized rounding process to hit on the same item for both $u$ and $v$ simultaneously. Furthermore, this strategy could not ensure the final \configuration\ to follow the no-duplication constraint, as an item $c$ can be displayed to a user $u$ at any slot with a nonzero \weight. The following lemma demonstrates the ineffectiveness of this rounding scheme.

\begin{lemma} \label{lemma:trivial_rounding}
There exists an \prob\ instance $I$ on which the above rounding scheme achieves only a total \scenario\ utility of $O(\frac{1}{m})$ of the optimal value in expectation.
\end{lemma}

\opt{short}{
\begin{proof}
Due to space constraints, please see Section \ref{subsec:independent} in the full version \cite{Online} for the proof.
\end{proof}
}
\opt{full}{
\begin{proof}
Assume that for all users $u,v \in V$ and $c \in \mathcal{C}$, we have $\text{p}(u,c) = 0$ and $\tau(u,v,c) = \tau$ for a constant $\tau > 0$. Intuitively, every user is indifferent among all items. In this case, a trivial optimal solution for the relaxed LP can be found by setting ${x^\ast}^c_{u,s} = \frac{1}{m}$ for all $c,u,s$. As the trivial rounding scheme determines the displayed items independently, for any pair of users $u,v$ and any slot $s$, the probability that $u$ and $v$ are co-displayed any item at slot $s$ is only $\frac{1}{m}$. Therefore, the expected total \scenario\ utility achieved is $\frac{n(n-1)}{m} \cdot \tau \cdot k$. On the other hand, co-displaying an arbitrary item to all users achieves a social utility of $n(n-1) \cdot \tau$, and repeating this with distinct items for all slots yields a total \scenario\ utility of $n(n-1) \cdot \tau \cdot k$. This independent rounding scheme thus achieves only $\frac{(n-1)\tau}{m(n-1)\tau} = O(\frac{1}{m})$ of the optimal value. Moreover, the resulting \configuration\ is highly unlikely to satisfy the no-duplication constraint.
\end{proof}
}

\subsection{Alignment-aware Algorithm} \label{subsec:details}

To address the above issues, %our idea is to leverage the dependent rounding schemes for labeling problems in \cite{JK02} to 
we devise the \textit{\stagethreefull} (\stagethree) rounding scheme, inspired by the dependent rounding scheme for labeling problems \cite{JK02}, as the cornerstone of \algo\ to find a target subgroup $U$ according to a set of focal parameters for co-display of the \roundingitem\ to all users in $U$. Given the optimal \fragsol\ $X^\ast$ to the LP relaxation problem, \algo\ iteratively 1) samples a set of focal parameters $(c,s,\alpha)$ with $c \in \mathcal{C}, s \in \{1, 2, \cdots, k\}$, and $\alpha \in [0,1]$ uniformly at random; it then 2) conducts \stagethree\ according to the selected set of parameters $(c,s,\alpha)$ until a complete \configuration\ is constructed. It is summarized in Algorithm \ref{alg:alignment_aware_rounding}.

\input{algo/algo.tex}

%===============RPS AND DPS (OBSOLETE; KDD/ICDE VERSION OF TWO PARAMETER SELECTION SCHEMES)===============
%We propose two strategies: RFS and \algod\. RFS is a simple and efficient \textit{randomized} strategy to sample $(c,s,\alpha)$ uniformly from all combinations, i.e., selecting $c \in \mathcal{C}, s \in 1,2,\cdots, k$, and $\alpha \in [0,1]$ uniformly at random. Nevertheless, RFS is only able to guarantee the \textit{expected \scenario\ utility} of the randomly generated solution. To further provide a worst-case performance bound, we propose a more sophisticated \textit{deterministic} strategy, \algod\, in Section \ref{subsec:derandomize} to carefully choose a favorable $(c,s,\alpha)$ by simultaneously maximizing the increment in the current \scenario\ utility and the expected \scenario\  utility acquired at the remaining slots. Note that \algod\ does not always outperform RFS since RFS embraces the power of \emph{randomness} to explore various possible solutions. Nevertheless, evaluation in Section \ref{sec:exp} manifests that \algod\ is better than RFS on average due to the joint optimization on the current and future allocations. 

\para{\stagethreefull.} Given the randomly sampled set of parameters $(c,s,\alpha)$, \stagethree\ finds the target subgroup as follows. With the \roundingitem\ $c$ and the \roundingslot\ $s$, a user $\hat{u}$ is \textit{eligible} for $(c,s)$ in \stagethree\ if and only if 1) $\hat{u}$ has not been displayed any item at slot $s$, and 2) $c$ has not been displayed to $\hat{u}$ at any slot. Users not eligible for $(c,s)$ are not displayed any item in \stagethree\ to ensure the no-duplication constraint. For each eligible user $\hat{u}$, \stagethree\ selects $c$ for $\hat{u}$ at slot $s$ (i.e., $\textbf{A}(\hat{u},s) \leftarrow c$) if and only if ${x^\ast}^c_{\hat{u},s}$ is no smaller than the \roundingalpha\ $\alpha$. In other words, given $(c,s,\alpha)$, \stagethree\ co-displays $c$ to a target subgroup $U$ that consists of every eligible user $\hat{u}$ with ${x^\ast}^c_{\hat{u},s} \geq \alpha$. Therefore, the \roundingalpha\ $\alpha$ plays a key role to the performance bound in the formation of subgroups. Later we prove that with the above strategy, for any pair of users $u,v$ and any item $c$, $\text{Pr}(u \xleftrightarrow{c} v) \geq \frac{{y^\ast}^c_e}{4}$; or equivalently, the expected social utility of $u$ from viewing $c$ with $v$ obtained in the final \configuration\ is at least a constant factor within that in the optimal LP solution.

\algo\ repeats the process of parameter sampling and \stagethree\ until a \textit{feasible} \configuration\ is fully constructed, i.e., each user is displayed exactly one item at each slot, and the no-duplication constraint is satisfied.

\opt{full}{
\para{Revisiting independence vs. dependence.} Recall the troublesome input instance in the proof of Lemma \ref{lemma:trivial_rounding} where independent rounding performs poorly. By exploiting the dependent rounding scheme in \stagethree, since ${x^\ast}^c_{u,s} = \frac{1}{m}$ for all $c,u,s$, upon the first time a \roundingalpha\ $\alpha \leq \frac{1}{m}$ is sampled, \stagethree\ co-displays the \roundingitem\ $c$ to \textit{every user} in the shopping group, which is the optimal solution. On the other hand, independent rounding could not facilitate co-displaying an item to all users as effectively.
}

\begin{example} \label{example:random}
\sloppy For Example \ref{example:running} with the \weight s shown in Table \ref{table:fragsol}, assume that the set of focal parameters are sampled as $(c,s,\alpha) = (c_1,3,0.06).$ Since ${x^\ast}^{c_1}_{u_A,3} = {x^\ast}^{c_1}_{u_B,3} = {x^\ast}^{c_1}_{u_D,3} = 0.33 > 0.06 > {x^\ast}^{c_1}_{u_C,3} = 0$, \stagethree\ co-displays the tripod to the subgroup \{Alice, Bob, Dave\} at slot 3. \opt{full}{Note that this solution is not the \scenario\ configuration in Figure \ref{fig:comp_example}. }
Next, for the second set of parameters $(c,s,\alpha) = (c_4,2,0.22)$, \{Bob, Charlie, Dave\} is formed and co-displayed the memory card at slot 2, since ${x^\ast}^{c_4}_{u_B,2} = {x^\ast}^{c_4}_{u_C,2} = {x^\ast}^{c_4}_{u_D,2} = 0.33 > 0.22 > {x^\ast}^{c_4}_{u_A,2} = 0$. \opt{short}{The subsequent sets of parameters $(c,s,\alpha)$ are respectively $(c_3,1,0.04)$, $(c_5,3,0.2)$, $(c_5,1,0.31)$, $(c_2,1,0.01)$, and $(c_2,2,0.19)$ in the next five iterations, achieving a total \scenario\ utility of 9.75. Please see Section \ref{subsec:details} in the full version \cite{Online} for more details.}
%===============START OF THE DETAILED EXAMPLE===============
\opt{full}{In the third iteration, RFS selects $(c,s,\alpha) = (c_3,1,0.04)$. As only ${x^\ast}^{c_3}_{u_C,1} = 0.33$ is nonzero among the \weight s for $c_3$ at slot 1, \stagethree\ assigns PSD to \{Charlie\} alone at slot 1. Next, in iteration 4, $(c,s,\alpha) = (c_5,3,0.2)$. At this moment, only Charlie has not been assigned an item at slot 3 since the others are co-displayed the tripod earlier. Because \weight\ ${x^\ast}^{c_3}_{u_C,5} = 0.33 > 0.2$, the SP camera is displayed to \{Charlie\} at slot 3. Iteration 5 generates $(c,s,\alpha) = (c_5,1,0.31)$. For the users without displayed items at slot 1, only Alice and Dave (but not Bob) have their \weight s of the SP camera larger than 0.31. Thus \{Alice, Dave\} are co-displayed the item at slot 1. The final two iterations with ${x^\ast}^{c_3}_{u_C,5}$ as $(c_2,1,0.01)$ and $(c_2,2,0.19)$ displays the DSLR camera to \{Bob\} at slot 1 and \{Alice\} at slot 2. This finalizes the construction of a \configuration\ as represented in Table \ref{table:algr_result}, achieving a total \scenario\ utility of 9.75.\footnote{It is worth noting that those iterations with focal parameters not leading to any item display are omitted from this example. Indeed, it suffices for RFS to sample from the combinations of focal parameters that does result in item displays, which also help improve the practical efficiency of \algor. We revisit this issue in the proof of Theorem \ref{thm:randomized_bound_long} and also in the enhancement strategies in Section \ref{subsec:enhancements}.}}
%===============END OF THE DETAILED EXAMPLE===============
\hfill \qedsymbol
\end{example}
%A: c_5 c_2 c_1
%B: c_2 c_4 c_1
%C: c_3 c_4 c_5
%D: c_5 c_4 c_1

\opt{short}{The theoretical guarantee of the \algo\ algorithm is given in the following results, which we explicitly prove in Section \ref{subsec:details} in the full version \cite{Online} due to the space constraint.} \opt{full}{We then show that \algo\ is a 4-approximation algorithm for \prob\ in expectation.}

\begin{restatable}{theorem}{randombound} \label{thm:randomized_bound_long}
\sloppy Given the optimal \fragsol\ $X^\ast$, \algo\ returns an expected 4-approximate \configuration\ in $O(n^2 \cdot k)$-time.
\end{restatable}

%===============START OF THE PROOF SKETCH IN SHORT VERSION===============
%\para{Proof Sketch.} Due to the space constraint, we present here a high-level sketch of the proof, while the detailed analysis is presented in the full version \cite{Online}. 

%Let $\text{OPT}$ be the optimal total \scenario\ utility in \prob. We use an \textit{iteration} to describe one round of parameter sampling and the consequent \stagethree. We start by proving that the expected value of preference utility achieved by \algo, $\mathbb{E}[\mathcal{R}_{\text{per}}]$, is at least $\sum_{c \in \mathcal{C}} \sum_{u \in V} \big( \text{p}(u, c) \cdot \frac{{x^\ast}^c_u}{2} \big)$, or equivalently, at least a half of the total preference utility obtained from the \fragsol\ $X^\ast$. First, we derive probability bounds for two events (in \cite{Online}): 1) In any iteration $t$, if $u$ is eligible for $(c,s)$, the probability $P^u_{\text{rec}}$ that $\mathbf{A}(u,s) \gets c$ is $\frac{{x^\ast}^c_{u,s}}{k \cdot m}$, by a direct analysis of \stagethree; and 2) In any iteration $t$, for any $c$, $s$, and a user $u$ eligible for $(c,s)$, the probability $P^u_{\text{ne}}$ that $u$ is not eligible for $(c,s)$ in iteration $(t+1)$ is at most $\frac{2}{k \cdot m}$, via an analysis on the total possibility that either $u$ is displayed $c$ at some slot $\hat{s}$ or $u$ is displayed some item $\hat{c}$ at slot $s$ in iteration $t$.

%Equipped with the above two important bounds, the probability lower bound that user $u$ is displayed item $c$ at slot $s$ can be derived by summing up the probability of display at each iteration: $\text{Pr}(\mathbf{A}(u,s) = c) = \sum^\infty_{t=1} \text{Pr($\mathbf{A}(u,s) \leftarrow c$ in iteration $t$)} = \sum^\infty_{t=1} P^u_{\text{rec}} \cdot \text{Pr[$u$ is eligible for $(c,s)$ in the $t$-th iteration]} = \sum^\infty_{t=1} P^u_{\text{rec}} \cdot (1-P^u_{\text{ne}})^{t-1} = \frac{P^u_{\text{rec}}}{P^u_{\text{ne}}} \geq \frac{{x^\ast}^c_{u,s}}{2}$. Thus, $\mathbb{E}[\mathcal{R}_{\text{per}}] \geq \sum_{c \in \mathcal{C}} \sum_{u \in V} \big( \text{p}(u, c) \cdot \frac{{x^\ast}^c_u}{2} \big).$

%The next step is to prove that the expected value of \textit{social} utility achieved by \algo, $\mathbb{E}[\mathcal{R}_{\text{soc}}]$, is at least $1/4$ of that in the optimal \fragsol. Note this ratio (4) is doubled compared to that of the preference utility, which is a byproduct of the fact that social utility depends on two users, thus requiring a more complicated analysis on the joint event of two displaying of items (as shown in \cite{Online}). Combining the approximation bounds of preference and social utilities completes the proof. \opt{short}{Two immediate corollaries are directly obtained from Theorem \ref{thm:randomized_bound_long} as follows. Please see \cite{Online} for all detailed proof and the time complexity analysis of \algo.}

%===============END OF THE PROOF SKETCH IN SHORT VERSION===============

\opt{full}{
\input{proof/proof_randomized.tex}
Two immediate corollaries are directly obtained from Theorem \ref{thm:randomized_bound_long} as follows.
}

\begin{restatable}{corollary}{repeatbound} \label{thm:randomized_corollary}
Repeating \algor\ and selecting the best output returns a $(4+\epsilon)$-approximate \configuration\ in $O(n^2 \cdot k \cdot \log_{\epsilon} n)$-time with high probability, i.e., with a probability $1-\frac{1}{n^{O(1)}}$. 
\end{restatable}

\begin{restatable}{corollary}{compositebound} \label{thm:composite_corollary}
\opt{full}{\sloppy}Given a (non-optimal) \fragsol\ $\Tilde{X}^\ast$ as a $\beta$-approximation of the LP relaxation problem, \algo\ returns an expected $(4 \cdot \beta)$-approximate \configuration. 
\end{restatable}

\opt{full}{
\input{proof/proof_corollaries.tex}
}

The second corollary is particularly useful in practice for improving the efficiency of \algo\ since state-of-the-art LP solvers often reach a close-to-optimal solution in a short time but need a relatively long time to return the optimal solution, especially for large inputs. Therefore, it allows for a quality-efficiency trade-off in solving \prob.

\subsection{Derandomizing \algo} \label{subsec:derandomize}
\opt{full}{\sloppy}From the investigation of \algo, we observe that the \roundingalpha\ $\alpha$ plays a key role in forming effective target subgroups in \stagethree. If $\alpha$ is close to $0$, \stagethree\ easily forms a large subgroup consisting of all users and co-displays the \roundingitem\ to them, similar to the ineffective \group\ approach. On the other hand, large $\alpha$ values lead to small subgroups, not good for exploiting social interactions. Due to the randomness involved in \algo, these caveats cannot be completely avoided. To address these issues, we aim to further strengthen the performance guarantee of \algo\ by derandomizing the selection of focal parameters to obtain a stronger version of the algorithm, namely \algodfull\ (\algod), which is a \textit{deterministic} 4-approximation algorithm. First, we observe that $\alpha$ can be assigned in a discrete manner.

\begin{observation} \label{observation:poly_many}
    There are $O(knm)$ distinct possible outcomes in \stagethree, each corresponding to a \roundingalpha\ $\alpha = {x^\ast}^c_{u,s}$, i.e., the \weight\ of an item $c$ to a user $u$ at a slot $s$.
\end{observation}

The above observation can be verified as follows. Given $c$ and $s$, the outcome of \stagethree\ with \roundingalpha\ $\alpha = x$, for any $x \in [0,1]$, is equivalent to that with $\alpha$ set to the smallest ${x^\ast}^c_{u,s} \geq x$. It enables us to derandomize \algo\ effectively. Instead of randomly sampling $(c,s,\alpha)$, we carefully evaluate the outcomes (of \stagethree) from setting ${\alpha}$ to every possible ${x^\ast}^c_{u,s}$ in the optimal \fragsol. Intuitively, it is desirable to select an ${\alpha}$ that results in the largest increment in the total \scenario\ utility. However, this short-sighted approach ignores the potentially significant increase in total \scenario\ utility in the future from the remaining users and slots that have not been processed. In fact, it always selects an outcome with $\alpha = 0$ to maximize the current utility increment. Therefore, it is necessary for \algod\ to carefully evaluate all potential future allocations of items.

\opt{short}{\revise{Specificially, \algod\ selects the set of focal parameters $(c,s,\alpha)$ to maximize a weighted sum of 1) the increment of \scenario\ utility in the current iteration via \stagethree\ with $(c,s,\alpha)$, and 2) the expected \scenario\ utility in the future from item assignments at slots that are \textit{left unfilled} in \stagethree\ with $(c,s,\alpha)$. Due to the space constraint, please see Section \ref{subsec:derandomize} in the full version \cite{Online} for the details of \algod, and an explicit proof of the following theoretical result.}}

\opt{full}{
Specifically, let $S_{\text{cur}} = \{ (\hat{u}, \hat{s}) | \mathbf{A}(\hat{u}, \hat{s}) = \text{NULL} \}$ denote the set of \textit{display units}, i.e., a slot $\hat{s}$ for a user $\hat{u}$, that have not been assigned an item before the current iteration. Let $S_{\text{tar}}(c,s,{x^\ast}^c_{u,s}) = \{ (\hat{u}, s) \in S_{\text{cur}} | {x^\ast}^{c}_{\hat{u},s} \geq {x^\ast}^c_{u,s}\}$ denote the set of display units to be assigned $c$ in \stagethree\ with ${\alpha} = {x^\ast}^c_{u,s}$. Let $S_{\text{fut}}(c,s,{x^\ast}^c_{u,s}) = S_{\text{cur}} \setminus S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})$ denote the set of remaining display units to be processed in the future. Moreover, let ${\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s}))$ be the \scenario\ utility gained by co-displaying $c$ to the target subgroup. Let ${\text{OPT}}_{\text{LP}}(S_{\text{fut}}(c,s,{x^\ast}^c_{u,s}))$ represent the expected \scenario\ utility acquired in the future from the display units in $S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})$. To strike a balance between the increment of \scenario\ utility in the current iteration and in the future, \algod\ examines every ${\alpha} = {x^\ast}^c_{u,s}$ to maximize 
\begin{align*}
    f(c,s,{x^\ast}^c_{u,s}) &= {\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})) \\
    &+ r \cdot {\text{OPT}}_{\text{LP}}(S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})),
\end{align*}
\vspace{-15pt}

\noindent where 
\vspace{-15pt}

\begin{small}
\begin{align*}
    % {\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})) &= \sum\limits_{(\hat{u},s) \in S_{\text{tar}}} [ \text{p}(\hat{u}, c) \\ &+ \sum\limits_{(\hat{v},s) \in S_{\text{tar}}, \hat{u} \neq \hat{v}} \tau(\hat{u},\hat{v},c) ], \\
    {\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})) &= \sum\limits_{(\hat{u},s) \in S_{\text{tar}}} \text{p}(\hat{u}, c) + \sum\limits_{\substack{e = (\hat{u},\hat{v}) \\ (\hat{u},s), (\hat{v},s) \in S_{\text{tar}}}} \text{w}^c_e, \\
    {\text{OPT}}_{\text{LP}}(S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})) &= \sum\limits_{c \in \mathcal{C}} \sum\limits_{s=1}^{k} [ \sum\limits_{(\hat{u},\hat{s}) \in S_{\text{fut}}} \text{p}(\hat{u}, c) {x^\ast}^c_{\hat{u},\hat{s}} \\ &+ \sum\limits_{\substack{e = (\hat{u},\hat{v}) \\ (\hat{u},\hat{s}), (\hat{v},\hat{s}) \in S_{\text{fut}}}} \text{w}^c_e {y^\ast}^c_{e,\hat{s}} ],
\end{align*}
\end{small}

\noindent $\text{w}^c_e = \tau(\hat{u},\hat{v},c)+\tau(\hat{v},\hat{u},c)$ for all $e = (\hat{u},\hat{v}) \in E$, and $r$ is the balancing ratio. In other words, \algod\ simultaneously optimizes the current and potential future \scenario\ utility in each iteration. It is summarized in Algorithm \ref{alg:deterministic_alignment_aware_rounding}.

\input{algo/damp.tex}

%===============TABLES FOR THE DETAILED EXAMPLE===============
\opt{full}{
\begin{table}[t]
	\centering
	\caption{\configuration\ returned by \algor\ for Example \ref{example:random}.}
	\label{table:algr_result}
	\begin{tabular}{l|ccc}
  &  Slot 1 & Slot 2 & Slot 3\\ \hline 
 $u_A$ &  $c_5$  & $c_2$  &  $c_1$    \\
 $u_B$ &  $c_2$  & $c_4$  &  $c_1$    \\
 $u_C$ &  $c_3$  & $c_4$  &  $c_5$  \\
 $u_D$ &  $c_5$  & $c_4$  &  $c_1$     \\
	\end{tabular}
\end{table}
\begin{table}[t]
	\centering
	\caption{\configuration\ returned by \algod\ for Example \ref{example:random}.}
	\label{table:algd_result}
	\begin{tabular}{l|ccc}
  &  Slot 1 & Slot 2 & Slot 3\\ \hline 
 $u_A$ &  $c_5$  & $c_1$  &  $c_2$    \\
 $u_B$ &  $c_5$  & $c_1$  &  $c_2$    \\
 $u_C$ &  $c_5$  & $c_3$  &  $c_2$  \\
 $u_D$ &  $c_5$  & $c_1$  &  $c_4$     \\
	\end{tabular}
\end{table}
\begin{table}[t]
	\centering
	\caption{Configuration by the baseline approaches for Example \ref{example:random}.}
	\label{table:baseline_result}
	\begin{tabular}{l|ccc}
 \personalized\ &  Slot 1 & Slot 2 & Slot 3\\ \hline 
 $u_A$ &  $c_5$  & $c_2$  &  $c_1$    \\
 $u_B$ &  $c_2$  & $c_1$  &  $c_4$    \\
 $u_C$ &  $c_3$  & $c_4$  &  $c_2$  \\
 $u_D$ &  $c_4$  & $c_5$  &  $c_3$     \\\\
 
 \group\ &&&\\ \hline 
 $\{u_A, u_B, u_C, u_D\}$ &  $c_5$  & $c_1$  &  $c_2$    \\\\
 
 \friendship\ &&&\\ \hline 
 $\{u_A,u_D\}$ &  $c_5$  & $c_1$  &  $c_4$    \\
 $\{u_B,u_C\}$ &  $c_2$  & $c_4$  &  $c_3$    \\\\
 
 \preference\ &&&\\ \hline 
 $\{u_A,u_B\}$ &  $c_2$  & $c_1$  &  $c_5$    \\
 $\{u_C,u_D\}$ &  $c_4$  & $c_5$  &  $c_3$    \\
	\end{tabular}
\end{table}
}

\begin{example}
\sloppy For the instance in Example \ref{example:running}, the first iteration of \algod\ with $r = \frac{1}{4}$ sets $\alpha = {x^\ast}^{c_5}_{u_B,1} = 0$, and \stagethree\ with $(c,s,{x^\ast}^c_{u,s}) = (c_5,1,0)$ co-displays the SP camera to everyone at slot 1, where $S_{\text{tar}}(c,s,{x^\ast}^c_{u,s}) = \{ (u_A,1), (u_B,1), (u_C,1), (u_D,1)\}$, $S_{\text{fut}}(c,s,{x^\ast}^c_{u,s}) = \{ (u_A,2), (u_B,2), (u_C,2), (u_D,2), (u_A,3), (u_B,3), (u_C,3),$ $(u_D,3)\}$, ${\text{ALG}}(S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})) =  \text{p}(u_A,c_5) + \text{p}(u_B,c_5) + \text{p}(u_C,c_5) + \text{p}(u_D,c_5) + \text{w}^{c_5}_{(u_A,u_B)} + \text{w}^{c_4}_{(u_A,u_C)} + \text{w}^{c_4}_{(u_A,u_D)} + \text{w}^{c_4}_{(u_B,u_C)} = 3.35$, ${\text{OPT}}_{\text{LP}}(S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})) = 6.97$, and $f(c,s,{x^\ast}^c_{u,s}) = 3.35 + \frac{1}{4} \cdot 6.97 = 5.09$ is maximized. The next iteration selects $\alpha = {x^\ast}^{c_1}_{u_A,2} = 0.33$ to co-display the tripod to \{Alice, Bob, Dave\} at slot 2. \algod\ selects $\alpha = {x^\ast}^{c_2}_{u_D,3} = 0$, $\alpha = {x^\ast}^{c_4}_{u_A,3} = 0$, and $\alpha = {x^\ast}^{c_3}_{u_D,2} = 0$ in the next three iterations, resulting in a total \scenario\ utility of 9.85, which is slightly larger than \algor\ (9.75) in Example \ref{example:random}. The returned \configuration\ is shown in Table \ref{table:algd_result}. 
%\opt{short}{For this running example, the optimal solution is the \configuration\ shown at the top of Figure \ref{fig:example}, with a total \scenario\ utility of 10.35. Both \algor\ and \algod\ achieve a near-optimal solution; by contrast, the total \scenario\ utility for the \personalized\ and \group\ approaches, as illustrated in Figure \ref{fig:comp_example}, are 8.25 and 8.35, respectively. For more details of the baseline approaches, please refer to Section \ref{subsec:derandomize} in the full version \cite{Online}. \hfill \qedsymbol}

For this running example, the optimal solution is the \configuration\ shown at the top of Figure \ref{fig:example}, with a total \scenario\ utility of 10.35. The \personalized\ approach retrieves the top-$3$ preferred items for each user, e.g., $\langle c_5, c_2, c_1 \rangle$ for Alice, and achieves a total \scenario\ utility of 8.25. For the \group\ approach, the total \scenario\ utility for the universal subgroup \{Alice, Bob, Charlie, Dave\} viewing each item is aggregated. For example, the total \scenario\ utility of the subgroup of all users viewing $c_1$ would be $\sum\limits_{u \in V} \text{p}(u,c_1) + \sum\limits_{u,u' in V} \tau(u,u',c_1)$, which equals the summation of all values in the first row in Table \ref{table:sat}, or 2.6 (note that $\lambda = 0.5$ and the objective is scaled up by 2 here). The top-$3$ items, i.e., $\langle c_5, c_1, c_2 \rangle$, is retrieved and co-displayed to all users. This achieves a total \scenario\ utility of 8.35. 

We also compare with two variations of the subgroup approach, namely the \friendship\ and \preference\ approaches, where the former pre-partitions the subgroups based on social relations among the users, while the latter finds subgroups with similar item preferences. The \friendship\ approach first partitions the social network into two equally sized and dense subgroups \{Alice, Dave\} and \{Bob, Charlie\}. Items are then determined analogously to the \group\ approach, resulting in a total \scenario\ utility of 8.4. Finally, the \preference\ approach partitions the network into \{Alice, Bob\} and \{Charlie, Dave\}. The total \scenario\ utility would be 8.7.

The configurations returned by these four baseline approaches are consistent with Figure \ref{fig:comp_example} and are also summarized in Table \ref{table:baseline_result}. To sum up, the total \scenario\ utility for \algor, \algod, and the \personalized, \group, \friendship\ and \preference\ approaches, are 9.75, 9.85, 8.25, 8.35, 8.4 and 8.7, respectively. Therefore, both \algor\ and \algod\ achieves a near-optimal solution. \hfill \qedsymbol
\end{example}

%A: c_5 c_1 c_2
%B: c_5 c_1 c_2
%C: c_5 c_3 c_2
%D: c_5 c_1 c_4
 
In \algod, $r$ serves as a turning knob to strike a good balance between the current increment in \scenario\ utility and the potential \scenario\ utility in the future. Specifically, we prove that by setting $r = \frac{1}{4}$ in each iteration, \algod\ is a deterministic 4-approximation algorithm for \prob. We also empirically evaluate the performance of \algod\ with different values of $r$ in Section \ref{subsec:diff_r}.%\opt{short}{ (presented in \cite{Online} due to space constraint).}\opt{full}{ }
}

\begin{restatable}{theorem}{derandombound} \label{thm:derandomized_bound_long}
\sloppy Given the optimal \fragsol\ $X^\ast$, \algod\ returns a worst-case 4-approximate \configuration\ in $O(n \cdot m \cdot k \cdot |E|)$-time.
\end{restatable}

%===============START OF THE PROOF SKETCH IN SHORT VERSION===============
% \opt{short}{
% \begin{proof}
% Please see Section \ref{subsec:derandomize} in \cite{Online}.
% \end{proof}
%\para{Proof Sketch.} We again provide a proof sketch here and leave the details in \cite{Online}. To prove the approximation ratio for \algod, we first show that, in an iteration of \textit{\algo} (instead of \algod), the expected value of $f(c,s,{x^\ast}^c_{u,s})$ is at least $\frac{{\text{OPT}}_{\text{LP}}(S_{\text{cur}})}{4}$. Thus, for each iteration of \algod, there exists at least one $(c,u,s)$ such that $f(c,s,{x^\ast}^c_{u,s}) \geq \frac{{\text{OPT}}_{\text{LP}}(S_{\text{cur}})}{4}$, and \algod\ always picks such a set of parameters.

%Let the total number of iterations in \algod\ be $T$. Let $S^{t}_{\text{tar}}$ and $S^{t}_{\text{fut}}$ denote $S_{\text{tar}}(c,s,{x^\ast}^c_{u,s})$ and $S_{\text{fut}}(c,s,{x^\ast}^c_{u,s})$ in the $t$-th iteration of \algod , and $S^{t}_{\text{cur}} = S^{t}_{\text{tar}} \cup S^{t}_{\text{fut}}$. By the above result, we have $\text{ALG}(S^t_{\text{tar}}) + \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^t_{\text{fut}}) \geq \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^t_{\text{cur}})$ for all $t = 1, 2, \cdots, T$. Also, $\text{OPT}_{\text{LP}}(S^t_{\text{cur}}) = \text{OPT}_{\text{LP}}(S^{t-1}_{\text{fut}})$ for all $t > 1$. Therefore, 
% \begin{small}
% \begin{align*}
%     \text{ALG}(S^1_{\text{tar}}) + \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^1_{\text{fut}}) &\geq \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^1_{\text{cur}})  \\
%     \text{ALG}(S^2_{\text{tar}}) + \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^2_{\text{fut}}) &\geq \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^2_{\text{cur}}) = \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^1_{\text{fut}})\\
%     &\vdots\\
%     \text{ALG}(S^{T}_{\text{tar}}) + \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^{T}_{\text{fut}}) &\geq \frac{1}{4} \cdot \text{OPT}_{\text{LP}}(S^{T-1}_{\text{fut}}).
% \end{align*}
% \end{small}
%by summing up all the inequalities, we have
%$\sum_{t=1}^{T} \text{ALG}(S^{t}_{\text{tar}}) \geq \frac{\text{OPT}_{\text{LP}}(S^1_{\text{cur}})}{4} - \frac{\text{OPT}_{\text{LP}}(S^{T}_{\text{fut}})}{4} = \frac{\text{OPT}}{4}$, which completes the proof.

%Practically, the computation of $f(c,s,{x^\ast}^c_{u,s})$ can be effectively paralleled in \algod\ with a parallelism of $O(nmk)$, which could effectively reduce the time complexity of \algod\ from $O(n^2 \cdot m^2 \cdot k^2 \cdot |E|)$ to $O(n \cdot m \cdot k \cdot |E|)$. Due to the space constraint, please see the full version \cite{Online} for the omitted details and the time complexity analysis.
%}
%===============END OF THE PROOF SKETCH IN SHORT VERSION===============

\opt{full}{
\input{proof/proof_derandomized.tex}
}

\subsection{Enhancements} \label{subsec:enhancements}
\revise{In the following, we detail enhancements of the \algo\ and \algod\ algorithms. First, we show that \algo\ (and \algod) supports values of $\lambda \neq \frac{1}{2}$ via a simple scaling on the inputs. We then design two advanced strategies, including an \textit{advanced LP transformation technique} and a \textit{new focal parameter sampling scheme}, to improve the efficiency of \algo\ and \algod. The LP transformation technique derives a new LP formulation to reduce the number of decision variables and constraints from $O((n+|E|)mk)$ to $O((n+|E|)m)$ by condensing the $x^c_{u,s}$ variables ($k$ is the number of slots). We prove that the optimal objective in the new formulation is exactly that in the original one. The focal parameter sampling scheme maintains a \textit{maximum \weight} $\bar{x^\ast}^c_s$ (detailed later) for each pair of item $c$ and slot $s$ to avoid unnecessary sampling of focal parameters $(c,s,\alpha)$ when $\alpha \geq \max\limits_{u \in V} {x^\ast}^c_{u,s}$, especially for a large $k$. We prove that the sampling results of the new sampling technique and the original one are the same. Therefore, the efficiency of \algo\ can be effectively improved without sacrificing the solution quality. Finally, we extend \algo\ and \algod\ to support \probtwo\ by tailoring \stagethree\ with consideration of the additional VR-related constraints. \opt{short}{Due to the space constraint, we present the details in Section \ref{subsec:enhancements} in the full version \cite{Online}.}}

\opt{full}{
\para{(1) Supporting Other Values of $\lambda$.}
First, observe that $\lambda = 0$ corresponds to a special case of maximizing only the total preference utility, where a simple greedy algorithm can find the exact optimal solution. Assume that $\lambda \neq 0$. To support the cases with $\lambda \neq \frac{1}{2}$, \algo\ first sets the \textit{scaled preference values} for each $(u,c)$ as $\text{p'}(u,c) = \frac{1-\lambda}{\lambda}\text{p}(u,c)$. This value is then used instead of $\text{p}(u,c)$ in the LP relaxation problem, as well as in the computation of $f(c,s,{x^\ast}^c_{u,s})$ in DPS in \algod. 
Since
\begin{align*}
    &(1-\lambda)\cdot\text{p}(u,c) + \lambda\cdot\sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c)\\
    =& 2 \lambda \cdot (\frac{1}{2}\cdot\text{p'}(u,c) + \frac{1}{2}\cdot\sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c)),
\end{align*}
each instance with $\lambda \neq \frac{1}{2}$ can be transformed to an instance with $\lambda = \frac{1}{2}$ by this scaling of input parameters, where \algo\ and \algod\ can achieve the approximation ratio.

\para{(2) Advanced LP Transformation.} Recall that the LP relaxation of the \prob\ problem (denote by $\mathsf{LP}_{\mathsf{SVGIC}}$) is 

$$ \text{max} \sum\limits_{u \in V} \sum\limits_{c \in \mathcal{C}} [ (1-\lambda) \cdot \text{p}(u, c) \cdot x^c_u + \lambda \cdot \sum\limits_{e = (u,v) \in E} ( \tau(u,v,c) \cdot y^c_e) ] $$

\noindent subject to the following constraints:
\begin{small}
\begin{align*}
    \sum_{s=1}^{k} x^c_{u,s} \leq 1, \quad & \forall u \in V, c \in \mathcal{C} \\%\label{ilp:no_replicated_item}\\
    \sum_{c \in \mathcal{C}} x^c_{u,s} = 1, \quad & \forall u \in V, s \in [k] \\%\label{ilp:one_slot_one_item}\\
    x^c_u = \sum_{s=1}^{k} x^c_{u,s}, \quad & \forall u \in V, c \in \mathcal{C} \\%\label{ilp:user_recommended}\\
    y^c_{e} = \sum_{s=1}^{k} y^c_{e,s}, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \\%\label{ilp:edge_recommended}\\
    y^c_{e,s} \leq x^c_{u,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \\%\label{ilp:direct_relation_1} \\
    y^c_{e,s} \leq x^c_{v,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \\%\label{ilp:direct_relation_2} \\
    x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e \geq 0, \quad & \forall u \in V, e \in E, s \in [k], c \in \mathcal{C}. %\label{ilp:integrality}.
\end{align*}
\end{small}

Solving $\mathsf{LP}_{\mathsf{SVGIC}}$, which is the first step of the \algo\ algorithm, deals with $O((n+|E|)mk)$ decision variables and $O((n+|E|)mk)$ constraints. In the following, we transform $\mathsf{LP}_{\mathsf{SVGIC}}$ into a more compact linear program formulation $\mathsf{LP}_{\mathsf{SIMP}}$ with fewer decision variables as follows.

$$ \text{max} \sum\limits_{u \in V} \sum\limits_{c \in \mathcal{C}} [ (1-\lambda) \cdot \text{p}(u, c) \cdot \mathtt{x}^c_u + \lambda \cdot \sum\limits_{e = (u,v) \in E} ( \tau(u,v,c) \cdot \mathtt{y}^c_e) ] $$

\noindent subject to the following constraints:
\begin{small}
\begin{align*}
    \mathtt{x}^c_{u} \leq 1, \quad & \forall u \in V, c \in \mathcal{C} \\
    \sum_{c \in \mathcal{C}} \mathtt{x}^c_{u} = k, \quad & \forall u \in V \\
    \mathtt{y}^c_{e} \leq \mathtt{x}^c_{u}, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \\
    \mathtt{y}^c_{e} \leq \mathtt{x}^c_{v}, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \\
    \mathtt{x}^c_{u}, \mathtt{y}^c_{e} \geq 0, \quad & \forall u \in V, e \in E, c \in \mathcal{C}.
\end{align*}
\end{small}

To avoid confusion, we use normal math symbols ($x$ and $y$) to represent decision variables in $\mathsf{LP}_{\mathsf{SVGIC}}$ and Typewriter symbols ($\mathtt{x}$ and $\mathtt{y}$) to denote those in $\mathsf{LP}_{\mathsf{SIMP}}$. Let $\text{OPT}_{\mathsf{SIMP}}$ and $\text{OPT}_{\mathsf{SVGIC}}$ denote the optimal objective values in $\mathsf{LP}_{\mathsf{SIMP}}$ and $\mathsf{LP}_{\mathsf{SVGIC}}$. We have the following observation. %Recall that an optimal solution is represented by $X^\ast$ (Please see the discussion for R4DW1.3). :

\begin{observation} \label{scaledLP}
$\text{OPT}_{\mathsf{SIMP}} = \text{OPT}_{\mathsf{SVGIC}}$ always holds. Moreover, given an optimal solution $\mathtt{X}^{\ast} = \{ \mathtt{x}^c_u \}$ for $\mathsf{LP}_{\mathsf{SIMP}}$, there exists an optimal solution ${X^\ast}$ of $\mathsf{LP}_{\mathsf{SVGIC}}$ with ${{x^\ast}}^c_{u,s} = \frac{1}{k} \cdot {\mathtt{x}^{\ast}}^c_u, \forall c, u, s$. 
\end{observation}

\begin{proof}
We first prove $\text{OPT}_{\mathsf{SIMP}} \leq \text{OPT}_{\mathsf{SVGIC}}$. Given any feasible solution $\mathtt{X}$ of $\mathsf{LP}_{\mathsf{SIMP}}$, let $X$ denote a solution of $\mathsf{LP}_{\mathsf{SVGIC}}$ such that ${x}^c_{u,s} = \frac{1}{k} \cdot \mathtt{x}^c_u, \forall c, u, s$. By construction, we have $x^c_u = \sum_{s=1}^{k} x^c_{u,s} = k \cdot \frac{1}{k} \cdot \mathtt{x}^c_u = \mathtt{x}^c_u$ for all $c,u,s$, and analogously $y^c_e = \mathtt{y}^c_{e}$ for all $c,e$. Therefore, $X$ is feasible in $\mathsf{LP}_{\mathsf{SVGIC}}$. Moreover, it achieves the same objective value in $\mathsf{LP}_{\mathsf{SVGIC}}$ as $\mathtt{X}$ in $\mathsf{LP}_{\mathsf{SIMP}}$, which implies $\text{OPT}_{\mathsf{SIMP}} \leq \text{OPT}_{\mathsf{SVGIC}}$. We then prove $\text{OPT}_{\mathsf{SIMP}} \geq \text{OPT}_{\mathsf{SVGIC}}$. Given any feasible solution $X$ of $\mathsf{LP}_{\mathsf{SVGIC}}$, let $\mathtt{X}$ denote a solution of $\mathsf{LP}_{\mathsf{SIMP}}$ such that $\mathtt{x}^c_u = x^c_u = \sum_{s=1}^{k} x^c_{u,s}$. Similarly, $\mathtt{X}$ is a feasible solution of $\mathsf{LP}_{\mathsf{SIMP}}$, and it achieves exactly the same objective value in $\mathsf{LP}_{\mathsf{SIMP}}$ as $X$ in $\mathsf{LP}_{\mathsf{SVGIC}}$. Therefore, $\text{OPT}_{\mathsf{SIMP}} \geq \text{OPT}_{\mathsf{SVGIC}}$. Combining the above, we have $\text{OPT}_{\mathsf{SIMP}} = \text{OPT}_{\mathsf{SVGIC}}$, and the second part of the observation follows from the above construction.
\end{proof}

As \algo\ requires only \textit{one} optimal solution for $\mathsf{LP}_{\mathsf{SVGIC}}$, it suffices for \algo\ to first solve the above simplified linear program $\mathsf{LP}_{\mathsf{SIMP}}$ with only $O((n+|E|)m)$ decision variables and constraints. \algo\ then scales the optimal solution by a factor of $\frac{1}{k}$ according to Observation \ref{scaledLP} to find an optimal solution for $\mathsf{LP}_{\mathsf{SVGIC}}$. Therefore, $\mathsf{LP}_{\mathsf{SIMP}}$ effectively improves the efficiency of \algo. % and further enhance the scalability of \algo\ to $k$, as the complexity of the linear program no longer depends on $k$.\\

% \begin{observation}
% Given an optimal solution $X^\ast = \{ {x^\ast}^c_{u,s} \}$ of $\mathsf{LP}_{\mathsf{SVGIC}}$, there exists another solution $\overline{X}$ achieving the same objective value in $\mathsf{LP}_{\mathsf{SVGIC}}$, where ${\overline{X}}^c_{u,s} = \frac{1}{k} \cdot \sum\limits_{s=1}^{k} {x^\ast}^c_{u,s}, \forall c, u, s$. 
% \end{observation}

% Intuitively, ${X^\ast}'$ can be viewed as re-distributing ${X^\ast}$ uniformly across all display slots. It is then straightforward to verify that (i) ${X^\ast}'$ is a feasible solution, and (ii) ${X^\ast}'$ achieves an exactly identical objective to $X^\ast$. 

% Therefore, the optimal value of the original LP is always equivalent to the optimal value of the following LP with an additional constraint that requires the decision variables ${x^\ast}^c_{u,s}$ not depending on $s$:

% $$ \text{max} \sum\limits_{u \in V} \sum\limits_{c \in \mathcal{C}} [ (1-\lambda) \cdot \text{p}(u, c) \cdot x^c_u + \lambda \cdot \sum\limits_{e = (u,v) \in E} ( \tau(u,v,c) \cdot y^c_e) ] $$

% \noindent subject to the following constraints:
% \begin{small}
% \begin{align*}
%     \sum_{s=1}^{k} x^c_{u,s} \leq 1, \quad & \forall u \in V, c \in \mathcal{C} \\%\label{ilp:no_replicated_item}\\
%     \sum_{c \in \mathcal{C}} x^c_{u,s} = 1, \quad & \forall u \in V, s \in [k] \\%\label{ilp:one_slot_one_item}\\
%     x^c_u = \sum_{s=1}^{k} x^c_{u,s}, \quad & \forall u \in V, c \in \mathcal{C} \\%\label{ilp:user_recommended}\\
%     y^c_{e} = \sum_{s=1}^{k} y^c_{e,s}, \quad & \forall e = (u,v) \in E, c \in \mathcal{C} \\%\label{ilp:edge_recommended}\\
%     y^c_{e,s} \leq x^c_{u,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \\%\label{ilp:direct_relation_1} \\
%     y^c_{e,s} \leq x^c_{v,s}, \quad & \forall e = (u,v) \in E, s \in [k], c \in \mathcal{C} \\%\label{ilp:direct_relation_2} \\
%     x^c_{u,s} = x^c_{u,s'}, \quad & \forall u \in V, c \in \mathcal{C}, s, s' \in [k]\\
%     x^c_{u,s}, x^c_u, y^c_{e,s}, y^c_e \geq 0, \quad & \forall u \in V, e \in E, s \in [k], c \in \mathcal{C}. %\label{ilp:integrality}.
% \end{align*}
% \end{small}

% This LP can be further transformed as follows:

\para{(3) Advanced Focal Parameter Sampling.} In \algo, a set of focal parameters $(c,s,\alpha)$ is sampled uniformly at random for each iteration. However, for input instances with a large $k$, the utility factor ${x^\ast}^c_{u,s}$ of assigning item $c$ to user $u$ at slot $s$ tends to become smaller, e.g., roughly $O(\frac{1}{k})$, especially after the above LP transformation strategy is applied. Recall that \algo\ compares $\alpha$ to every user eligible for viewing item $c$ at slot $s$ and displays $c$ if ${x^\ast}^c_{u,s} \geq \alpha$. If $\alpha > \max\limits_{u \in V} {x^\ast}^c_{u,s}$, \algo\ essentially remains idle (i.e., making no progress) in the current round and needs to re-sample another set of focal parameters in the next iteration. For instances with large $k$, it is thus more difficult for \algo\ to effectively sample a set of \textit{good} focal parameters without the above property.

To address the above issue, we design an advanced focal parameter sampling scheme as follows. For each pair of $(c,s)$, \algo\ maintains the \textit{maximum \weight} $\bar{x^\ast}^c_s = \max\limits_{u \in V} \{ {x^\ast}^c_{u,s} | u \, \text{is eligible for} \, (c,s)\}$. Specifically, $\bar{x^\ast}^c_s$ is initialized as $\max\limits_{u \in V} {x^\ast}^c_{u,s}$ after $X^\ast$ (the optimal solution of LP) is retrieved, and it is constantly updated along the rounding process (as users eligible for $(c,s)$ decrease). In each iteration, \algo\ first randomly samples a pair $(c,s)$ with probability $\frac{\bar{x^\ast}^c_s}{\sum\limits_{c \in \mathcal{C}, s \in [k]}\bar{x^\ast}^c_s}$, i.e., proportional to the value $\bar{x^\ast}^c_s$. It then samples $\alpha$ uniformly at random from $[0,\bar{x^\ast}^c_s]$. The following observation indicates that the distribution of outcomes in this advanced sampling scheme is equivalent to the distribution of outcomes when $(c,s,\alpha)$ is sampled directly and only from the pool of focal parameters that lead to a successful assignment of at least one item to one user at some slot. 

\begin{observation}
For any set of good focal parameter $(c,s,\alpha)$ such that $\alpha \leq \max\limits_{u \in V} {x^\ast}^c_{u,s}$, the probability of the event that \stagethree\ ends up with the same behavior as if $(c,s,\alpha)$ is sampled in the advanced focal parameter sampling scheme is the conditional probability of the same event in the original sampling scheme given that a set of good focal parameters is sampled.
\end{observation}
\begin{proof}
First, in the original sampling scheme, a set of good focal parameters is sampled if $\alpha$ is at most $\bar{x^\ast}^c_s$ for the selected $(c,s)$. Denote this event $\mathsf{GOOD}$. The total probability of this event is thus $\text{Pr}_{\text{orig}}(\mathsf{GOOD}) = \sum\limits_{c \in \mathcal{C}, s \in [k]} \frac{1}{k \cdot m}(\bar{x^\ast}^c_s)$. Next, by construction, it is straightforward that the advanced sampling scheme only samples good focal parameters. Consider a set of good focal parameter $(c,s,\alpha)$. Denote $u_1$ and $u_2$ as the users such that $u_1 = \argmax\limits_{{x^\ast}^c_{u,s} < \alpha} {x^\ast}^c_{u,s}$ and $u_2 = \argmin\limits_{{x^\ast}^c_{u,s} \geq \alpha} {x^\ast}^c_{u,s}$. By definition, if \stagethree\ chooses any $\alpha \in ({x^\ast}^c_{{u_1},s}, {x^\ast}^c_{{u_2},s}]$, it ends up with the same behavior as if $(c,s,\alpha)$ is sampled. Denote this event $\mathsf{TARGET}$. With $(c,s)$ given, this happens with probability $p_\alpha = {x^\ast}^c_{{u_2},s} - {x^\ast}^c_{{u_1},s}$. Note that $u_2$ is guaranteed to exist, and we replace ${x^\ast}^c_{{u_1},s}$ with 0 if $u_1$ does not exist (i.e., the case where every eligible user is assigned $c$ by \stagethree). In the advanced sampling scheme, the probability of this event is thus $\text{Pr}_{\text{adv}}(\mathsf{TARGET}) = \frac{\bar{x^\ast}^c_s}{\sum\limits_{c \in \mathcal{C}, s \in [k]}\bar{x^\ast}^c_s} \cdot p_\alpha$. On the other hand, in the original sampling scheme, the probability of this event is $\text{Pr}_{\text{orig}}(\mathsf{TARGET}) = \frac{1}{k \cdot m} \cdot p_\alpha$. We have
\begin{align*}
    \text{Pr}_{\text{orig}}(\mathsf{TARGET} | \mathsf{GOOD}) &= \frac{\text{Pr}_{\text{orig}}(\mathsf{TARGET})}{\text{Pr}_{\text{orig}}(\mathsf{GOOD})}\\
    &= \frac{\frac{1}{k \cdot m} \cdot p_\alpha}{\sum\limits_{c \in \mathcal{C}, s \in [k]} \frac{1}{k \cdot m}(\bar{x^\ast}^c_s)}\\
    &= \frac{p_\alpha}{\sum\limits_{c \in \mathcal{C}, s \in [k]}\bar{x^\ast}^c_s}\\
    &= \text{Pr}_{\text{adv}}(\mathsf{TARGET}).
\end{align*}
The observation follows.
\end{proof}

Therefore, the advanced focal sampling scheme effectively improves the efficiency of \algo\ since it discards the non-contributing sampling events in advance. Note that it can also be applied to improve \algod\ such that the events of selecting non-controlling focal parameters will not be simulated in the derandomization process. %Therefore, it achieves a significant speedup to both \algo\ and \algod. 
The main algorithm \algo\ with the advanced LP transformation strategy and focal sampling scheme are detailed in Algorithm \ref{alg:modified_main_algo}.

\input{algo/algo_modified.tex}

\para{Extending \algo\ for \probtwo.} To modify \algo\ (and consequently, \algod) to support the teleportation and subgroup size constraints in VR, the LP relaxation problem is first replaced by the corresponding formulation in Section \ref{subsec:hardness_ip}, i.e., with Constraints \ref{ilp2:indirect_relation_1}, \ref{ilp2:indirect_relation_2} and \ref{ilp2:integrality}. Next, in each iteration of \stagethree, instead of displaying the \roundingitem\ $c$ to all eligible users $\hat{u}$ with ${x^\ast}^c_{u,s} \geq \alpha$, \stagethree\ first checks the number of users already displayed $c$ at the \roundingslot\ $s$. It then iteratively adds \textit{the eligible user with the highest \weight\ of $c$ at slot $s$} until the number of users displayed $c$ at slot $s$ reaches the size constraint $M$ or every user is examined. If the size constraint is reached, \stagethree\ \textit{locks} the item $c$ at slot $s$ by setting ${x^\ast}^c_{u,s} = 0$ for all remaining eligible users, as well as removes $(c,s,\alpha)$ from the set of candidate parameter sets in \algod. Therefore, \algo\ never displays more than $M$ users to the same item in the final \configuration.
}

==> stash/sec5_extensions.tex <==
\section{Extensions for Practical Scenarios}\label{sec:extension}

\revise{In this section, we extend \prob\ and \algo\ to support a series of practical scenarios. 1) \textit{Commodity values}. Each item is associated with a commodity value to maximize the total profit.  2) \textit{Layout slot significance}. Each slot location is associated with a different significance (e.g., center is better) according to retailing researches \cite{slot, shelf}. 3) \textit{Multi-View Display}, where a user can be displayed multiple items in a slot, including one default, personally preferred item in the \textit{primary view} and multiple items to view with friends in \textit{group views}, and the primary and group views can be freely switched. 4) \textit{Generalized social benefits}, where social utility can be measured from not only the pairwise (each pair of friends) but also group-wise (any group of friends) perspectives. 5) \textit{Subgroup change}, where the fluctuations (i.e., change of members) between the partitioned subgroups at consecutive slots are limited to ensure smooth social interactions as the elapse of time. 6) \textit{Dynamic scenario}, where users dynamic join and leave the system with different moving speeds. \opt{short}{Due to the space constraint, we present the details in Section \ref{sec:extension} in the full version of the paper \cite{Online}.}}

\opt{full}{
\para{A. Commodity Value.} The current objective function, i.e., maximizing the total utility among all users, is not designed from retailer's perspective. In contrast, it will be more profitable to maximize the \textit{total expected profit} by taking into account the commodity values, while regarding the final \scenario\ utility as the willingness/likelihood of purchases. Therefore, the ILP formulation of \prob\ and \algo\ can be modified to examine the total \scenario\ utility weighted by a commodity value $\omega_c$ for each item $c$. Let $\omega_c$ denote the commodity price of each item $c$. The new objective of \prob\ is the weighted total \scenario\ utility as follows.

$$ \sum\limits_{u \in V} \sum\limits_{s=1}^{k} \omega_{\mathbf{A}^{\ast}(u,s)} \cdot [\text{p}(u, \mathbf{A}^{\ast}(u,s)) + \sum\limits_{v | u \xleftrightarrow{\mathbf{A}^{\ast}(u,s)} v} \tau(u,v,\mathbf{A}^{\ast}(u,s))]. $$


\para{B. Layout Slot Significance.} 
Retailing researches \cite{slot, shelf} manifest that different slot locations in the item placement layout have varying significance for users. For example, the slots at the center of an aisle are nine times more important than the slots at the ends \cite{slot}. Vertical slots right at the eye-level of users are also more significant \cite{shelf}. Therefore, it is important for \prob\ to not only select the items but also optimize the corresponding placements in the shelf. Specifically, let $\gamma_s$ represent the relative significance of slot $s$ in the layout. The new objective of \prob\ is the \scenario\ utility, weighted by the relative significance as follows.

$$ \sum\limits_{u \in V} \gamma_s \cdot \sum\limits_{s=1}^{k} [\text{p}(u, \mathbf{A}^{\ast}(u,s)) + \sum\limits_{v | u \xleftrightarrow{\mathbf{A}^{\ast}(u,s)} v} \tau(u,v,\mathbf{A}^{\ast}(u,s))]. $$


% \para{C. Social Benefits from Unaligned Display.} The objective function in \prob\ only considers the social utility of co-display items at \textit{aligned} slots, i.e., the same slots displayed to friends. % for users to gain social influence from friends, they need to view the item at the same slot in the \configuration. 
% In contrast, \textit{unaligned co-display} also considers the remote social interactions (e.g., via messengers) of the friends at different slots for the same item. %Intuitively, social benefits should be the highest when the users view the item at identical slots as in the basic \prob\ problem, and then decrease as the distance between two slots increases. 
% Let $\zeta(s,s') \in [0,1]$ denote be the weight of the social benefit when the co-display happens \textit{across} two different slots $s$ and $s'$, and let $\zeta(s,s) = 1$ because face-to-face social interactions are usually more encouraged. We introduce a generalized notation $u \xleftrightarrow{c}_{s,s'} v$ to represent the case with user $u$ seeing item $c$ at slot $s$ and another user $v$ viewing $c$ at slot $s'$. The new objective of \prob\ is then generalized as follows.
% \begin{small}
% $$ \sum\limits_{u \in V} \sum\limits_{s=1}^{k} [\text{p}(u, \mathbf{A}^{\ast}(u,s)) + \sum\limits_{v | u \xleftrightarrow{\mathbf{A}^{\ast}(u,s)}_{s,s'} v} \zeta(s,s') \cdot \tau(u,v,\mathbf{A}^{\ast}(u,s))]. $$
% \end{small}
% }

\newpage

\para{C. Multi-View Display} (MVD). \configuration\ with CID allows each user to see only \textit{one} item at each slot. In contrast, MVD \cite{RL14,LH18} has been proposed to support the display of multiple items at the same slot, so that the primary view (for personally preferred item) and the group view (for common item with friends) can be freely switched. %However, switching from the default displayed item to another item may incur an additional cost to immersion. Therefore, it is important to display the most profitable item as the default for the users. To extend \prob\ to also support MVD, 
Let $\beta$ denote the maximum number of items (i.e., views) displayed for each user in each slot (depending on the user interface). %Let $\text{c}_{\text{switch}}$ represent the immersion loss factor during a view switching. In the following, %. Instead of a scalar function $\mathbf{A}$, 
an \textit{MVD-supportive} \configuration\ $\mathbb{A}$ maps a tuple $(u,s)$ to an itemset $\mathbb{A}(u,s)$ with at most $\beta$ items, and the new objective function of \prob\ is as follows.

$$ \sum\limits_{u \in V} \sum\limits_{s=1}^{k} \big( \sum\limits_{c \in \mathbb{A}^{\ast}(u,s)} [\text{p}(u,c) + \sum\limits_{v | u \xleftrightarrow{c} v} \tau(u,v,c)] $$ %- (|\mathbb{A}^{\ast}(u,s)| - 1) \cdot \text{c}_{\text{switch}} \big). 

\para{D. Generalized Social Benefits.} In \prob\, $\tau(u,v,c)$ considers only the \textit{pair-wise} social interaction, i.e., social discussion and influence between two users viewing the common item. However, existing research on social influence \cite{HJH16KDD, HyperInfluence17, HyperInfluence19} manifests that quantifying the magnitude of social influence from \textit{group-wise} interactions is more general since the pair-wise interaction is a special case of the group-wise interaction. Therefore, let $\tau(u,\mathcal{V},c)$ denote the subgroup social utility for user $u$ when co-displaying $c$ to \textit{a subgroup of friends} $\mathcal{V}$ learned from group-wise social interaction models such as \cite{HJH16KDD}. Let $u \xleftrightarrow[s]{c} \mathcal{V}$ represent the \textit{maximal group} co-display\footnote{Here only the maximal groups, instead of every subgroup, are examined in the objective function; otherwise, duplicated social utilities will be summed up because multiple overlapping subgroups are contained in maximal groups.}, i.e., user $u$ sees item $c$ at slot $s$ with every user in $\mathcal{V}$, and \textit{no friend} of $u$ outside $\mathcal{V}$ also sees $c$ at slot $s$. Thus new objective of \prob\ is generalized as follows.

$$ \sum\limits_{u \in V} \sum\limits_{s=1}^{k} [\text{p}(u, \mathbf{A}^{\ast}(u,s)) + \sum\limits_{\mathcal{V} | u \xleftrightarrow[s]{c} \mathcal{V}} \tau(u,\mathcal{V},\mathbf{A}^{\ast}(u,s))].$$

%Here we note that if $u \xleftrightarrow[s]{c} \mathcal{V}$ is defined only as representing \textit{group} co-display, i.e., that user $u$ sees item $c$ together at slot $s$ with every user in $\mathcal{V}$, but without the maximal criteria, the formulation would be inaccurate since the objective would thus be over-estimating the benefit by aggregating the benefits for every subgroup $\mathcal{V}'$ of the maximal group $\mathcal{V}$. 
%To address this issue, the appropriate way is to instead letting the notation $u \xleftrightarrow[s]{c} \mathcal{V}$ denote  It is then appropriate to formulate the objective as the equation above.
% \begin{small}
% $$ \sum\limits_{u \in V} \sum\limits_{s=1}^{k} [\text{p}(u, \mathbf{A}^{\ast}(u,s)) + \sum\limits_{\mathcal{V} | u \xleftrightarrow[s]{\mathbf{A}^{\ast}(u,s)} v} \tau(u,\mathcal{V},\mathbf{A}^{\ast}(u,s))]. $$
% \end{small}

\para{Algorithm Extension for Scenarios A--D.} 
\noindent In the following, we first introduce a new ILP formulation to support the above practical scenarios. Decision variable $x^c_{u,s}$ now indicates whether user $u$ views item $c$ \textit{in the primary view} at slot $s$. On the other hand, let decision variable $w^c_{u,s}$ denote whether $u$ can see $c$ \textit{in some view}, i.e., in the primary view or a group view, at slot $s$. Therefore, $x^c_{u,s} = 1$ implies $w^c_{u,s} = 1$. To consider the layout slot significance, let $w^c_u = \sum\limits_{s=1}^{k} \gamma_s \cdot w^c_{u,s}$ be the weighted sum of all $w$ decision variables, and here $w^c_u$ is not required to be binary. Therefore, $w^c_u$ represents the total significance of the assigned slots for $u$ to view $c$. To capture maximal co-display, for all subgroups of users $\mathcal{V} \subseteq V$, let $y^c_{u,\mathcal{V},s}$ now indicate the \textit{maximal group} co-display. In other words, $u \xleftrightarrow[s]{c} \mathcal{V}$ if and only if $y^c_{u,\mathcal{V},s} = 1$. Analogously, let $y^c_{u,\mathcal{V}}$ be the weighted sum of $y^c_{u,\mathcal{V},s}$. The new objective function is as follows.

%Unaligned co-display is obsolete and has been re-termed indirect display in SVGIC-ST
%Also, to support unaligned co-display, for $e = (u,v)$, let $z^c_{e,s,s'}$ indicate whether $u$ and $v$ are co-displayed item $c$ at slots $s$ and $s'$. Let $z^c_{e} = \sum_{s=1}^{k} \sum_{s'=1}^{k} (\zeta(s,s') \cdot z^c_{e,s,s'})$ be the total social benefit of (aligned or unaligned) co-displaying item $c$ to $u$ and $v$ among all slots. 

\small
\begin{align*}
\text{max} \quad \sum\limits_{c \in \mathcal{C}} \omega_c \cdot [\sum\limits_{u \in V} \big( \text{p}(u, c) \cdot w^c_u + \sum\limits_{\mathcal{V} \subseteq V} ( \tau(u,\mathcal{V},c) \cdot y^c_{u,\mathcal{V}}) \big)] %\\ + \sum\limits_{u\neq v \in V} ( \tau(u,v,c) \cdot z^c_{u,v}))
\end{align*}
\normalsize

subject to the constraints,
\footnotesize
\begin{align}
    \sum_{c \in \mathcal{C}} x^c_{u,s} = 1, \quad & \forall u \in V, s = 1 ... k \label{ilp_ext:one_slot_one_default_item}\\
    \sum_{c \in \mathcal{C}} w^c_{u,s} \leq \beta, \quad & \forall u \in V, s = 1 ... k \label{ilp_ext:one_slot_many_item}\\
    x^c_{u,s} \leq w^c_{u,s}, \quad & \forall u \in V, s = 1 ... k, c \in \mathcal{C} \label{ilp_ext:default_item_can_see} \\
    \sum_{s=1}^{k} x^c_{u,s} \leq 1, \quad & \forall u \in V, c \in \mathcal{C} \label{ilp_ext:no_replicated_item}\\
    x^c_u = \sum_{s=1}^{k} (\gamma_s \cdot x^c_{u,s}), \quad & \forall u \in V, c \in \mathcal{C} \label{ilp_ext:user_recommended}\\
    y^c_{\mathcal{V}} = \sum_{s=1}^{k} (\gamma_p \cdot y^c_{\mathcal{V},s}), \quad & \forall \mathcal{V} \subseteq V, c \in \mathcal{C} \label{ilp_ext:group_recommended}\\
    %z^c_{e} = \sum_{s=1}^{k} \sum_{s'=1}^{k} (\zeta(s,s') \cdot z^c_{e,s,s'}), \quad & \forall e = (u,v) \in E, s,s' \in 1 ... k, s \neq s', c \in \mathcal{C} \label{ilp_ext:unaligned_recommended} \\
    y^c_{\mathcal{V},s} \leq x^c_{u,s}, \quad & \forall u \in \mathcal{V}, s = 1 ... k, c \in \mathcal{C} \label{ilp_ext:direct_relation_1} \\
    y^c_{\mathcal{V},s} + x^c_{u,s} \leq 1, \quad & \forall u \notin \mathcal{V}, s = 1 ... k, c \in \mathcal{C} \label{ilp_ext:direct_relation_2} \\
    %z^c_{e,s,s'} \leq x^c_{u,s}, \quad & \forall e = (u,v) \in E, s \neq s' \in 1 ... k, c \in \mathcal{C} \label{ilp_ext:unaligned_1} \\
    %z^c_{e,s,s'} \leq x^c_{v,s'}, \quad & \forall e = (u,v) \in E, s \neq s' \in 1 ... k, c \in \mathcal{C} \label{ilp_ext:unaligned_2} \\
    x^c_{u,s}, y^c_{\mathcal{V},s} \in \{ 0,1 \}, \quad & \forall u \in V, e \in E, s,s' \in 1 ... k, c \in \mathcal{C} \label{ilp_ext:integrality}.%, z^c_{e,s,s'}
\end{align}

\normalsize
Constraint \ref{ilp_ext:one_slot_one_default_item} guarantees that a user is displayed exactly one default item (for the primary view) at each slot. Constraint \ref{ilp_ext:one_slot_many_item} ensures that at most $\beta$ items can be viewed at one slot in MVD. Constraint \ref{ilp_ext:default_item_can_see} states that the default item can be viewed in the MVD, i.e., if $c$ is displayed ($x^c_{u,s} = 1$), then $w^c_{u,s}$ will become 1. Constraint \ref{ilp_ext:no_replicated_item} guarantees that the default displayed items for each user do not replicate. Constraint \ref{ilp_ext:user_recommended} ensures that $x^c_u$ (significance of the slot where $u$ is displayed $c$) is the weighted sum of $x^c_{u,s}$. Similarly, constraints \ref{ilp_ext:group_recommended} 
%and \ref{ilp_ext:unaligned_recommended} 
state that $y^c_{\mathcal{V}}$
%and $z^c_{e}$ are 
is the weighted sum of $y^c_{\mathcal{V},s})$ (on the slot significance)
%and $z^c_{e,s,s'}$ (on the social benefit factor). 
Constraints \ref{ilp_ext:direct_relation_1} and \ref{ilp_ext:direct_relation_2} specify the maximal co-display. Constraint \ref{ilp_ext:direct_relation_1} states that $y^c_{\mathcal{V},s}=1$ only if every $x^c_{u,s}=1$, implying that $c$ is displayed to every $u$ in $\mathcal{V}$ at slot $s$. When $y^c_{\mathcal{V},s}=1$, constraint \ref{ilp_ext:direct_relation_2} ensures no other $x^c_{u,s}$ is 1 for $u$ outside of $\mathcal{V}$, so that $\mathcal{V}$ is indeed the maximal set. %Constraints \ref{ilp_ext:unaligned_1} and \ref{ilp_ext:unaligned_2} consider the unaligned co-display. When $z^c_{e,s,s'}=1$, both $x^c_{u,s}=1$ and $x^c_{v,s'}=1$ hold, i.e., $u$ sees $c$ at slot $s$, and $v$ views $c$ at slot $s'$. 
Finally, constraint \ref{ilp_ext:integrality} ensures the decision variables to be binary, i.e., $\in \{0,1\}$.

The LP relaxation of the above formulation also relaxes the last constraint, so that binary decision variables $x^c_{u,s}, y^c_{\mathcal{V},s}$ becomes real number in $[0,1]$. The other two phases of \algor\ and \algod\ remain unchanged. The commodity value $\omega_c$ and the layout slot significance $\gamma_s$ will not affect the theoretical guarantee of \algor\ and \algod\ because the original proof can be modified by replacing the preference utility and social utility values with weighted versions. Furthermore, in any iteration $t$ in \algo, for any subgroup of users $\mathcal{V}$ with all users $u \in \mathcal{V}$ eligible for $(c,s)$, as the maximal co-displayed subgroups contain at most $(\max|\mathcal{V}|)$ users, Lemma \ref{lemma:ratio} can be analogously modified to upper bound the probability that \textit{at least one} user in $\mathcal{V}$ is not eligible for $(c,s)$ in iteration $(t+1)$ by summing exactly $2 (\max|\mathcal{V}|)$ summation terms as in the last inequality in the proof of Lemma \ref{lemma:ratio}. Consequently, by following the proof scheme, \algor\ and \algod\ can achieve $2 (\max|\mathcal{V}|)$-approximation. Moreover, the advanced focal parameter sampling scheme can be employed in the above model. 

\para{E. Subgroup Changes.} While the partitions of subgroups in \algo\ enables flexible configurations and facilitates social discussion, drastic subgroup changes between adjacent slots may undermine the smoothness of social interactions and discussions within the group when users are exploring the VE. To address this issue, one approach is to incorporate a constraint on \textit{edit distances} between the partitioned induced subgroups at consecutive slots. Specifically, a pair of friends $u$ and $v$ in the same subgroup (i.e., viewing a common item) at slot $s$ but separated into different subgroups at slot $s+1$ will contribute $1$ to the edit distance between the two slots. To reduce the subgroup changes, IP of the extended \algo\ discourages the intermediate solution (the \fragsol) to introduce large subgroup changes by constraining the total edit distances across all consecuetive slots (or adjacent slots, if the slots are additionally formulated as spatial projects) in the \configuration. In the rounding scheme, \algo\ examines the potential outcomes before co-displaying a \roundingitem\ to the target subgroup. It voids the current iteration and re-sample another set of pivot parameters, if the solution incurs a large subgroup change. Finally, after the complete \configuration\ is constructed, \algo\ can facilitate a local search by exchanging the sub-configuration at different slots to reduce the total subgroup change.

\para{F. Dynamic Scenario.} To support the dynamic join and leave of users with different walking speeds, executing the whole \algo\ for every dynamic event is computationally intensive. Therefore, one approach is to first solve the relaxed LP for the partial \prob\ instance with the new setting, whereas the majority of \weight s remain the same (temporarily regarded as constants in LP), so that the \weight s are updated efficiently. \stagethree\ then assigns new users to existing target subgroups according to their \weight s, and it also invokes local search to examine the potential profit from exchanging users among existing target subgroups. Moreover, similar to in \probtwo, \textit{teleportation} in VR enables a user to move directly to her friends at a different slot. Therefore, when two users are co-displayed an item (directly or indirectly) but are far apart from each other in the store, the shopping application could suggest one of them to teleport to the other's location.
}

==> stash/sec6_exp.tex <==
\section{Experiments} \label{sec:exp}
In this section, we evaluate the proposed \algor\ and \algod\ along with various baseline algorithms on three real datasets. \opt{short}{We also build a prototype of a VR store with Unity and SteamVR to conduct a user study.}\opt{full}{Moreover, a case study on the real dataset is provided to demonstrate the characteristics of solutions derived from different approaches. Finally, we build a prototype of a VR store with Unity and SteamVR to conduct a user study.}

\subsection{Experiment Setup and Evaluation Plan} \label{subsec:setup}
\para{Datasets.} To evaluate the proposed algorithms, three real datasets are tested in the experiment. The first dataset \textit{Timik} \cite{Timik} is a 3D VR social network containing 850k vertices (users) and 12M edges (friendships) with 12M check-in histories of 849k virtual Point-of-Interests (POIs). The second dataset, \textit{Epinions}\cite{Epinions}, is a website containing the reviews of 139K products and a social trust network with 132K users and 841K edges. The third dataset, \textit{Yelp} \cite{Yelp}, is a location-based social network (LBSN) containing 1.5M vertices, 10M edges, and 6M check-ins. For Timik and Yelp, we follow the settings in \cite{CYS18,AG19,CC17} to treat POIs in the above datasets as the candidate items in \prob. The preference utility and social utility values are learned by the PIERT learning framework \cite{YL18TOIS} which jointly models the social influence between users and the latent topics of items. Following the scales of the experiments in previous research \cite{SD17,SBR15}, the default number of slots $k$, the default number of items $m$, and the default size of user set $n$ selected from the social networks to visit a VR store are set as 50, 10000, and 125, respectively.%\footnote{Note that a small-to-medium scale value of $n$ is practical for VR applications, e.g., VRChat \cite{VRChat} allows at most 16 users, and IrisVR \cite{IrisVR} allows up to 12 users.}

\para{Baseline Methods.} We compare \algor\ and \algod\ with five baseline algorithms: Personalized Top-$k$ (PER), Fairness Maximization in Group recommendation (FMG) \cite{SD17}, Social-aware Diverse and Preference selection (SDP) \cite{CYS18}, Group Recommendation and Formation (GRF) \cite{SBR15}, and Integer Programming (IP). PER and FMG correspond to the two baseline approaches outlined in Section \ref{sec:intro}. Specifically, PER retrieves the top-$k$ preferred items for each user (the \personalized\ approach), while FMG selects a bundled itemset for all users as a group (the \group\ approach) with considerations of fairness of preference among the users. SDP selects socially-tight subgroups to display their preferred items, which corresponds to the subgroup approach outlined in Section \ref{sec:algo}. GRF splits the input users into subgroups with similar item preferences without considering the social network topology, which can be viewed as a variation of the subgroup approach where the subgroups are partitioned based on preferences instead of social connections. Finally, IP is the integer program formulated in Section \ref{subsec:hardness_ip} that finds the optimal solutions of small \prob\ instances by Gurobi \cite{Gurobi}. All algorithms are implemented in an HP DL580 Gen 9 server with four 3.0 GHz Intel CPUs and 1TB RAM. Each result is averaged over 50 samples. \opt{short}{The datasets and algorithms used are released as a public download in \cite{OnlineRepo}.}

\para{Evaluation Metrics.} To evaluate the algorithms considered for \prob\ and analyze the returned \configuration s, we introduce the following metrics: 1) total \scenario\ utility achieved, 2) total execution time (in seconds), 3) the percentages of personal preference utility (\textit{Personal\%}) and social utility (\textit{Social\%}) in total \scenario\ utility, 4) the percentage of \textit{Inter}-subgroup edges (\textit{Inter\%}) and \textit{Intra}-subgroup edges (\textit{Intra\%}) in the returned partition of subgroups, 5) the average network density among partitioned subgroups, normalized by the average density of the original social network, 6) the percentage of friend pairs viewing common items together (\textit{Co-display\%}), 7) the percentage of users viewing items alone (\textit{Alone\%}), and 8) \textit{regret ratio} \revise{(a fairness measure detailed later in Section \ref{subsec:group_formation_exp}.)} \opt{full}{Moreover, for evaluating the performance of all methods in \probtwo, we measure 9) \textit{feasibility ratio}: the number of feasible solutions divided by the total number of instances, and 10) \textit{group size constraint violation}: the number of partitioned subgroups exceeding the predefined size constraint.}

\revise{
\para{Evaluation Plan.} To evaluate the performance of the above algorithms, \opt{full}{in Section \ref{subsec:small_exp}, }we use IP to derive the optimal total \scenario\ utility on small datasets.\footnote{Since solving IP is $\mathsf{NP}$-hard, Gurobi cannot solve large instances within hours.} The social networks and items in the small datasets are respectively sampled by random walk and uniform sampling from Timik according to the setting of \cite{AN15VLDB}.\opt{short}{ Due to the space constraint, please see Section \textbf{6.2} in the full version \cite{Online} for the experimental results on small datasets.} Next, in Section \ref{subsec:large_exp_sensitivity}\opt{short}{ (Section \textbf{6.3} in \cite{Online})}, we evaluate the efficacy of \algor\ and \algod\ in large datasets with input scales following previous research \cite{SD17,SBR15}, and also conduct experiments on different inputs generated by PIERT~\cite{YL18TOIS} (default), AGREE, and GREE~\cite{DC18}. We examine the efficiency of all algorithms, including various configurations of mixed integer programming (MIP) algorithms, in Section \ref{subsec:large_exp_scalability}\opt{short}{ (Section \textbf{6.4} in \cite{Online})}. We then compare the algorithms on the aforementioned group formation-related metrics, which are independent to the objective of this paper, in Section \ref{subsec:group_formation_exp}\opt{short}{ (Section \textbf{6.5} in \cite{Online})}. A case study on a 2-hop ego network in Yelp is shown in \opt{full}{Section \ref{subsec:case_study}}\opt{short}{Section \textbf{6.6} in \cite{Online}} to examine the subgroup partition patterns in different algorithms. Section \opt{full}{\ref{subsec:diff_r}}\opt{short}{\textbf{6.7} in \cite{Online}} conducts a sensitivity test on $r$, an important algorithmic parameter of the deterministic \algod\ algorithm, and Section \opt{full}{\ref{subsec:subgroup_constraint}}\opt{short}{\textbf{6.8} in \cite{Online}} provides experimental results on the \probtwo\ problem. Finally, we build a prototype of VR store with Unity 2017.1.1.1 (64bit), Photon Unity Network free 1.86, SteamVR Plugin 1.2.2, VRTK, and 3ds Max 2016 for hTC VIVE HMD to validate the proposed objective in modelling \prob. We detail the user study in Section \ref{sec:user_study}\opt{short}{ (Section \textbf{6.9} in \cite{Online})}.
}

%user study description
%\para{User Study.} Finally,  

% \opt{short}{%%%4 figures (obj:n,k, time:n,m)
% 	\subfigure[][\centering Total \scenario\ utility \newline vs. size of user set ($n$).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_obj_n.pdf}
% 		\label{fig:small_obj_n} }
% 	\subfigure[][\centering Total \scenario\ utility \newline vs. number of slots ($k$).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_obj_k.pdf}
% 		\label{fig:small_obj_k} }
% 	\subfigure[][\centering Execution time vs. \newline size of user set ($n$).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_time_n_colored.pdf}
% 		\label{fig:small_time_n} }
% 	\subfigure[][\centering Execution time vs. \newline size of item set ($m$).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_time_m_colored.pdf}
% 		\label{fig:small_time_m} }
% }
\opt{full}{%%%6 figures
\begin{figure}[t]
	\centering
	\subfigure[][\centering Total \scenario\ utility \newline vs. size of user set ($n$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_obj_n.pdf}
		\label{fig:small_obj_n} } 
	\subfigure[][\centering Execution time vs. \newline size of user set ($n$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_time_n_colored.pdf}
		\label{fig:small_time_n} }
	\subfigure[][\centering Total \scenario\ utility \newline vs. size of item set ($m$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_obj_m.pdf}
		\label{fig:small_obj_m} } 
	\subfigure[][\centering Execution time vs. \newline size of item set ($m$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_time_m_colored.pdf}
		\label{fig:small_time_m} }		
	\subfigure[][\centering Total \scenario\ utility \newline vs. number of slots ($k$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_obj_k.pdf}
		\label{fig:small_obj_k} } 
	\subfigure[][\centering Execution time vs. \newline number of slots ($k$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/small_scale/small_time_k_colored.pdf}
		\label{fig:small_time_k} } 
	\caption{Comparisons on small datasets.}
	\label{exp:small_exp}
\end{figure}
}

\opt{full}{
\subsection{Comparisons on Small Datasets}
\label{subsec:small_exp}

%To evaluate the performance of the above algorithms, we use IP to derive the optimal total \scenario\ utility on small datasets.\footnote{Since solving IP is $\mathsf{NP}$-hard, Gurobi cannot solve large instances within hours.} The social networks and items in the small datasets are respectively sampled by random walk and uniform sampling from Timik according to the setting of \cite{AN15VLDB}. %the above moved from evaluation plan
Figure \ref{fig:small_obj_n} manifests that \algor\ and \algod\ outperform the other approaches regarding the total \scenario\ utility for different $n$ (i.e., the size of user set). Solutions of \algod\ are close to optimal since \algod\ extracts the target subgroups by jointly optimizing the current and expected future total \scenario\ utility in each iteration. \algod\ outperforms other baselines by at least 50.8\% to 62.8\% as $n$ grows, because the social interactions on extracted target subgroups become increasingly important when the size of user set increases. In contrast, the values of total \scenario\ utility of PER grows slowly because it is not designed to cope with the interplay and trade-off between personal preferences and social interactions. Moreover, while FMG and GRF seem to benefit from large values of $n$, their solution qualities are still limited due to the fixed partition of subgroups generated without leveraging CID.

\begin{figure}[tp]
  \centering \includegraphics[width = 0.95\columnwidth]{fig/small_scale/small_obj_lambda.pdf}
  \caption{Normalized total \scenario\ utility of diff. $\lambda$.}
  \label{fig:small_obj_lambda}
\end{figure}

\opt{full}{Figure \ref{fig:small_obj_m} presents the total \scenario\ utility under varied numbers of items ($m$). However, $m$ does not seem to affect the total \scenario\ utility by much since any user's top preferred items are already contained in the top-100 items.} Moreover, Figure \ref{fig:small_obj_k} presents the total \scenario\ utility under varied number of slots ($k$). \algod\ and \algor\ significantly outperform the baselines by at least 134.7\% and 102.1\% in terms of the total \scenario\ utility when $k$ grows to 20, because \stagethree\ leverages the flexibility provided by \notion\ to optimize the social utility for different slots, which is beneficial for a large $k$ as it becomes difficult to find more commonly interested items for static subgroup members. \opt{short}{The values of total \scenario\ utility with regard to different numbers of items ($m$) are almost the same when $n$ and $k$ are fixed (please refer to \cite{Online} due to space constraint).} \opt{short}{Figures \ref{fig:small_time_n} and \ref{fig:small_time_m} show the execution time by varying the size of user set ($n$) and the size of item set ($m$).}\opt{full}{Figures \ref{fig:small_time_n}, \ref{fig:small_time_m} and \ref{fig:small_time_k} show the execution time by varying the size of user set ($n$), the size of item set ($m$), and the number of slots ($k$).} The running times of \algor\ and \algod\ are at most 7.5\% and 17.4\% of that of IP. \algor\ and \algod\ require slightly more time than PER, GRF, and FMG, since the baseline approaches focus only on one of preference utility, social utility, or subgroup partition, instead of considering all of them jointly. Figure \ref{fig:small_obj_lambda} evaluates the impact of $\lambda$ on the total \scenario\ utility of all schemes normalized by that of IP. The normalized total \scenario\ utilities of FMG and SDP improve when the social utility becomes more important as $\lambda$ grows. However, it is difficult for them to address the diverse personal preferences. In contrast, PER achieves the highest preference utility and the lowest social utility, but tends to generate a small total \scenario\ utility. 
}

\subsection{Sensitivity Tests on Large Datasets}
\label{subsec:large_exp_sensitivity}
\begin{figure}[tp]
  \centering \includegraphics[width = 0.95\columnwidth]{fig/large_scale/timik_obj_n_large_withIP.pdf}
  \caption{Total \scenario\ utility vs. size of user set ($n$).}
  \label{fig:timik_obj_n}
\end{figure}
\begin{figure}[tp]
  \centering \includegraphics[width = 0.95\columnwidth]{fig/large_scale/dataset_obj_n_withIP.pdf}
  \caption{Total \scenario\ utility in diff. datasets.}
  \label{fig:dataset_obj}
\end{figure}
\begin{figure}[tp]
  \centering \includegraphics[width = 0.95\columnwidth]{fig/large_scale/timik_input.pdf}
  \caption{Total \scenario\ utility vs. different input.}
  \label{fig:timik_input}
\end{figure}

We evaluate the efficiency and efficacy of \algor\ and \algod\ in large datasets with the scales of the three dimensions following previous research \cite{SD17,SBR15}, i.e., $m=10000$, $k=50$, and $n=125$. %the above moved from evaluation plan
Figure \ref{fig:timik_obj_n} presents the total \scenario\ utility by varying the sizes of user set in Timik. The results manifest that \algor\ and \algod\ outperform all baselines by at least 30.1\%, while \algod\ is slightly better than \algor\ since it selects better pivot parameters for \stagethree. \revise{Moreover, the returned objective of \algor\ and \algod\ respectively achieve at least 93.7\% and 96.4\% of it of IP, manifesting that our algorithms are effective.} Compared with GRF, the improvement of \algod\ grows from 43.6\% to 54.6\% as $n$ increases, since GRF splits the users into subgroups without considering social relations, but social interactions among \emph{close friends} become more important for a larger group. By striking a balance between preference and social utility, \algor\ and \algod\ achieve a greater total \scenario\ utility. Compared with PER and GRF, FMG achieves a higher social utility but a lower preference utility because it displays a universal configuration to all users.

Figure \ref{fig:dataset_obj} compares the results on Timik, Yelp, and Epinions. The social utility obtained in Epinions is lower than in Yelp due to the sparser social relations in the review network, and group consensus thereby plays a more important role in Yelp. %Timik users can access virtual POIs easily with or without friends, and both personal preferences and social interactions are very important in the VR applications. 
Despite the different characteristics of datasets, \algor\ and \algod\ prevail in all datasets and outperform all baselines since \stagethree\ operates on the \weight s from the optimal LP solution, which does strike a good balance among all factors. FMG and SDP benefit from the high social utility in Yelp and outperform PER. By contrast, PER performs nearly as good as FMG and SDP in Epinions since the social utility is lower. %Note that PER concerns only the personal preferences but still obtains a small social utility in Foursquare, because popular locations are usually selected by PER when they are preferable to many users. 

\revise{Next, to examine the influence of input models on the tackled problem, Figure \ref{fig:timik_input} shows the experimental results on different inputs generated by PIERT~\cite{YL18TOIS} (default), AGREE, and GREE~\cite{DC18}. PIERT jointly learns preference and social utility by modeling the social influence between users and the latent topics of items. GREE and AGREE also learn the two utilities jointly \cite{DC18}, while the former assumes the social influence between users is equal and the later learns sophisticated weights of the triple (user, user, item). \algo\ and \algod\ outperform the baselines with regards to all different input models, manifesting that our method is generic to different distributions of inputs. Note that the social utilities returned by \algor\ and \algod\ with PIERT and AGREE are slightly greater than the ones with GREE. The result manifests that \algor\ and \algod\ can select better items for users to enjoy if social utilities are different across items.}

\subsection{Scalability Tests on Large Datasets}
\label{subsec:large_exp_scalability}
\begin{figure}[tp]
	\centering
	\subfigure[b][\centering Execution time vs. \newline size of user set ($n$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/large_scale/timik_time_n_colored.pdf}
		\label{fig:timik_time_n} } 
	\subfigure[b][\centering Execution time vs. \newline size of item set ($m$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/large_scale/timik_time_m_colored.pdf}
		\label{fig:timik_time_m} }
	\caption{Execution time in Yelp.}
	\label{fig:large_scalability}
\end{figure}
\begin{figure}[tp]
  \centering \includegraphics[width = 0.48\columnwidth]{fig/large_scale/timik_IP_tradeoff.pdf}
  \caption{Efficiency and efficacy of different IP heuristics.}
  \label{fig:timik_IP_tradeoff}
\end{figure}

Figure \ref{fig:timik_time_n} presents the execution time in Yelp with different $n$. IP cannot terminate within 24 hours when $n \geq 25$, and SDP needs 300 seconds to return a solution even when $n=5$. Figure \ref{fig:timik_time_m} shows the execution time with different $m$. Note that \algor\ and \algod\ are both more scalable to $m$ than the baseline approaches because \stagethree\ exploits the \fragsol\ without $m$ in the complexity. Although \algod\ provides a stronger theoretical guarantee, the scalability of \algor\ on $n$ is better than \algod\ because \algor\ samples the target subgroups randomly. However, practical VR applications, e.g., VRChat \cite{VRChat} and IrisVR \cite{IrisVR}, seldom have $n > 25$. \delete{Moreover, recall that the SVGIC problem simultaneously explores three dimensions: $n$ (the size of user set), $m$ (the size of item set), and $k$ (the number of slots). Therefore, forming the subgroups and configuring the items in SVGIC is combinatorially harder than traditional optimization problems in group recommendation %\cite{SBR15, SD17} 
or group formation.} %\cite{CYS16TKDD, CYS16TKDE}.

\revise{To examine the performances of different mixed integer programming (MIP) algorithms, we further conducted experiments with Primal-first Mixed Integer Programming (IP-Primal), Dual-first Mixed Integer Programming (IP-Dual), Concurrent Mixed Integer Programming (IP-C), Deterministic Concurrent Mixed Integer Programming (IP-DC), and the Barrier Algorithm (IP-Barrier) in the Gurobi \cite{Gurobi} package. Figure \ref{fig:timik_IP_tradeoff} shows the tradeoff between efficiency and efficacy of five different IP algorithms on the Timik dataset with the default parameters ($(k,m,n) = (50,10000,125)$). For every MIP algorithm, we evaluate the solution quality of different algorithms with the running time constrained by 200, 1000 and 5000 times the running time of our proposed \algod\ algorithm for solving the same instance. Note that none of the examined algorithms returns any feasible solution within 100 times the running time of \algod. The y-axis shows the relative objective value normalized by the solution found by \algod, which manifests none of the 5 baselines achieve any solution better than that of \algod\ in 5000X of the running time of \algod. As such, although there is some subtle difference in performance across different MIP algorithms, none of the examined algorithms shows a reasonable scalability.}

\opt{short}{%% short version (4 figures)
\begin{figure}[tb]
	\centering
	\subfigure[][\centering Inter/Intra\% and subgroup density (Timik).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/timik_density.pdf}
		\label{fig:timik_inter_intra_density} }
	\subfigure[][\centering Inter/Intra\% and subgroup density (Epinions).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/ep_density.pdf}
		\label{fig:ep_inter_intra_density} }
		
	\subfigure[][\centering CDF of Regret ratio (Timik).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/timik_regret.pdf}
		\label{fig:timik_regret} } 
	\subfigure[][\centering CDF of Regret ratio (Epinions).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/ep_regret.pdf}
		\label{fig:ep_regret} }
		
% 	\subfigure[][\centering Inter/Intra\% and subgroup density (Yelp).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/yelp_density.pdf}
% 		\label{fig:yelp_inter_intra_density} } 
% 	\subfigure[][\centering CDF of Regret ratio (Yelp).] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/yelp_regret.pdf}
% 		\label{fig:yelp_regret} } 
	\caption{Comparisons on subgroup metrics.}
	\label{exp:group_all}
\end{figure}
}

%% full version (9 figures)
\opt{full}{	
\begin{figure*}[tb]
	\centering
	\subfigure[][\centering Inter/Intra\% and subgroup density (Timik).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/timik_density.pdf}
		\label{fig:timik_inter_intra_density} } 
	\subfigure[][\centering Inter/Intra\% and subgroup density (Epinions).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/ep_density.pdf}
		\label{fig:ep_inter_intra_density} }
	\subfigure[][\centering Inter/Intra\% and subgroup density (Yelp).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/yelp_density.pdf}
		\label{fig:yelp_inter_intra_density} } 

	\subfigure[][\centering Share rate and alone rate (Timik).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/timik_share_alone.pdf}
		\label{fig:timik_share_alone} } 
	\subfigure[][\centering Share rate and alone rate (Epinions).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/ep_share_alone.pdf}
		\label{fig:ep_share_alone} }
	\subfigure[][\centering Share rate and alone rate (Yelp).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/yelp_share_alone.pdf}
		\label{fig:yelp_share_alone} }
	
	\subfigure[][\centering Regret ratio (Timik).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/timik_regret.pdf}
		\label{fig:timik_regret} } 
	\subfigure[][\centering Regret ratio (Epinions).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/ep_regret.pdf}
		\label{fig:ep_regret} }
	\subfigure[][\centering Regret ratio (Yelp).] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/subgroup_metrics/yelp_regret.pdf}
		\label{fig:yelp_regret} } 
	\caption{Comparisons on subgroup metrics.}
	\label{exp:group_all}
\end{figure*}
}

\subsection{Comparisons on Subgroup Metrics}
\label{subsec:group_formation_exp}

\opt{short}{ %short version (4 figures)
In the following, we analyze the subgroups in the \configuration s returned from all algorithms in terms of subgroup-related metrics. Figures \ref{fig:timik_inter_intra_density} and \ref{fig:ep_inter_intra_density} compare the ratios of Inter-/Intra-subgroup edges averaged across all slots in the \configuration s in the Timik and Epinions datasets, respectively. It also shows the average network density among the partitioned subgroups normalized by the original density of the input social network. The results from all datasets indicate that the majority of preserved edges by \algo\ are within the same subgroups (large Intra\%). FMG achieves 100\% in Intra\%, 0\% in Inter\%, and 1 in normalized density because it consistently views the whole network as a large subgroup. In contrast, PER has a high Inter\% as it separates most users into independent subgroups to display their favorite items. There exist a small subset of widely liked or adopted items in Epinions that appear as most users' favorite (hence the small nonzero Intra\% of PER), while famous VR locations (e.g., transportation hubs in VR world of Timik) are inclined to be associated with high preference utilities by the exploited recommendation learning models as they generate a lot of check-ins among all users. Therefore, they have a higher chance to be co-displayed by PER. Among all methods, \algo\ achieves the largest normalized density as \stagethree\ carefully considers the \weight s to partition the network into dense communities. 

\revise{Figures \ref{fig:timik_regret} and \ref{fig:ep_regret} report the Cumulative Distribution Function (CDF) of \textit{regret ratios} of all algorithms in the Timik and Epinions datasets. The regret ratio reg$(u)$ \cite{KL14KDD} is a game-theory based measurement for satisfaction of individual users and the overall \textit{fairness} of the solution. For each user $u$, the regret ratio reg$(u)$, and its converse, \textit{happiness} ratio $\text{hap}(u)$, are defined as
\vskip -0.15in
$$\text{reg}(u) \equiv 1 - \text{hap}(u), \quad \text{hap}(u) \equiv \frac{\sum\limits_{c \in \mathbf{A}^{\ast}(u,\cdot)} \text{w}_{\textbf{A}}(u,c)}{\max\limits_{\mathcal{C}_u} \sum\limits_{c \in \mathcal{C}_u} \Bar{\text{w}}_{\textbf{A}}(u,c)}$$
\noindent where the numerator in $\text{hap}(u)$ is the achieved \scenario\ utility, the denominator with $\Bar{\text{w}}_{\textbf{A}}(u,c) = (1-\lambda)\cdot\text{p}(u,c) + \lambda\cdot\sum_{v \in V} \tau(u,v,c)$ is an \textit{upper bound} of possible \scenario\ utility when all users view $c$ together with user $u$, and $\mathcal{C}_u$ is a $k$-itemset, corresponding to a very optimistic scenario favoring $u$ the most. Note that the second term of $\Bar{\text{w}}_{\textbf{A}}(u,c)$ is different from $\text{w}_{\textbf{A}}(u,c)$ in Definition \ref{def:savg_utility}. In other words, the upper bound is the \scenario\ utility of $u$ if she dictates the whole \configuration\ selfishly. Therefore, a high $\text{hap}(u)$ (equivalently, a low reg$(u)$) implies that user $u$ is relatively satisfied with the \configuration, and \textit{fairness} among the users can be observed by inspecting the distribution of regret ratio in the final configurations.}


\algor\ and \algod\ consistently have the lowest regret ratios. Among the other approaches, PER incurs the highest regret ratios for users in all datasets, since it does not foster social interactions in shared views. Consistent with the performances on \scenario\ utility, FMG and SDP outperform PER and GRF in the Timik dataset, but their performances are comparable in Epinions because the sparser social relations in the review network generates lower social utility. Interestingly, in Timik, some users in GRF are highly satisfied (as the CDF of GRF matches well with that of \algor\ and \algod\ from the beginning) but some others have very high regret ratios (as the CDF dramatically rises near the end). This indicates that a portion of the users in GRF may actually have their preferences sacrificed, i.e., they are forced to share views on uninterested items with other subgroup members. In contrast, FMG and SDP show flatter CDFs, implying the user preferences are more balanced. However, users in FMG and SDP consistently have regret ratios over 20\%, while the regret ratios seldom exceed 20\% in \algor/\algod; this is because the randomly chosen pivot parameters (in \algo) and the deterministically optimized one (in \algod) can effectively form dense subgroups with similar item preferences. More experimental results on subgroup metrics can be found in Section \textbf{6.5} in the full version \cite{Online}.}

\opt{full}{ % full version (9 figures)
In the following, we analyze the subgroups in the \configuration s returned from all algorithms\footnote{Some of the results of \algod\ are omitted as they are similar to \algor.} in terms of subgroup-related metrics. Figures \ref{fig:timik_inter_intra_density}, \ref{fig:ep_inter_intra_density}, and \ref{fig:yelp_inter_intra_density} compare the ratios of Inter-/Intra-subgroup edges averaged across all slots in the \configuration s in the Timik, Yelp, and Epinions datasets, respectively. It also shows the average network density among the partitioned subgroups normalized by the original density of the input social network. The results from all datasets indicate that the majority of preserved edges by \algo\ are within the same subgroups (large Intra\%). FMG achieves 100\% in Intra\%, 0\% in Inter\%, and 1 in normalized density because it consistently views the whole network as a large subgroup. In contrast, PER has a high Inter\% as it separates most users into independent subgroups to display their favorite items. This phenomenon is more obvious in Yelp (with a 100\% Inter\%, i.e., \textit{every} user is left alone as a tiny subgroup) than in Timik (about 30\% of the social edges are Intra-subgroup edges) or Epinions (a nonzero Intra\%). This is because Yelp is a product-review application, where the POIs (restaurants, stores, service centers, etc.) are highly diversified, making it more difficult for different users to have aligned preferences, e.g., user A has her $k$-th favorite POI (indicated by check-in records) identical to user B's $k$-th favorite POI, such that PER happens to co-display the POI to them. On the other hand, there exist a small subset of widely liked or adopted items in Epinions that appear as most users' favorite (hence the small nonzero Intra\% of PER), while famous VR locations (e.g., transportation hubs in VR world of Timik) are inclined to be associated with high preference utilities by the exploited recommendation learning models as they generate a lot of check-ins among all users. Therefore, they have a higher chance to be co-displayed by PER.

Among all methods, \algo\ achieves the largest normalized density as \stagethree\ carefully considers the \weight s to partition the network into dense communities. The normalized density achieved by \algo\ in Yelp is the lowest among the three datasets due to the aforementioned issue of diversified interests but is still higher than all other algorithms. As a result, \algo\ has the most abundant social connections among subgroup members, which usually trigger enthusiastic discussions and purchases. It is worth noting that VR users generally interact with more strangers during the trip, whereas users in traditional LBSN mainly interact with friends in their spatial proximity. Therefore, the local community structures in Timik are less apparent than those of Yelp. As such, despite adopting different partitioning criteria, the average densities of the subgroups retrieved by SDP and GRF do not differ much in Timik.

Figures \ref{fig:timik_share_alone}, \ref{fig:yelp_share_alone}, and \ref{fig:ep_share_alone} illustrate the Co-display\% and Alone\% among the returned \configuration s. As shown, \algo\ has a high Co-display\% near $1.0$ (implying almost all pairs of friends are sharing the views of common items) and a near-zero Alone\% (showing that almost no users are left alone in the configuration) in all datasets. Note that the Co-display\% is based on friend pairs and the Alone\% is calculated based on all users, i.e., they are not complementary statistics (thus do not sum up to 100\%). %As VR users are able to freely explore different POIs, the personal interests towards the POIs are more diverse in Timik than that in Foursquare. Thus, PER achieves a higher Co-display\% in Foursquare than in Timik since spatially close users in LBSNs tend to prefer visiting similar places, enabling more co-displays. 
Although FMG achieves 100\% in Co-display\% and 0\% in Alone\%, it sacrifices the preferences of group members by forming huge subgroups for co-display. On the other hand, both \algo\ and GRF are able to maintain high values of Co-display\% while taking into account the personal preferences. In all datasets, GRF leaves a considerably high portion of users alone because it forms the subgroups according to item preferences. Therefore, some users with unique profiles of interests are more inclined to be left alone. %We revisit this issue in the case study in Section \ref{sec:case_study}. 
The only other method with a higher Alone\% than GRF is PER, which does not facilitate shared views. 

Figures \ref{fig:timik_regret}, \ref{fig:yelp_regret}, and \ref{fig:ep_regret} report the CDF of regret ratios of all algorithms in the the Timik, Yelp, and Epinions datasets. The regret ratio reg$(u)$ \cite{KL14KDD} is a game-theory based measurement for satisfaction of individual users and the overall \textit{fairness} of the solution. For each user $u$, the regret ratio reg$(u)$, and its converse, \textit{happiness} ratio $\text{hap}(u)$, are defined as
$$\text{reg}(u) \equiv 1 - \text{hap}(u), \quad \text{hap}(u) \equiv \frac{\sum\limits_{c \in \mathbf{A}^{\ast}(u,\cdot)} \text{w}_{\textbf{A}}(u,c)}{\max\limits_{\mathcal{C}_u} \sum\limits_{c \in \mathcal{C}_u} \Bar{\text{w}}_{\textbf{A}}(u,c)}$$
\noindent where the numerator in $\text{hap}(u)$ is the achieved \scenario\ utility, the denominator with $\Bar{\text{w}}_{\textbf{A}}(u,c) = (1-\lambda)\cdot\text{p}(u,c) + \lambda\cdot\sum_{v \in V} \tau(u,v,c)$ is an \textit{upper bound} of possible \scenario\ utility when all users view $c$ together with user $u$, and $\mathcal{C}_u$ is a $k$-itemset, corresponding to a very optimistic scenario favoring $u$ the most. Note that the second term of $\Bar{\text{w}}_{\textbf{A}}(u,c)$ is different from $\text{w}_{\textbf{A}}(u,c)$ in Definition \ref{def:savg_utility}. In other words, the upper bound is the \scenario\ utility of $u$ if she dictates the whole \configuration\ selfishly. Therefore, a high $\text{hap}(u)$ (equivalently, a low reg$(u)$) implies that user $u$ is relatively satisfied with the \configuration, and \textit{fairness} among the users can be observed by inspecting the distribution of regret ratio in the final configurations.
\algor\ and \algod\ consistently have the lowest regret ratios. Among the other approaches, PER incurs the highest regret ratios for users in all datasets, since it does not foster social interactions in shared views. Consistent with the performances on \scenario\ utility, FMG and SDP outperform PER and GRF in the Timik and Yelp datasets, but their performances are comparable in Epinions because the sparser social relations in the review network generates lower social utility. Interestingly, in Timik and Yelp, some users in GRF are highly satisfied (as the CDF of GRF matches well with that of \algor\ and \algod\ from the beginning) but some others have very high regret ratios (as the CDF dramatically rises near the end). This indicates that a portion of the users in GRF may actually have their preferences sacrificed, i.e., they are forced to share views on uninterested items with other subgroup members. In contrast, FMG and SDP show flatter CDFs, implying the user preferences are more balanced. However, users in FMG and SDP consistently have regret ratios over 20\%, while the regret ratios seldom exceed 20\% in \algor/\algod; this is because the randomly chosen pivot parameters (in \algo) and the deterministically optimized one (in \algod) can effectively form dense subgroups with similar item preferences. }

%============CASE STUDY================
\opt{full}{
\subsection{A Case Study on Partitioning Subgroups} \label{subsec:case_study}

\begin{figure*}[tp]
  \centering \includegraphics[width = 0.95\textwidth]{fig/case_study.pdf}
  \caption{Illustration of subgroup partitioning approaches.}
  \label{fig:case_study}
\end{figure*}

Figure \ref{fig:case_study} depicts a 2-hop ego network (the subnetwork consisting of all 2-hop friends) of a user A in Yelp and two slots with the highest regret. Note that user A is studied here because she has a unique profile of preference that does not resemble any of her friends (B, E, and F), as shown in the table listing the top-4 POIs of the preference utility for each user. The shaded areas illustrate the partitioned subgroups at the specific slot, while solid and dashed lines depict intra-subgroup and inter-subgroup social edges. The icon beside each subgroup represents the selected POI (displayed item). 

As indicated in the table, A has a unique profile of preference that does not resemble any of her friends B, E and F. Therefore, A and her friends are partitioned into distinct subgroups by GRF. On the other hand, \algo\ assigns a baseball field to $\{A,E,F,G\}$ at slot 1, and a bar to $\{A,B,C,D\}$ at slot 2. Therefore, \algo\ is able to capture different interests of A and select proper subgroups of friends for them. However, A is not co-displayed the library with $\{B,C,D\}$ at slot 1 and the beach with $\{E,F,G\}$ at slot 2 because none of the two POIs is in A's favor. On the other hand, SDP partitions the ego-network into three cliques based on the network topology and then assigns a music place and a movie theater to $\{A,B\}$, favoring B's but sacrificing A's interests. Moreover, A is inclined to be dissatisfied for not joining $\{E,F,G\}$ to the baseball field (the third preferred POI) at slot 2. GRF gathers the users with similar interests and leaves A alone, since none of her friends is a big fan of the two restaurants. Therefore, the regret ratios for A are 35.2\% (SDP), 41.2\% (GRF), and 19.6\% (\algo) accordingly. Indeed, this case study manifests that flexible partitions of subgroups are crucial the situations of friends not necessarily sharing similar interests. 
}

%============EXP RESULT OF DIFF R================
\opt{full}{
\subsection{Sensitivity Test of \algod} \label{subsec:diff_r}
\begin{figure}[tp]
	\centering
	\subfigure[][\centering Total \scenario\ utility vs. diff. $r$.] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/derandomize/diff_r_obj.pdf}
		\label{fig:diff_r_obj} } 
	\subfigure[][\centering Execution time vs. diff. $r$.] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/derandomize/diff_r_time.pdf}
		\label{fig:diff_r_time} } 
	\subfigure[][\centering Normalized density vs. diff. $r$.] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/derandomize/diff_r_density.pdf}
		\label{fig:diff_r_density} } 
	\subfigure[][\centering Inter/Intra\% vs. diff. $r$.] {\
		\centering \includegraphics[width = 0.44 \columnwidth]{fig/derandomize/diff_r_inter_intra.pdf}
		\label{fig:diff_r_inter_intra} } 

	\caption{Sensitivity test on $r$ in \algod.}
	\label{fig:diff_r}
\end{figure}
In the following, we investigate the \configuration s found by \algod\ with different values of $r$ in a small sample dataset (such that IP can find the optimal solution as a baseline). Figure \ref{fig:diff_r_obj} shows the total preference utility, social utility and \scenario\ utility in the returned solutions. An interesting observation is that $r = 0.25$ does not achieve the highest total \scenario\ utility among all values. Instead, with $r$ values from 0.7 to 1.0, \algod\ finds very nearly-optimal solutions, where the optimal objective found by IP is indicated by the grey dashed line. This phenomenon can also be found in the behavior of \algod\ in other datasets. However, we note that the result from setting $r = 0.25$ is still promising, achieving an objective of 86.1\% of the optimal, which is consistent to the theoretical guarantee. On the other hand, no theoretical guarantee can be derived with other values of $r$. The results also manifest that the behavior of \algod\ tends to resemble the group approach with small values of $r$ (e.g., \algod\ finds a large subgroup of all users with $r \leq 0.2$) and gradually becomes more alike to the personalized approach as $r$ grows (e.g., the social utility is close to 0 for $r\geq 1.5$, meaning that almost every user is displayed her own favorite items). This is actually consistent to the design of \algod, since 1) a small $r$ essentially ignores the potential future gain in utility from allocating other items than the current \roundingitem, leading to a greedy behavior of always including every eligible user into the targeted subgroup in \stagethree. Consequently, runnning every iteration with $r$ close to 0 finds a large subgroup of all users in every slot; 2) a large $r$ values only the future gain and thereby tends to select very few users into the targeted subgroup. This reluctant behavior in the extreme (consider $r = \infty$) thus leads to subgroups consisting of only one user, essentially simulating the personalized approach. In summary, this again manifests that \algod\ can strike a balance between the suboptimal personalized and group approaches with a good selection of $r$.

Figure \ref{fig:diff_r_time} depicts the execution time of \algod\ with different values of $r$. Intuitively, the more reluctant \algod\ is to include users in the current targeted subgroup, the more iterations are needed before it constructs a complete \configuration. For $n$ users and $k$ slots, the total number of iterations would be $k$ if every targeted subgroup includes all $n$ users but would increase to $kn$ if every iteration displays the \roundingitem\ to only one user. Therefore, $\algod$ has a larger execution time with larger values of $r$. Figures \ref{fig:diff_r_density} and \ref{fig:diff_r_inter_intra} further show the average normalized density and Inter/Intra\% among the subgroups in the solutions of \algod\ with different values of $r$. Consistent to the above discussion, the behavior of \algod\ essentially spans a spectrum from the personalized to the group approach.
}

%============EXP RESULT OF ADVANCED PROBLEM================
\opt{full}{
\begin{figure}[tp]
	\centering
	\subfigure[][\centering Total violation vs. subgroup size constraint (Timik, $n=25$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/general/general_violation_timik25.pdf}
		\label{fig:violation_M_Timik25} } 
	\subfigure[][\centering Total violation vs. subgroup size constraint (Epinions, $n=15$).] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/general/general_violation_ep15.pdf}
		\label{fig:violation_M_Ep15} }
	\caption{Comparisons on \probtwo.}
	\label{exp:subgroup_constraint}
\end{figure}

\begin{figure}[tp]
    \centering
    \includegraphics[width = 0.9 \columnwidth] {fig/general/general_obj_timik15.pdf}
    \caption{Total \scenario\ utility vs. subgroup size constraint (Timik, $n=15$).}
    \label{fig:obj_M_Timik15}
\end{figure}

\begin{figure}[tp]
    \centering
    \includegraphics[width = 0.9 \columnwidth] {fig/general/general_obj_ep15.pdf}
    \caption{Total \scenario\ utility vs. subgroup size constraint (Epinions, $n=15$).}
    \label{fig:obj_M_Ep15}
\end{figure}
% 	\subfigure[][\centering Total \scenario\ utility vs. subgroup size constraint (Timik, $n=15$).] {\
% 		\centering \includegraphics[width = 0.9 \columnwidth] {fig/general/general_obj_timik15.pdf}
% 		\label{fig:obj_M_Timik15} } 
% 	\subfigure[][\centering Total \scenario\ utility vs. subgroup size constraint (Epinions, $n=15$).] {\
% 		\centering \includegraphics[width = 0.9 \columnwidth] {fig/general/general_obj_ep15.pdf}
% 		\label{fig:obj_M_Ep15} } 

\begin{figure}[tp]
	\centering
	\subfigure[][Percentage of diff. $\lambda$.] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/user_lambda.pdf}
		\label{fig:user_lambda} }
% 	\subfigure[][{User anticipation of diff. methods.}] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/user_prob.pdf}
% 		\label{fig:user_prob} }
	\subfigure[][Total \scenario\ utility and user satisfaction.] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/user_obj_satisfaction.pdf}
		\label{fig:user_obj} }
% 	\subfigure[][95\% confidence interval of user satisfaction improvement.] {\
% 		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/user_imp_CI.pdf}
% 		\label{fig:user_sat} }
	\subfigure[][Inter/Intra\% and subgroup density.] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/userstudy_density.pdf}
		\label{fig:user_density} }
	\subfigure[][Co-display rate and alone rate.] {\
		\centering \includegraphics[width = 0.44 \columnwidth] {fig/user_study/userstudy_share_alone.pdf}
		\label{fig:user_share_alone} }
	\caption{Comparisons on user study.}
	\label{exp:user_study}
\end{figure}

\subsection{Experimental Results for \probtwo} \label{subsec:subgroup_constraint}
In the following, we investigate the behavior of all methods in \probtwo, where the default discount factor is 0.5, and the subgroup size constraint $M$ is varied. As none of the baseline algorithms considers the subgroup size constraint, for \probtwo\ with subgroup size constraint $M$, we first pre-partition the user set in to $\lceil \frac{N}{M} \rceil$ subgroups with balanced sizes. The results of all baseline algorithms on the partitioned subproblems are then aggregated into the final returned \configuration\ for them. Figures \ref{fig:violation_M_Timik25} and \ref{fig:violation_M_Ep15} show the total violation of subgroup size constraint (in total number of users) of all methods aggregated over all display slots in a total of 10 sampled instances in Timik (with $n=25$) and Epinions (with $n=15$), respectively. The suffix ``-P'' in the method name represents prepartitioning of the user set into $\lceil \frac{N}{M} \rceil$ subgroups with balanced sizes, and the suffix ``-NP'' indicates no prepartitioning is applied. The results manifest that the pre-partitioning helps decrease the total violation of the subgroup size constraint for all baseline methods except PER because the methods do not take the cap on subgroup sizes into account. \algo\ never violates the constraint since the greedy cutoff in \stagethree\ prevents large targeted subgroups. PER also achieves 100\% feasibility since it does not consider social interactions. Among the baseline methods that consider social interactions, GRF incurs the lowest violation since only it partitions the user set into subgroups based on preference. However, it still has a low feasibility if not used with the pre-partition technique.

Figures \ref{fig:obj_M_Timik15} and \ref{fig:obj_M_Ep15} compares the total \scenario\ utility achieved by all methods \textit{with pre-partitioning} in Timik and Epinions, respectively, with $n=15$ and the subgroup size constraint varies from 3 to 15, where infeasible solutions achieves a total \scenario\ utility of 0. Note that all the baseline methods, except for PER, could still violate the subgroup size constraint even incorporated with the prepartitioning technique. This is because they from time to time display the same item to different pre-partitioned subgroups (or, in the case of GRF, subgroups of them) at the same display slot. \algo\ consistently outperforms all other methods except for the cases where $M$ is very small (3 in Epinions). GRF achieves high total \scenario\ utility in Epinions as it achieves 100\% feasibility and also selects proper distinct and preferred items for separated small subgroups of users in the sparse Epinions network. However, GRF has a surprisingly low feasiblity in Timik (around 20\%), leading to a low total \scenario\ utility. This is because GRF displays the commonly-preferred popular VR locations in Timik to almost all pre-partitioned subgroups at the first few display slots due to its greedy (and thus deterministic) algorithmic behavior in selecting display items for subgroups. Therefore, while its accumulative violation is the lowest (among all methods that possibly violate the constraint), it often finds slightly oversized subgroups at slots 1 and 2, and thereby has a low feasibility.
}

\subsection{User Study} \label{sec:user_study}

For the user study, we recruit 44 participants
%\footnote{The number of user participants is close to the user studies in VR research (e.g., 16 in \cite{VS18}) and conventional group recommendation (e.g., 10 in \cite{SD17} and 50 in \cite{SBR15}).} 
to visit our VR store. Their social networks, preference utility, and $\lambda$ are pre-collected with questionnaires, which follows the setting of \cite{SBR15}, and the social utility is learned by PIERT \cite{YL18TOIS}. A Likert scale questionnaire \cite{likert} is used to find the preference utility of items, where users are allowed to discuss about the products while filling the preference questionnaire so that the social utility can be learned. % from the products that are above average in terms of preference utility of a pair of friends \cite{YL18TOIS}.} 
Finally, they are asked to provide $\lambda$ in [0,1]. We investigate the following research question: %Q1) Before visiting a VR store, are the participants anticipating \scenario? Q2)
After experiencing the VR store, are the participants satisfied with the \configuration s generated by \algo, PER, FMG, and GRF   ? User feedbacks are collected in Likert score \cite{likert} from 1 to 5 (very unsatisfactory, unsatisfactory, average, satisfactory, and very satisfactory). Each group of participants visits the VR stores twice via hTC VIVE with the items selected by each scheme in randomized order. 

Figure \ref{fig:user_lambda} reports that $\lambda$ values specified by the users range from 0.15 to 0.85 with the average as 0.53, indicating that both personal preferences and social interactions are essential in VR group shopping. %For Q1, an instance of \prob\ and the solutions of \algo, PER, and FMG are respectively shown to the participants in the questionnaire for review to find the most anticipated one before visiting our VR store. Figure \ref{fig:user_prob} presents the user anticipation of different approaches in \scenario. The results manifest that the participants prefer the solution of \algo\ more than that of PER and FMG by at least 29.2\%. For Q2, 
%, while Figure \ref{fig:user_sat} presents the percentage of user satisfaction improvement of AVG against different approaches.\footnote{\algor\ and \algod\ both find the optimal solutions in all the user study cases.} 
Figure \ref{fig:user_obj} compares the total \scenario\ utility as well as the recorded user satisfaction of each method. \algo\ outperforms the baselines by at least 34.2\% and 29.6\% in terms of the average total \scenario\ utility and average user satisfaction, respectively. The difference of \algo\ is statistically significant (p-value $\leq$ 0.019 $<$ 0.05). %The variance of user satisfaction improvement for GRF is large since GRF may split close friends into subgroups that do not share a common view on any item. In other words, users may not enjoy social interactions with friends of common interests during group shopping.
It is worth noting that we also calculate the correlation between the \scenario\ utility and user satisfaction (Spearman correlation 0.835; Pearson correlation 0.814), which manifest that the \scenario\ utility is a good estimation of user satisfaction.

%Comparing Figure \ref{fig:user_prob} and \ref{fig:user_sat}, the participants have a lower anticipation of group recommendation than personalized recommendation because they think their desired items may not be displayed. However, the user satisfaction of FMG becomes closer to PER after experiencing VR, because VR group shopping provides interactive shopping experience similar to offline shopping, and social discussions are thereby important, e.g., friends sometimes hangout and shop together to improve their relationship. Since the detailed user behaviors are logged, we analyze the videos during shopping and find the total number of interactions between participants for AVG is 32.9\% and 47.2\% greater than that of FMG and GRF respectively, indicating that users are more immersed in group shopping with close friends and homophily users found by AVG. 
Figures \ref{fig:user_density} and \ref{fig:user_share_alone} report the subgroup metrics in the user study datasets. GRF, which separates users into subgroups according to preference similarities, returns a low normalized density (0.21), i.e., users in the same subgroup tends to be strangers. Compared with the results in large-scale datasets (Figure \ref{exp:group_all}), GRF performs worse here since the normalized density is more sensitive when the user set is relatively small. In contrast, AVG flexibly assigns proper items to different subgroups of friends such that the normalized density is greater than 1 and the alone rate is 0\%.

%We interview a group comprised of 4 participants aged from 29 to 31. As quoted from the interview from one of them, ``Those common displayed items are really well chosen. I decided to buy some of the items after discussing with friends, but I wouldn't buy them if I came shopping alone. Most importantly, it is fun to view different items with different friends in each slot. I don't have to leave any of them alone due to our dissimilar interests any more with this technique in VR shop.'' That is, displaying common items based on social utilities does boost sales through fruitful social discussions. Moreover, from the perspective that group shopping is a sort of social event, friends with diverse interests can still enjoy shopping together in VR shops thanks to the CID technique.

%Through the user study, we find that males are more inclined to explore the displayed items for every participant right after entering the VR stores, while most females start shopping immediately without exchanging display information until they want other participants to join their views for discussions. We interview a group comprised of 3 males and 1 female aged from 29 to 31. As quoted from the interview from one of the male participant, ``It's fun to make jokes on friends when they are displayed with strange items such as a rocket. So, synchronizing displayed items first allows me to know where I can switch to their views for those items.'' That is, displaying distinct items to users also brings potential social benefit by entertaining male users, while offline shopping fails to do so since the whole group of users are forced to view common items together.

%Since we have different interests, it is more important to satisfy myself during shopping. However, it is sweet to display common items for me to ask friends for opinions.
%A group comprised of 4 colleagues and friends, including 3 males and 1 female aged from 29 to 31 and two of them is a couple. The female participant is often left alone (not co-displayed items with others) in the configurations due to her unique preference profile. We found that although her boyfriend is co-displayed preferred items with other male participants, he frequently changes to the female's views for interactions. As quoted from the interview of the female's boyfriends, "No, I don't like the items displayed to her at all. But she is my girl, I cannot leave her alone." That is, separating close friends into different subgroups may trigger them to change views for social interactions, even they are not interested to what their friends are displayed with.
%We interview a group comprised of 4 colleagues and friends, including 3 males and 1 female aged from 29 to 31. As quoted from the interview, ``This is my first time using VR shopping but the experience is really amazing. I think AVG is sweet because the VR store allows dynamically changing views to join discussions with other people.'' Moreover, several group members were strangers before the user study but become friends on Facebook after the immersive and interactive VR shopping experience.




==> stash/sec7_conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

To the best of our knowledge, there exists no prior work tackling flexible configurations under the envisaged scenario of VR group shopping. In this paper, we formulate the \prob\ problem to retrieve the optimal \configuration\ that jointly maximizes the preference and the social utility, \revise{and prove \prob\ is $\mathsf{NP}$-hard to approximate within a ratio of $\frac{32}{31} - \epsilon$}. We introduce an IP model and design a novel 4-approximation algorithm, \algo, and its deterministic version, \algod, by exploring the idea of \stagethreefull\ (\stagethree) that forms subgroups of friends to display them the same items. %\textbf{We extend \prob\ with practical VR operations and constraints to define the \problemtwo\ (\probtwo) problem, and prove that \probtwo\ cannot be approximated within a constant ratio in polynomial time. We extend \algo\ to support \probtwo\ and guarantee feasibility of the solution.}. 
Experimental results on real VR datasets manifest that our algorithms outperform baseline approaches by at least 30.1\% in terms of solution quality.
